Applied Choreographies

Choreographic Programming is a correct-by-construction paradigm where a compilation procedure synthesises deadlock-free, concurrent, and distributed communicating processes from global, declarative descriptions of communications, called choreographies. Previous work used choreographies for the synthesis of programs. Alas, there is no formalisation that provides a chain of correctness from choreographies to their implementations. This problem originates from the gap between existing theoretical models, which abstract communications using channel names (\`a la CCS/{\pi}-calculus), and their implementations, which use low-level mechanisms for message routing. As a solution, we propose the theoretical framework of Applied Choreographies. In the framework, developers write choreographies in a language that follows the standard syntax and name-based communication semantics of previous works. Then, they use a compilation procedure to transform a choreography into a low-level, implementation-adherent calculus of Service-Oriented Computing (SOC). To manage the complexity of the compilation, we divide its formalisation and proof in three stages, respectively dealing with: a) the translation of name-based communications into their SOC equivalents (namely, using correlation mechanisms based on message data); b) the projection of a choreography into a composition of partial, single-participant choreographies (towards their translation into SOC processes); c) the translation of partial choreographies and the distribution of choreography-level state into SOC processes. We provide results of behavioural correspondence for each stage. Thus, given a choreography specification, we guarantee to synthesise its faithful and deadlock-free service-oriented implementation.

==> abstract.tex <==
%auto-ignore
Choreographic Programming is a correct-by-construction paradigm for
concurrent, distributed
programming, where global declarative descriptions of communications
(choreographies) are used to synthesise deadlock-free communicating processes.
%
Choreographies are global descriptions of communications in concurrent systems,
which have been used in different methodologies for the verification or
synthesis of programs. However, there is no formalisation that provides a chain
of correctness from choreographies to their implementations. This problem
originates from the gap between previous theoretical models, which abstract
communications using channel names (à la CCS/$\pi$-calculus), and their
implementations, which use low-level mechanisms for message routing.

As a solution, we propose the framework of Applied Choreographies (AC). In AC,
programmers write choreographies in a language that follows the standard
syntax and semantics of previous works. Then, choreographies are compiled to a
real-world execution model for Service-Oriented Computing (SOC). To manage the
complexity of this task, our compilation happens in three steps, respectively
dealing with: implementing name-based communications using the concrete
mechanism found in SOC, projecting a choreography to a set of processes, and
translating processes to a distributed implementation in terms of services.
For each step a suitable correspondence result guarantees that the behaviour
is preserved, thus ensuring the correctness of the global compilation process.
This is the first correctness result of an end-to-end translation from
standard choreographies to programs communicating through correlation;
a communication mechanism widely used in SOC and microservice architectures.

==> additional_material.tex <==
%auto-ignore
\section{Applied Choreographies}

\input{applied_choreographies/figures/chor_semantics_sos}

\input{applied_choreographies/figures/chor_swap}

\newpage

\section{Typing}

In addition to the description in \cref{sec:typing} we comment the additional
rules in \cref{fig:typing_rules_full}. 

In Rule $\did{T}{End}$ $\end$ holds if the protocols for all sessions have
terminated (i.e., all local typings have type $\gend$). In Rule $\did{T}{Def}$
the condition $\Gamma' |_{\locs} \subseteq \Gamma$ checks that the body of
the recursive procedure does not introduce unexpected services
($\Gamma'|_{\locs}$ returns all service typings in $\Gamma'$).

\input{applied_choreographies/figures/chor_typing_rules_full}

\newpage

\input{applied_choreographies/figures/chor_typing_swap}

\input{applied_choreographies/figures/chor_typing_buffer}

\newpage

% \subsubsection{Typing Example}

% \input{applied_choreographies/examples/typing_example}

% \newpage

\section{Endpoint Projection}
We report the complete definition of choreography annotation, process
projection, merging function, and grouping function, respectively in
\cref{fig:cc_annotation}, \cref{fig:cc_projection},
\cref{fig:merging_function}, and \cref{fig:grouping}.

\input{applied_choreographies/figures/annotation}

\section{Dynamic Correlation Calculus}

\input{applied_choreographies/figures/jc_semantics}

\input{applied_choreographies/figures/jc_structural_congruence}

% \input{applied_choreographies/figures/compilation_example_supp}

==> endpoint_FC.tex <==
%auto-ignore
We end this section by presenting the definition of Endpoint Projection of FC and its target calculus, called Endpoint Frontend Calculus. Formally, eFC is a subset of FC, whose syntax corresponds to only partial actions of the Frontend Calculus, i.e., all FC terms except $\prid{start}$ and $\prid{com}$.
%
% In term $\prid{req}$, process $\pid p$ requests the creation of some external
% processes at their respective locations $\til l$ to start a new session $k$.
% By ``external'', we mean that the behaviour of such processes is defined in a
% separate choreography module. Role annotations are as for term $\prid{start}$.% in which $\pid p$ will play role $\role A$ 
% %  $\wtil{l.\role B}$ means that each location $l$ in
% % $\wtil{l.\role B}$ is expected to spawn a process that behaves as specified by
% % the related role $\role B$.
% Term $\prid{acc}$ is the dual of $\prid{req}$ and defines a choreography module that provides the 
% implementation of some service processes.
% % The dual of $\prid{req}$ is term $\prid{acc}$,
% % which provides the implementation of service processes.
% % Specifically, term
% % $\prid{acc}$ defines a reusable choreography module that accepts, at locations
% % $\til l$, the creation of processes $\pids q$ playing their respective roles
% % $\roles B$.
% %
% We assume that $\prid{acc}$ terms are always at the top level (not guarded by other actions).
% % Following the design idea that services should always be available, shared by
% % other models~\cite{CHY12,CM13}, we assume that all $\prid{acc}$ terms in a
% % choreography are at top level (not guarded by other actions).
% %
% In term $\prid{send}$, process $\pid p$ sends a message to an external process that plays $\role B$ in session $k$.
% Dually, in term $\prid{recv}$, process $\pid q$ receives a message for one of the operations $o_i$ from an external 
% process playing role $\role A$ in session $k$, and then proceeds with the corresponding continuation
% --- this is the standard branching found in session-oriented calculi~\cite{HVK98,HYC08,MY13}.
%
% \subsection{Semantics} % (fold)
%
Running eFC choreographies are paired with the deployment $\env$, hence the semantics of eFC is (a subset of) the semantics of FC.
% \input{figures/eFC_semantics}

==> examples/choreography_example.tex <==
\subsection{An example} % (fold)
\label{sub:example}
%
We show an example of a system for verified file transfer written in AC. We use
the example in 
%\cref{sec:endpoint_projection} and 
\cref{sec:compiler} to illustrate our 
%endpoint projection and 
compilation.

\paragraph{Verified file transfer.}
\input{figures/choreography_example}
%
The program \emph{i}) validates the file request of a Client on a Server,
\emph{ii}) transfers a file in multiple parts, and \emph {iii}) verifies the
transfer with a checksum. The Server logs all requests.
%
We report in \cref{fig:choreography_example} the code of program $C$,
parallel composition of the two partial choreographies $C = C_c \pp C_s$.
$C_c$ and $C_s$ respectively define the client- and the server-side code.

In $C$, process $\pid c$ --- the only active process --- plays the role of the
Client $\role C$. In $C_s$, $\pid a$ plays the Access Manager ($\role A$),
$\pid{dm}$ the Download Manager ($\role{DM}$) and $\pid l$ the Logger ($\role
L$). In $C_c$ (Line 18 of $C_c$) process $\pid f$ plays $\role F$, accessing
the file system. We locate $\role A, \role{DM}$, $\role L$, and $\role F$ at
respectively $l_\role A$, $l_\role {DM}$, $l_\role L$, and $l_\role C$.

Lines 1 of $C_c$ and $C_s$ start session $k_d$ between $\pid c, \pid a, \pid
{dm}$, and $\pid l$. At Lines 2 of $C_c$ and $C_s$, $\pid c$ makes a request
for a file to $\pid a$.
%
Lines 4-15 of $C_s$ define the outcome of a valid request (Line 3). Following
the Lines, $\pid a$ forwards the resource request to $\pid {dm}$ and confirms
(on $ok$) to $\pid c$ the request. $\pid{dm}$ asks $\pid l$ to $log$ the
request.
%
Lines 7-14 define the recursive procedure TRANSFER, called at Line 15, for the
multi-part file download. If $\pid {dm}$ has $\m {more}$ packets of the
resource, it sends the $\m{next}$ to $\pid c$ on operation $pkt$ and TRANSFER
repeats. Else $\pid{dm}$ ends $k_d$ sending to $\pid c$ the checksum of the
file.
% 
Lines 17-19 of $C_s$ specify the outcome of an invalid request: $\pid a$
notifies $\pid {dm}$ and $\pid c$ of the failed attempt ($ko$) and $\pid{dm}$
asks to $log$ the event to $\pid l$.

Observe that $C_c$ defines at Lines 3-15 a procedure to STORE the file. At
Line 18 of $C_c$, after the approval, $\pid c$ (playing user $\role U$) starts
a new session $k_s$ with $\pid f$, asking $\pid f$ to create a file to store
the incoming packets. Then, in STORE, if $\pid c$ receives a new packet of
bytes from $\pid{dm}$ (Line 5), it asks $\pid f$ to append them to the local
file and STORE repeats. Else $\pid c$ receives the checksum from $\pid {dm}$
(Line 8) and $\pid c$ forwards it to $\pid f$. Finally, $\pid f$ notifies
$\pid c$ whether it $saved$ or $discarded$ the file wrt the checksum.

\begin{remark} To illustrate compositionality of ACs, we (logically) divided
	the example into two choreographies, (resp. the client- and server-side
	described above). However, we could specify the system as single
	choreography, e.g.,
	%
		{\footnotesize$$ 1.\ \start{k_d}{\prc cC}{l_{\role A}.\prc aA,
			l_{\role{DM}}.\prc {dm}{DM},l_{\role L}.\prc lL};
			\quad 2.\ \com{k_d}{\prc cC.\m{mkReq()}}{\prc aA.get(\jpath{req})};
			\quad
			\ldots $$}
\end{remark}

We comment some features of AC programs in the example.

\paragraph{Session Descriptors.} At Lines 1 of $C_c$ and $C_s$ $\pid c$
requests to start a new session $k_d$ with some service processes $\pid a$,
$\pid{dm}$, and $\pid l$. We describe the structure of the session descriptor,
stored in the state of the mentioned processes under path $\jpath{kd}$.

\begin{figure}
\begin{center}\includegraphics[width=.9\columnwidth]
{figures/structure_of_k}\end{center}
\caption{Example of structure of Session Descriptor}
\label{fig:example_session_descriptor}
\end{figure}

We report in \cref{fig:example_session_descriptor} such structure.
Following the path $\jpath{A}$, we find a subtree with \emph {i}) a node
$\jpath{l}$ that stores the location $l_{\role A}$ of $\pid a$ and
\emph{ii}) a set of nodes, named after all the other roles in $k_d$, leading
to subtrees containing the correlation keys related to the roles in the paths.
%
For example, the path $\jpath{A.C}$ points the tree $t_\role{AC}$, which
contains the correlation key used by $\pid a$ to send messages to $\pid c$.

\paragraph{Parallelism.}
%
Lines 5-6 of $C_s$ show how Rule $\did{C}{Eq}$ can exchange the order of
execution of actions. The actions at Lines 5 and 6 regard different processes
(resp. $\pid a$, $\pid s$, and $\pid l$) and the two instructions can swap
along Rule $\did{CS}{EtaEta}$ of the swap relation.
%
A possible reduction of $C$, starting from Line 5 of $C_s$, can apply Rule
$\did {C} {Eq}$ to swap Lines 5 and 6, reduce Line 6 with Rule $\did{C}{Com}$
to a partial reception for process $\pid l$, and swap back the two Lines.
Next, either $\pid a$ delivers its message with $\did{C}{Send}$ or
$\did{C}{Eq}$ applies, letting $\pid l$ consume its message. Observe that the
swap is non-deterministic, allowing other possible executions.

\paragraph{Asynchrony.} AC supports asynchronous communication with queues,
however, we need the swap relation to let a process send or receive a message
asynchronously.
%
% and despite its choreography defines that other actions should happen before
% it.
%
Consider Lines 4-5 of $C_s$. We can apply $\did{C}{Com}$ on Line 4 and let
$\pid a$ send its message to $\pid {dm}$. This reduces Line 4 to a partial
reception on $\pid {dm}$. Then, we can apply $\did{C}{Eq}$, swap the redex of
Line 4 with Line 5, and let Line 5 execute with $\did{C}{Send}$. Finally, we
let $\pid{dm}$ consume its message with $\did{C}{Recv}$ on Line 4.

==> examples/choreography_example_new.tex <==
\begin{example}
\alert{Bla bla example in \cref{fig:example}.}

Codice modulare e multisessioni.

\noindent\hspace{15pt}\begin{minipage}{.55\textwidth}
\begin{lstlisting}[numbers=left,mathescape,backgroundcolor=\color{white},escapeinside=||]
|\Suppressnumber|$\ldots \mbox{as Lines 1--2 in \cref{example:intro}}
\ldots$|\Reactivatenumber{3}|
$\addCode{\req{k'}{\pid s[\role S]}{l_{\role D}.\role D}}$
$\addCode{\com{k'}{\pid s[\role S].\m{mkShipping}( x )}{\role D.ship}};$
$\addCode{\com{k'}{\role D}{\pid s[\role S]}{.shipCosts( y )};}$
$\com{k}{\pid s[\role S].\m{mkOrder}( x, y )}
	{\pid b[\role B].openTx( order )};$
$\com{k}{\pid c[\role C].cc}{\pid b[\role B].pay( cc )};$
\end{lstlisting}
\vspace{-5pt}\rule{360pt}{.5pt}
\end{minipage}
\begin{minipage}{.35\textwidth}
\begin{lstlisting}[numbers=left,mathescape,backgroundcolor=\color{white},
firstnumber=9]
$\m{if}\ \pid b.\m{closeTx}( cc, order )$
 $\com{k}{\pid b[\role B]}{\pid c[\role C].ok()};\
 \com{k}{\pid b[\role B]}{\pid q[\role S].ok()};$
 $\addCode{\com{k'}{\pid s[\role S]}{\role D.confirmShipping()}}$
$\m{else}$
 $\com{k}{\pid b[\role B]}{\pid c[\role C].ko()};\
 \com{k}{\pid b[\role B]}{\pid q[\role S].ko()};$
 $\addCode{\com{k'}{\pid s[\role S]}{\role D.discardShipping()}}$
\end{lstlisting}	
\end{minipage}

\noindent\hspace{15pt}\begin{minipage}{.55\textwidth}
\begin{lstlisting}[numbers=left,mathescape,backgroundcolor=\color{white}]
$\addCode{\acc{k'}{l_{\role D}.\pid d[\role D]};}$
$\addCode{\com{k'}{\role S}{\pid d[\role D].ship( order )};}$
$\addCode{\com{k'}{\pid d[\role D].\m{quoteShip}( order )}{\role S.shipCosts};}$
\end{lstlisting}
\end{minipage}
\begin{minipage}{.45\textwidth}
\begin{lstlisting}[numbers=left,mathescape,backgroundcolor=\color{white},
firstnumber=4]
$\addCode{\com{k'}{\role S}{\pid d[\role D]}.\{}$
 $\addCode{confirmShipping(),}$
 $\addCode{discardShipping()} \quad \}$
\end{lstlisting}
\end{minipage}

\end{example}


==> examples/compilation_example.tex <==
% \subsection{Compilation example}

% As an example of compilation let us consider the choreography $$\epp{C}{} =
% \epp{C}{\pid c} \pp
% \epp {C} {\pid f} \pp \epp{C} {\pid a} \pp \epp{C}{\pid {dm}} \pp \epp{C}
% {\pid l}$$ commented in \cref{sec:epp_example}, projection of the
% choreography $C = C_c \pp C_s$ presented in \cref{sub:example}.
% %
% We associate a default deployment $\env$ to $\epp{C}{}$ such that for some
% $\Gamma$ and $\env$ \emph{i}) $\Gamma \hlseq {\env,\epp{C}{}}$ holds;
% \emph{ii}) the location of process $\pid c$ is $l_\role C$. $l_\role C$
% is also the location of the service process $\pid f$, which allows us to show
% how the compilation of active and service processes work. 
% %
% \cref{fig:example_compilation} reports the result of the compilation
% $\genenc{\env,\epp{C}{}}$ where, on top it shows the composition of
% compiled services and below it, from left to right, the compiled behaviours of
% processes $\pid {c}$, $\pid {a}$, and $\pid l$.
%
\input{figures/compilation_example.tex}
%
% We highlight some salient parts of the compilation to illustrate how
% $\genenc{\env,\epp{C}{}}$ behaves accordingly to $\env,\epp{C}{}$. 
% %

% \paragraph{Compiled Services.}
% The network of compiled services, on top of
% \cref{fig:example_compilation}, shows that there is a compiled service
% for all locations ($l_\role C, l_\role A, l_\role{DM}$, and $l_\role L$) in
% $C$.
% %
% In particular, $S_c$, the service located at $l_\role C$, contains
% \emph{i}) as its start behaviour the compilation of the process projection of
% $\pid f$ (which accepts requests on $l_\role C$ in $C$) and \emph{ii}) a
% running process whose behaviour is the compilation of the process projection
% of $\pid c$, and whose state and queue map are those of $\pid c$ in
% $\env$.% % The other services
% % $S_a$, $S_{dm}$, and $S_l$ are similar and contain as start behaviour the
% % compilation of the projections on $\pid a$, $\pid {dm}$, and $\pid l$,
% % respectively.

% \paragraph{Starting a new session.}
% Lines 1-12 of $\genenc{\epp{C}{\pid c}}$ show an excerpt of the compiled code
% of the request to start session $k_d$ for process $\pid c$: $\req{k_d}{\prc
% cC}{l_{\role A}.\role A,l_{\role{DM}}.\role{DM},l_{\role L}.\role L}$. 
% %
% As defined by function $\m{start}$, at Lines 1-4 the process sets the locations
% of all involved roles in the Session Descriptor, rooted in $\jpath{kd}$.
% %
% Lines 5-7 define the interaction to start the process playing role $\role A$:
% line-wise, the process creates the queue to received from role $\role A$, it
% requests the creation of a new process at the relative location $\jpath
% {kd.A.l}$, passing to it the Session Descriptor, and, it waits for the process
% to return the updated Session Descriptor. Lines 10-12 signal the start of the
% session to all the started processes.
% %
% Lines 1-6 of $\genenc{\epp{C}{\pid a}}$ and $\genenc{\epp{C}{\pid l}}$ show
% the code that complements the start.
% %
% At the end of the procedure, $\env, \epp{C}{}$ and $\genenc{\env,\epp
% {C} {}}$ properly set a Session Support for session $k_d$.

% \paragraph{In-session message passing.}\hspace{0pt}
% %
% We show that the originating choreography and its compilation handle
% communications similarly. We compare the execution of Lines 2 of $\epp{C}{\pid
% c}$\footnote{Although not shown in the paper, Line 2 of $\epp{C}{\pid c}$
% corresponds to Line 2 of $C_c$ as partial actions are projected verbatim on
% their process by the EPP.} and $\epp{C}{\pid a}$ with that of Line 13 of
% $\genenc {\epp {C}{\pid c}}$ and Line 7 of $\genenc{\epp{C}{\pid a}}$.


% % . 
% % %
% % Line 2 of $\epp{C}{\pid c}$ corresponds to line 13 of $\genenc{\epp{C}{\pid
% % c}}$ and line 2 of $\epp{C}{\pid a}$ corresponds to line 7 of $\genenc{\epp{C}
% % {\pid a}}$.
% % %
% % Considering the execution of $C_c \pp C_s$ at lines 2, we have (let $C_c'$ and
% % $C_s'$ resp. continuations of $C_c$ and $C_s$):
% % %
% % {\footnotesize
% % $$\begin{array}l
% % \env,\com{k_d}{\prc cC.\m{mkReq()}}{\role A.get};C_c' \pp \com{k_d}{\role C}
% % {\prc aA.get(\jpath{req})};C_s' \quad \to
% % \\[2pt]
% % \env',C_c' \pp \com{k_d}{\role C}
% % {\prc aA.get(\jpath{req})};C_s' \quad \to \quad \env'',C_c' \pp C_s'
% % \end{array}$$
% % }
% %
% Let $\env$ be the deployment associated with $\epp{C}{}'$, reduction of $\epp
% {C}{}$ to the considered Lines. $\env, \epp{C}{}' \to \env',\epp{C}{}''$
% applying Rule $\did{C}{Send}$ on Line 2 of $\epp{C}{\pid c}$. In $\env'$ the
% queue in which $\pid a$ receives from $\pid c$ contains the sent message:
% $\env'( \pid a ).\equeues( t_c ) = (get, t_m)$, $t_c$ correlation key rooted at
% $\jpath{kd.C.A}$ in the state of $\pid c$ and $t_m$ evaluation of function
% $\m{mkReq()}$.
% %
% Similarly, Line 13 of $\genenc {\epp {C}{\pid c}}$ reduces with Rule
% $\did{DCC}{Send}$. The Rule delivers the message on operation $get$, carrying the evaluation of $e$, to the service located at $\jpath
% {kd.A.l}$,
% which contains all service processes compilation of $\pid a$, and in the queue
% correlating with $\jpath {kd.A.C}$.
% %
% By the compilation, the compiled process relative to $\pid c$ has the state of
% $\pid c$, hence, the value rooted at $\jpath {kd.A.C}$ is equal to $t_c$,
% $\jpath{kd.A.l}$ is equal to the location of $\role A$, and the evaluation of
% $e$ is equal to $t_m$. Moreover, since the network has just started (at Line 13
% of $\genenc{\epp{C}{\pid c}}$ and correspondent), we know that the receiving
% process had no message in the queue correlating with $\jpath {kd.A.C}$, thus,
% after the reduction, it only has message $(get, t_m)$.
% The state of $\env',\epp{C}{}''$ corresponds to the state of
% $\genenc{\env',\epp {C}{}''}$.
% %
% On this result, if $\env',\epp{C}{}''$ reduces with Rule $\did{C}{Recv}$,
% $\genenc{\env',\epp {C}{}''}$ can apply Rule $\did{DCC}{Recv}$ and we are sure
% that \emph{i}) the consumed message by the receiver ($\pid a$ and its compiled
% correspondent) is $(get, t_m)$, \emph{ii}) the relative queues are now
% empty, and \emph{iii}) the receiver included in its state $t_m$ under
% path $\jpath{req}$.

% % In the first reduction, $\pid c$ sends its message to $\pid a$ following rule
% % . As a result, $\env$ is modified in such way that its update
% % $\env'$ has
% % %
% % $\env'( \pid a ).\equeues( t_c ) = (get, t_m)$
% % %
% % , where $t_m$ is the result of the evaluation of function $\m{mkReq()}$ and
% % $t_c$
% % the correlation key used by $\pid c$ to send messages to $\pid a$ ($t_c =
% % \jpath{kd.C.A}(\env (\pid c ).\estate )$).
% % %
% % Then rule $\did{C}{Recv}$ applies and $\pid a$ receives the message sent from
% % $\pid c$. $\env''$, update of $\env'$, stores this effect by picking (removing)
% % the first message from the corresponding queue of $\pid a$ and by assigning its
% % content ($t_m$) to variable $\jpath{req}$, hence $\jpath{req}(\env''(
% % \pid a ).\estate) = t_m$ and $\env''( \pid a ).\equeues( t_c ) = \emptyseq
% % $.

% % Let us now look at the related reductions of the compilation of
% % $\genenc{\env,\epp{C}{}}$. Let $P_\pid c$ be the DCC process at $S_c$ result of
% % the compilation of $\epp{C}{\pid c}$ and $P_\pid a$ the correspondent DCC
% % process started by $P_\pid c$ in service $S_a$.
% % %
% % The execution of line 13 of $\genenc{\epp{C}{\pid c}}$ and Line 7 of $\genenc{\epp
% % {C}{\pid a}}$ reduces with rule $\did{DCC}{Send}$
% % %
% % {\footnotesize
% % $$
% % 	\jsrv{\genenc{\epp{C}{\pid f}}, P_\pid c}{l_\role	C} \pp
% % 	\jsrv{\ \genenc{\epp{C}{\pid a}}, P_\pid a}{l_\role A} \to
% % 	\jsrv{\genenc{\epp{C}{\pid f}}, P_\pid c'}{l_\role	C} \pp
% % 	\jsrv{\ \genenc{\epp{C}{\pid a}}, P_\pid a'}{l_\role A}
% % $$}
% % %
% % $P_\pid c$ consumes Line 13 and reduces to $P_\pid c'$. $P_\pid c'$ is equal to
% % $P_\pid c$ except that its behaviour starts from Line 14 of $\genenc{\epp{C}
% % {\pid c}}$. 

% % Let $t = \env( \pid p ).\estate$ and $M = \env( \pid a
% % ).\equeues$

% % \noindent$P_\pid a = \jprc{\oneway{get}{\jpath{req}} \qfrom{\jpath
% % {kd.C.A}};\ldots} {t} {M}$

% % $P_\pid a$ reduces, with rule $\did{DCC}{Send}$, to

% % \noindent$P_\pid a'=\jprc{\oneway{get}{\jpath{req}}
% % \qfrom{\jpath{kd.C.A}};\ldots}{t} {M'}$

% % where $M'( t_c ) = (get, t_m)$, which is the same effect commented above
% % produced by $\did{C}{Send}$.
% % % Notably, we are sure that the AC process $\pid
% % % a$\footnote{\alert{actually sarebbe il processo freshly named che interpreta
% % % $\role A$ in $l_\role A$}} and $P_\pid a$ have the same queues and values
% % % because the latter has the state and queue mapping of the former by the
% % % definition of the compilation.
% % %
% % Next, $P'_\pid a$ can receive the message sent by $P_\pid c$ with rule $\did
% % {DCC}{Recv}$
% % %
% % {\footnotesize
% % $$
% % 	\jsrv{\genenc{\epp{C}{\pid f}}, P'_\pid c}{l_\role	C} \pp
% % 	\jsrv{\ \genenc{\epp{C}{\pid a}}, P'_\pid a}{l_\role A} \to
% % 	\jsrv{\genenc{\epp{C}{\pid f}}, P_\pid c'}{l_\role	C} \pp
% % 	\jsrv{\ \genenc{\epp{C}{\pid a}}, P_\pid a''}{l_\role A}
% % $$
% % }
% % %
% % Where

% % \noindent$P_\pid a''=\jprc{\cond{isValid( \jpath{req} )}{\ldots}{\ldots} }
% % {t'} {M''}$

% % in which $t' = t \tcopy{\jpath{req}}{t_m}$ and therefore $\jpath{req}(t') =
% % t_m$ and $M''( t_c ) = \emptyseq$.
% % %
% % As expected, this is the same effect of the execution of $\did{C}{Recv}$ in

% % the choreography.

==> examples/projection_example.tex <==
\subsection{Projection Example}
\label{sec:epp_example}
\input{figures/projection_example.tex}

As an example, we project the choreography $C = C_c \pp C_s$ presented in
\cref{sub:example}. Applying the definition of EPP to $C$ we
obtain $\epp{C}{} = \epp{C}{\pid c} \pp \epp{C}{\pid f} \pp \epp{C} {\pid a}
\pp \epp{C}{\pid {dm}} \pp \epp{C}{\pid l}$.
%
\cref{fig:example_epp} reports some excerpts of $\epp{C} {}$,
i.e., $ \epp{C}{\pid a}$, $\epp{C}{\pid {dm}}$, and $\epp {C}{\pid l}$. We
illustrate how $\epp{C}{}$ implements the same behaviour of $C$.

\paragraph{Start.} The start of a new session, like the one at Lines 1 of $C_c$
and $C_s$, applies the same effect in the projection. Let $\epp{C}{\pid p}'$ be
the continuation of the process projection of $C$ on $\pid p$ after Line 1. The
execution of Lines 1 of the process projections composing $\epp {C} {}$ is
%
{\footnotesize$$
\hspace{-5pt}\begin{array}{l}
\env,\begin{array}{l}
\req{k_d}{\prc cC}{l_{\role A}.\prc aA,l_{\role {DM}}.\prc {dm}{DM},l_ {\role
L}.\prc lL}; \epp{C}{\pid c}' 
\\
\pp  
\acc{k_d}{l_{\role A}.\prc aA}; \epp{C}{\pid a}' \pp
\acc{k_d}{l_{\role {DM}}.\prc {dm}{DM}}; \epp{C}{\pid s}' 
\\
\pp
\acc{k_d}{l_{\role L}.\prc lL}; \epp{C}{\pid l}' \pp \epp{C}{\pid f}
\end{array}
\to
\env',\ \epp{C}{\pid c}' \pp \epp{C}{\pid a}' \pp \epp{C}{\pid {dm}}' \pp
\epp{C}{\pid l}' \pp \epp{C}{\pid f}
\end{array}
$$}
%
Let the location of process $\pid c$ be $l_\role C$ in $\env$. The effect of
the start is $\delta=\deltastart{k_d} {l_{\role C}.\pid c [\role C],l_{\role
A}.\prc aA,l_{\role {DM}}.\prc {dm}{DM},l_ {\role L}.\prc lL}$ which can
generate the same $\env'$ as the start at Lines 1 of $C_c$ and
$C_s$.

\paragraph{Communications.} The EPP projects a complete communication to a
partial send for the sender and a partial receive for the receiver. Line 6 of
$C_s$ is\\
%
$\com{k_d}{\prc {dm}{DM}.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})}$
%
and in $\epp{C}{}$ it is projected into a partial send for $\pid {dm}$ (at Line
4 of $\epp {C}{\pid {dm}}$) and a partial receive for $\pid{l}$ (at Line 2 of
$\epp{C}{\pid l}$). The semantics of Line 6 of $C_s$ and that of Line 4 of
$\epp {C}{\pid {dm}}$ and Line 2 of $\epp{C}{\pid l}$ is equal as the complete
action breaks into a partial send, equal to the effect of Line 4 of $\epp {C}
{\pid {dm}}$, and continues as a partial receive, equal to $\epp {C} {\pid l}$.

\paragraph{Conditionals.} 
The EPP of a conditional merges the behaviour of all processes in its branches
as branched receptions. For example, at Line 3 of $C_s$, process $\pid a$
evaluates a condition that either branches in the behaviour described at Lines
4-15 or at Lines 17-19. At Line 3 of $\epp{C}{\pid
a}$ the conditional is preserved verbatim.
%
For the other processes present in the branches of the conditional, the EPP
merges their behaviours on a branched reception: $\epp{C}{\pid{dm}}$ projects
the conditional on the branches guarded by operations $ok$ or $ko$ (resp. at
Lines 3 and 6). $\epp{C} {\pid l}$ merges the branches of the conditional into
a single branch on operation $log$, at Line 2.

==> examples/typing_example.tex <==
\input{figures/protocols_example}
%
We show, in \cref{fig:preview_example_protocols}, how we can write the
protocols that type the example choreographies in \cref
{fig:choreography_example}. Notably, we define two independent protocols that
are implemented, composed, and interleaved at runtime by the choreographies
they type.
%
The first protocol, called $G_d$, specifies the interaction of the system that
allows a Client to authenticate on a Server, download a file from it, and
verify its integrity, also logging all requests.
%
The roles in the protocol are the same used in \cref
{fig:choreography_example}, i.e., $\role C$ for the Client, $\role{DM}$ for
the download manager, $\role A$ for the access manager and $\role L$ for the
logger.

Following $G_d$, $\role C$ asks to to $\role A$ $get$ a file with a message
that must contain two values of type $\tstring$: $\jpath{creds}$ for the
credentials of $\role C$ and $\jpath{rsc}$ for the resource identifier of the
file (e.g., a URL). $\role A$ notifies $\role{DM}$ whether the credentials
and the resource identifier are valid or not:

\begin{itemize}
	\item If they are not, $\role A$ forwards to $\role{DM}$ the outcome of the
	validation ($\tstring$) on operation $ko$. $\role A$ also sends an empty
	message\footnote{empty parentheses are a short-cut for type $\tunit$} to
	$\role C$ on operation $ko$ as response to the failed attempt. Finally,
	$\role {DM}$ ends the branch forwarding to $\role L$, on $log$, the error
	received from $\role A$.

	\item If they are valid, $\role A$ sends to $\role{DM}$ the identifier of
	the file on operation $ok$. $\role A$ confirms the request to $\role C$
	with an empty message on operation $ok$. $\role {DM}$ asks to $log$ the
	request of the file ($\tstring$) to $\role L$. The protocol continues
	with the definition of procedure $\m{rec}\;\mathbf{t}$ where $\role {DM}$ sends to $\role C$ either: \emph{i}) a chunk (packet) of $\tbytes$ of the file, on $pkt$, and repeats $\mathbf{t}$, or \emph{ii}) the checksum of the file, on $chksum$, if there are no more	packets, ending the protocol.
\end{itemize}
%
The second protocol, $G_s$, defines the interaction between the User
$\role U$ of an operative system and a process $\role F$ that accesses the
filesystem. In $G_s$, $\role U$ asks to $\role F$ to $create$
a new file ($\tstring$). Then the protocol defines the procedure $\m{rec}\;\mathbf{s}$. $\role U$ can either ask $\role F$ to \emph{i}) $append$ a new packet of $\tbytes$ to the file, repeating $\mathbf{s}$ or \emph{ii}) $check$ the file against its checksum ($\tstring$). Based on the outcome of the checksum, $\role F$ either notifies $\role U$ that it $saved$ the file, or $discarded$ it.

==> figures/annotation.tex <==
\begin{figure}
$$\begin{array}{rcl}
			@C & = & \emptyset@C \hfill
			\\\\
			d@C & = & \begin{cases}
				\eta ; d@C'								& \mbox{if } C = \eta ; C'
				\\
				d@C_1 \pp d@C_2 					& \mbox{if } C = C_1 | C_2
				\\
				\com{k}{\role A}{\pid q[\role B].\{o_i(x_i);d@C_i)\}_{i \in I}}
																						& \mbox{if } C = \genbranchI
				\\
				\recDef{X\carr{\pids p}}{d'@C''}{d'@C'}
																						& \mbox{if } 
																							\begin{array}l
																							C = \recDef{X}{C''}{C'} 
																							\ \wedge \
																							\\
																							\pids p = \fp(C'')
																							\ \wedge \
																							d' = d \cup 
																								(X,X\carr{\pids p})	
																							\end{array}

				\\
				\genacc ; d@C' 											&	\mbox{if } C = \genacc ; C'	
				\\
				\cond{\pid p.e}{d@C_1}{d@C_2}
																						& \mbox{if } 
																							C = \cond{\pid p.e}{C_1}{C_2}
				\\
				\recCall{X\carr{\pids p}} 					&	\mbox{if } C = X
																							\ \wedge \ 
																							(X,X\carr{\pids p}) \in d
				\\
				\inact															& \mbox{if } C = \inact
			\end{cases}
\end{array}$$
	\caption{Choreography Calculus --- Annotation operator}
	\label{fig:cc_annotation}
\end{figure}

==> figures/cc_example_1.tex <==
\begin{figure}
$
\begin{array}{l}
	g = \gcom{\role A}{\role B}{login(\tvoid)}; \\
			\qquad \gcom{\role B}{\role A}{\{ \;
					ok(\tstring);\gend \; , \; 
					ko( \tstring ); \gend
				\; \}}	
	\\\\
	l \;\m{impl}\; g[B]
	\\\\
	\start{k[g]}{\pid p[\role A]}{l.\pid q[\role B]};
	\\
	\com{k}{\pid p[\role A].\jpath{crds}}
		{\pid q[\role B].login(\jpath{crds} )};
	\\
	\cond{\pid q.authOk(\jpath{crds})}
		{ \\\quad\com{k}{\pid q[\role B]}{\pid p[\role A].ok( \jpath{redir} )\\}}
		{ \\\quad\com{k}{\pid q[\role B]}{\pid p[\role A].ko( \jpath{error} )\\}}
\end{array}
$
	\caption{Example of Complete Choreography}
	\label{fig:cc_example_1}
\end{figure}

==> figures/chor_env_aux_ops.tex <==
\begin{figure*}
\begin{displaymath}
\begin{array}{c}
% 	\env[\pid p,t_c \mapsto \til m] = 
% 	\env\big[ \pid p, \equeues \mapsto 
% 		\env(\pid p).\equeues[ t_{c} \mapsto \til m ]\big]
% \qquad \qquad
\\[5pt]
\env[\pid p, \equeues, t_c \mapsto \til m] =
\env\Big[ \pid p \mapsto \env(\pid p)\big[ \equeues \mapsto 
	\env( \pid p).\equeues[ t_c \mapsto \til m]\big] \Big]
\;\; \prid{\equeues\mbox{-}up}
\qquad \qquad
\env[\pid p, \estate \mapsto t] =
\env\big[ \pid p \mapsto \env(\pid p)[ \estate \mapsto t] \big]
\; \prid{\estate\mbox{-}up}  
% \\[10pt]
% \env[ \m{M}_i ]_{i\in I} =  \env[ \m{M}_j ][ \m{M}_i ]_
% {i
% \in I/ \{j\}}, j \in
% I 
% \;\; \prid{s\mbox{-}up} 
% \hfill
% \env[ \m{M}_i ]_{i\in I,j \in J} = \env[ \m{M}_h ]_{j \in J}[ \m{M}_i ]_{i \in
% I/
% \{h\},j \in J}, h \in
% I
% \;\; \prid{cs\mbox{-}up}
% \\[8pt]
% \prid{\m{sd}\mbox{-}up}
% \quad
% \left.\begin{array}l
% 	J = I\setminus\{i\}, \quad t_h = t_{locs}\tcopy{t_{sd}}{\jpath k}
% 	\\
% 	t_{locs} =	t_\bot \bigtcopy_{i \in I}(\ {\jpath{k.A_{\mathit i}.l}},{
% 	(l_i,\emptyset)}\ )
% 	\\
% 	t_{sd} = t_\bot \bigtcopy_{i \in I,j \in J}(\ {\jpath{k.A_{\mathit i}.A_
% 	{\mathit
% 	j}}},
% 			{ t_{\role A_i \role A_j}}\ )
% 	\\
% 	\m{fresh}(\env,l_i,t_{\role A_j \role A_i})
% \end{array}\right\}
% 	\m{sd}(\ \env,(\ l_i.\pid p_i[\role A_i]\ )_{i\in I},k\ )
% 		=	\env
% 	\begin{array}{l}
% 		\left[\
% 			\pid p_i,\equeues, t_{\role A_j \role A_i} \mapsto \epsilon\ 
% 		\right]_{i \in I, j \in J}
% 		\\
% 		\big[\ 
% 			\pid p_h,\estate \mapsto \env(\pid p_h).\estate 
% 				\tcopy{\jpath{k}}{t_h}
% 		% 		\bigtcopy_{j\in I,h\in I\setminus\{i\}}
% 		% ({\jpath{k.A_{\mathit j}.A_{\mathit h}}},{ t_{\role A_j \role A_h}})
% 		\ \big]_{h \in I}	
% 	\end{array}
%
% \left.\begin{array}l
% t_{l} = t_\bot
% \bigtcopy_ {i}
% 	(\ \jpath{k.A}_i\jpath{.l}, l_i \ ) 
% \\
% t_{q} = t_\bot
% 	\bigtcopy_{i,j}(\ \jpath{k.A}_i\jpath{.A}_j, 
% 		\m{\fresh queue\_id}(\env, l_j) \ )
% \\[5pt]
% t_{s} = t_{l}\tmerge t_{q}
% \hfill i \in I \hfill j \in I / \{i\}
% \end{array}\right\}
% \quad \Rightarrow \quad
% 	\m{init\_s}(\ \env,(\ l_i.\pid p_i[\role A_i]\ )_{i},k\ )
% 		=	\env
% 	\begin{array}{l}
% 		\big[\ \pid p_i,\estate \mapsto \env(\pid p_i).\estate \tmerge
% 				t_{s}\ \big]_{i}
% 		\\
% 		\big[\ \pid p_i,\equeues, \jpath{k.A}_j\jpath{.A}_i( t_{s} ) 
% 		\mapsto \emptyseq\ \big]_{i,j}
% 	\end{array}
% \\\\
% 	\nexists\; \pid p \in \dom(\ D( l )\ )\;\; \mbox{s.t.}\;\; t\; \in \dom( \env
% 	(\pid p ).\equeues )
% 	\quad \Rightarrow \quad 
% 	\m{\fresh queue\_id}(\env, l) = t
% 	\hfill
% 	t \tmerge t' = t \bigtcopy_{x}(\ x, x(t')\ ),\  x \in \m{leaves}(t')
\end{array}
\end{displaymath}
\caption{Choreography Calculus, auxiliary functions on $\env$.}
\label{fig:aux_ops_env}
\end{figure*}


==> figures/chor_global_typing_semantics.tex <==
\begin{figure}
$$
\begin{array}{c}
	\infer[\did{G}{Send}]
	{
		\gcom{\role A}{\role B}{\{\op{o}_i(U_i); G_i\}} 
		\quad \to \quad
		\grecv{\role A}{\role B}
		{\op{o}_j(U_j)};G_j
	}
	{
		\{i,j\} \subseteq I
	}
	\qquad
	\infer[\did{G}{Recv}]
	{
		\grecv{\role A}{\role B}{\op{o}(U)}; G 
		\quad \to \quad
		G
	}
	{\ }
	\\[15pt]
	\infer[\did{G}{Rec}]
	{
		\gengrecDef \quad \to \quad G'
	}
	{
		G[\gengrecDef / \gengrecCall] \to G'
	}
	% \\[5pt]
	% \infer[\did{G}{ACom}]
	% {
	% 	\gcom{\role A}{\role B}{\{\op{o}_i(S_i);G_i\}_{i \in I}}
	% 	\longto
	% 	\gcom{\role A}{\role B}{\op{o}_j(S_j);G_h'}
	% }
	% {
	% 	\begin{array}{c}
	% 		j \in I
	% 		\qquad
	% 		G_j = \gcom{\role C}{\role D}{\{\op{o}_k'(S_k');G_k'\}_{k \in K}}
	% 		\\[.2em]
	% 		\{\role A, \role B \} \cap \{\role C, \role D\} = \{\role A\}
	% 		\qquad
	% 		h \in K	
	% 		\qquad
	% 		G_j \to G_h'
	% 	\end{array}
	% }
	\qquad
	\infer[\did{G}{Swap}]
	{
		G_1 \longto G_1'
	}
	{
		G_1 \swapG G_2
		&
		G_2 \to G_2'
		&
		G_2' \swapG G_1'
	}
\end{array}
$$
\caption{Global types --- Semantics.}
\label{fig:cc_global_types_semantics}
\end{figure}

==> figures/chor_global_typing_semantics_fix.tex <==
\begin{figure}
  {\small
  $$
  \begin{array}c
    \infer[\did{G}{Act}]
    {
      G \quad \to \quad G'
    }{
      (\mu, G') \in \gnext_{\emptyset}(G)
    }
    \qquad
    \infer[\did{G}{Eq}]
    {
      G \quad \to \quad G'
    }
    {
      G \equiv G_1 &
      G_1 \to G_1' &
      G_1' \equiv G'
    }
  \end{array}
  $$
  \hrule
  $$
    G[\gengrecDef'] \quad \equiv \quad G\left[\ G'[\gengrecDef'/\gengrecCall]\ \right]
  $$
  \hrule
  $$
  \begin{array}c    
    \begin{array}{l}
      \gnext_{\mathbb{R}}(\gcom{\role A}{\role B}{\{o_i(U_i);G_i\}})
      =
      \\
      \qquad 
      \mathbb{S} \ \cup \
      \bigcup_{ji}
      \left\{
        \left(
          \mu_j, \gcom{\role A}{\role B}{o_i(U_i);G_{ij}}
        \right)
      \right\}_j
      \quad 
      \begin{array}l
      \mathbb{S} = \bigcup_i
        \left\{
          \left(
              \gcom{\role A}{\role B}{o_i(U_i)}, 
              \grecv{\role A}{\role B}{o_i(U_i);G_i}
          \right)
        \right\} \mbox{ if } \role A \not \in \mathbb{R},
      \\
      \emptyset \mbox{ otherwise}
      \\
      \wedge \ \gnext_{\mathbb{R} \cup \{\role B\}}(G_i) = \left\{(\mu_j,G_
      {ij})\right\}_j
      \end{array}
      \\[2em]
      \gnext_{\mathbb{R}}(\grecv{\role A}{\role B}{o(U);G})
      =
      \begin{array}l
      \mathbb{S}\ \cup\
      \bigcup_j
      \left\{
        \left(
          \mu_j, \grecv{\role A}{\role B}{o(U);G_j}
        \right)
      \right\}_j
      \end{array}
      \quad
      \begin{array}l
      \mathbb{S} = 
      \left\{
        \left(
          \grecv{\role A}{\role B}{o(U)},G
        \right)
      \right\} \mbox{if } \role B \not \in \mathbb{R},
      \\
      \emptyset \mbox{ otherwise}
      \\
      \wedge \ \gnext_{\mathbb{R} \cup \{\role B\}}(G) = 
      \left\{\left(
        \mu_j, G_j
      \right)\right\}_j
      \end{array}
    \end{array}
    \\[4.5em]
    \gnext_{\mathbb{R}}(\gend) \quad = \quad
    \gnext_{\mathbb{R}}(\gengrecDef) \quad = \quad
    \gnext_{\mathbb{R}}(\gengrecCall) \quad = \quad \emptyset
  \end{array}
  $$
  % $$
  %   \begin{array}c      
  %     \grecs(\gcom{\role A}{\role B}{\{o_i(U_i);G_i\}}) = 
  %      \bigcup_i\grecs(G_i)
  %     \qquad
  %     \grecs(\grecv{\role A}{\role B}{o(U)};G) = \grecs(G)
  %     \\[.5em]
  %     \grecs(\gengrecDef) = \{\gengrecDef\} \cup \grecs(G)
  %     \qquad
  %     \grecs(\gengrecCall) = \grecs(\gend) = \emptyset
  %   \end{array}
  % $$
  }
  \caption{Global types --- Semantics.}
  \label{fig:global_types_semantics}
\end{figure}

==> figures/chor_local_typing_semantics.tex <==
\begin{figure}
	\begin{displaymath}
		\begin{array}{c}
			\infer[\did{T}{Act}]
			{
				\pair{k[\role A]}{\alpha.\{o_i(S_i);T_i\}_{i \in I}} \longto 
				\pair{k[\role A]}{T_j}
			}
			{
				j \in I
			}
			\\\\
			\infer[\did{T}{Rec}]
			{
				\pair{k[\role A]}{\genlrecDef} \longto \pair{k[\role A]}{T'}
			}
			{
				\pair{k[\role A]}{T[ \ \genlrecDef / \genlrecCall \ ]} \to 
				\pair{k[\role A]}{T'}
			}
			\\\\
			\infer[\did{T}{ASend}]
			{
				\pair{k[\role A]}{\lsend{B}{\{o_i(S_i);T_i\}_{i \in I}}} \longto
				\pair{k[\role A]}{\lsend{B}{o_j(S_j);T'_{h}}}				
			}
			{
				j \in I
				&
				T_j = \alpha.\{o_{k}'(S_{k}');T_{k}'\}_{k \in K}
				&
				\role B \neq \m{role}(\alpha)
				&
				h \in K
			}
			\\\\
			\infer[\did{T}{Conc}]
			{
				\Gamma_1, \Gamma_2 \longto \Gamma_1, \Gamma_2'
			}
			{
				\Gamma_2 = \pair{k[\role A]}{\alpha.\{o_i(S_i);T_i\}_{i}}
				&
				\Gamma_2 \to \Gamma_2'
				&
				k[\m{role}(\alpha)] \not \in \Gamma_1
			}
			\\\\
			\m{nxtSbj}(T) = \begin{cases}
				\m{nxtSbj}(T'[\genlrecDef' / \genlrecCall]) 
					& \mbox{if } T = \genlrecDef'
				\\
				\m{role}(\alpha) & \mbox{if } T = \alpha.\{o_i(S_i);T_i\}_{i}
			\end{cases}
			\\\\
			\alert{used by $\did{T}{Conc}$} \quad
			
			$\Gamma_1, (\Gamma_2, \Gamma_3 ) \equiv (\Gamma_1, \Gamma_2), \Gamma_3$

			$\Gamma_1, \Gamma_2 \equiv \Gamma_2, \Gamma_1$
			\\\\
		\end{array}
	\end{displaymath}
	\caption{Local types, Semantics and Structural Equivalence}
	\label{fig:cc_local_types_semantics}
\end{figure}

==> figures/chor_seff.tex <==
\begin{figure*}
% \begin{subfigure}{\textwidth}
\begin{displaymath}
\begin{array}{l}
%
\did{\env}{Send}
\quad
\env \seff \com{k}{\pid p[\role A].e}{\role B.o}
	=
	\m{upd\_que}(\env,\pid q, t_c, \til m::(o,t_m) )
	% \env[\pid q,\equeues, t_c \mapsto \til m,\ (o,t_m)]
\quad\mbox{if}\quad
{\arraycolsep=0pt\def\arraystretch{1.2}
\left\{\begin{array}{c}
	l = \troot{\jpath{k.B.l} (\env(\pid p).\estate)}
	\qquad
	t_c = \jpath{k.A.B}(\env(\pid p).\estate)
	\\
	\pid q \in \env(l)
	\quad
	\env(\pid q).\equeues(t_c) = \til m
	\quad
	t_m = \evalfn(e,\ \env(\pid p).\estate)
\end{array}\right.}
\\[12pt]
\did{\env}{Recv}\quad
	\env \seff \com{k}{\role A}{\pid q[\role B].o(x)}
	=
	\m{upd\_que}\Big(
		\m{up\_st}\big(\ \env, \pid q, \env(\pid q).\estate \tcopy{x}
		{t_m}\ \big),\pid q,t_c,\til m	\Big)
\hfill\mbox{if}\hfill
{\arraycolsep=0pt\def\arraystretch{1.2}
\left\{\begin{array}{l}
	% \delta = \com{k}{\role A}{\pid q[\role B].o(x)}\qquad
	t_c = \jpath{k.A.B}(\env(\pid q).\estate)
	\\
	\env(\pid q).\equeues(t_c) = (o,t_m)::\ \til m
\end{array}\right.
}
\end{array}
\end{displaymath}
\caption{Choreography calculus, effects $\env \seff \delta$.}
\label{fig:cc_effects}
\end{figure*}

==> figures/chor_semantics.tex <==
\begin{figure*}
{\footnotesize
\begin{displaymath}
\hspace{-5pt}\begin{array}{c}
\infer[\did{C}{Send}]
{
	\env,\ \eta; C
	\quad \to\quad
	\env',\ C
}{
	\eta = \gensend
	&
	\renv{\env}{\eta}{\env'}
}
\quad
\infer[\did{C}{Recv}]
{
	\env,\ \genbranchI
	\quad \to\quad
	\env',\ C_j
}{
	j \in I
	&
	\renv{\env}{\com{k}{\role A}{\pid q[\role B].o_j(x_j)}}{\env'}
}
\\[5pt]
\infer[\did{C}{Com}]
{
	\env,\ \eta; C
	\to
	\env',\ \genrecv;C
}{
	\eta = \gencom
	% \\[1pt]
	&
	\renv{\env}{\gensend}{\env'}
}
% \quad
% \infer[\did{C}{Cond}]
% {
% 	\env,\ \cond{\pid p.e}{C_1}{C_2}
% 	\quad\to\quad
% 	\env,\ C_i
% }
% {
% 	i = 1 \text{ if } \evalfn(e, \env(\pid p).\estate) = \text{ true, }
% 	i = 2 \text{ otherwise}
% }
% \\[5pt]
% \infer[\did{C}{Ctx}]
% {
% 	\env, \recDef{X}{C_2}{C_1} \to
% 	\env^\prime, \recDef{X}{C_2}{C^\prime_1}
% }
% {
% 	\env, C_1 \to \env^\prime, C^\prime_1
% }
\quad
\infer[\did{C}{Eq}]
{
	\env, C_1 \to \env^\prime, C_2
}
{
	\ctx{R} \in \{\,\equiv\,,\,\swapC\,\}
	&
	C_1 \,\ctx{R}\, C^\prime_1
	\\[1pt]
	\env, C^\prime_1 \to \env^\prime, C^\prime_2
	&
	C^\prime_2 \,\ctx{R}\, C_2
}
\\[5pt]
\infer[\did{C}{Start}]
{
	\env,\ \genstart; C
	\to
	\env',\
	C[k'/k][\pids r/\pids q] 
}
{
	\env\fresh{k',\pids r}
% 	&
% 	\fresh{k'}
% 	&
% 	\pid p \in \env(l)
%	&
%	\delta = \deltastart{k'}{l.\prc pA, \wtil{l.\prc rB}}
	% \eta[k'/k][\pids r/\pids q]
	&
	\renv{\env}{\start{k'}{\prc pA}{\wtil{l.\prc rB}}}{\env'}
}
% \infer[\did{C}{Par}]
% {
% 	\env, C_1\pp C_2
% 	\to
% 	\env', C'_1 \pp C_2
% }
% {
% 	\env, C_1
% 	\to
% 	\env', C'_1
% }
% \quad
% \\[5pt]
% \infer[\did{C}{PStart}]
% {
% 	\begin{array}{c}
% 	\env,
% 	\req{k}{\pid p[\role A]}
% 	{\wtil{l.\role B}}; C
% 	\pp
% 	\prod_i
% 	\big(
% 	\genacci; C_i
% 	\big)
% 	\to
% 	\\ \qquad
% 	\env',\ 
% 	C[k'/k] \pp \prod_i\big(\ C_i[k'/k][\pids r_i /\pids q_i] \ \big)
% 	\pp
% 	\prod_i
% 	\big(
% 	\genacci; C_i
% 	\big)
% 	\end{array}
% }
% {
% 	\begin{array}c
% 	i \in \{1,\dots,n\}
% 	\quad
% 	\fresh{k'}
% 	\quad
% 	\{ \wtil{l.\role B} \} = \biguplus_i \{\wtil{l_i.\role B_i}\}
% 	\quad
% 	\fresh{\pids r}
% 	\\[2pt]
% 	\{\pids r\} = \bigcup_i \{ \pids r_i \}
% 	\quad
% 	\pid p \in \env(l)
% 	\quad
% 	\delta = \deltastart{k'}{l.\pid p[\role A],\wtil{l_1.\pid r_1[\role
% 	B_1]},\dots,\wtil{l_n.\pid r_n[\role B_n]}}
% 	\quad
% 	\renv{\env}{\delta}{\env'}
% 	\end{array}
% }
\end{array}
\end{displaymath}}
\vspace{-1em}
\caption{Frontend Choreographies, semantics (selected).}
\label{fig:cc_semantics}
\end{figure*}

==> figures/chor_semantics_inline.tex <==
\begin{figure*}
{\footnotesize
\setlength{\arraycolsep}{3pt}
$$
\hspace{-5pt}\begin{array}{llll}
\did{C}{Send}
&
\eta = \gensend
\ \wedge \
\renv{\env}{\eta}{\env'}
& \Rightarrow &
\env,\ \eta; C
\to
\env',\ C
\\[3pt]
\did{C}{Recv}
&
j \in I
\ \wedge \
\renv{\env}{\com{k}{\role A}{\pid q[\role B].o_j(x_j)}}{\env'}
& \Rightarrow &
\env,\ \genbranchI
\to
\env',\ C_j
\\[3pt]
\did{C}{Com}
&
\hspace{-5pt}\begin{array}l
	\eta = \gencom
	\\
	\wedge \
	\renv{\env}{\gensend}{\env'}
\end{array}
& \Rightarrow &
\env,\ \eta; C
\to
\env',\ \genrecv;C
\\[8pt]
\did{C}{Eq}
&
\hspace{-5pt}\begin{array}l
\ctx{R} \in \{\,\equiv\,,\,\swapC\,\}
\ \wedge \
C_1 \,\ctx{R}\, C^\prime_1
\ \wedge \
\\
\env, C^\prime_1 \to \env^\prime, C^\prime_2
\ \wedge \
C^\prime_2 \,\ctx{R}\, C_2	
\end{array}
& \Rightarrow &
\env, C_1 \to \env^\prime, C_2
\\[8pt]
\did{C}{Start}
&
\env\fresh{k',\pids r}
\ \wedge \
\renv{\env}{\start{k'}{\prc pA}{\wtil{l.\prc rB}}}{\env'}
& \Rightarrow &
\env,\ \genstart; C
\to
\env',\	C[k'/k][\pids r/\pids q] 
\end{array}
$$}
\vspace{-1em}
\caption{Frontend Choreographies, semantics (selected).}
\label{fig:cc_semantics}
\end{figure*}

==> figures/chor_semantics_sos.tex <==
\begin{figure*}
{\footnotesize
\begin{displaymath}
\hspace{-5pt}\begin{array}{c}
\infer[\did{C}{Send}]
{
	\env,\ \eta; C
	\quad \to\quad
	\env',\ C
}{
	\eta = \gensend
	&
	\renv{\env}{\eta}{\env'}
}
\quad
\infer[\did{C}{Recv}]
{
	\env,\ \genbranchI
	\quad \to\quad
	\env',\ C_j
}{
	j \in I
	&
	\renv{\env}{\com{k}{\role A}{\pid q[\role B].o_j(x_j)}}{\env'}
}
\\[5pt]
\infer[\did{C}{Com}]
{
	\env,\ \eta; C
	\to
	\env',\ \genrecv;C
}{
	\eta = \gencom
	% \\[1pt]
	&
	\renv{\env}{\gensend}{\env'}
}
% \quad
% \infer[\did{C}{Cond}]
% {
% 	\env,\ \cond{\pid p.e}{C_1}{C_2}
% 	\quad\to\quad
% 	\env,\ C_i
% }
% {
% 	i = 1 \text{ if } \evalfn(e, \env(\pid p).\estate) = \text{ true, }
% 	i = 2 \text{ otherwise}
% }
% \\[5pt]
% \infer[\did{C}{Ctx}]
% {
% 	\env, \recDef{X}{C_2}{C_1} \to
% 	\env^\prime, \recDef{X}{C_2}{C^\prime_1}
% }
% {
% 	\env, C_1 \to \env^\prime, C^\prime_1
% }
\quad
\infer[\did{C}{Eq}]
{
	\env, C_1 \to \env^\prime, C_2
}
{
	\ctx{R} \in \{\,\equiv\,,\,\swapC\,\}
	&
	C_1 \,\ctx{R}\, C^\prime_1
	\\[1pt]
	\env, C^\prime_1 \to \env^\prime, C^\prime_2
	&
	C^\prime_2 \,\ctx{R}\, C_2
}
\\[5pt]
\infer[\did{C}{Start}]
{
	\env,\ \genstart; C
	\to
	\env',\
	C[k'/k][\pids r/\pids q] 
}
{
	\env\fresh{k',\pids r}
% 	&
% 	\fresh{k'}
% 	&
% 	\pid p \in \env(l)
	&
	\delta = \deltastart{k'}{l.\prc pA, \wtil{l.\prc rB}}
	% \eta[k'/k][\pids r/\pids q]
	&
	\renv{\env}{\delta}{\env'}
}
% \infer[\did{C}{Par}]
% {
% 	\env, C_1\pp C_2
% 	\to
% 	\env', C'_1 \pp C_2
% }
% {
% 	\env, C_1
% 	\to
% 	\env', C'_1
% }
% \quad
% \\[5pt]
% \infer[\did{C}{PStart}]
% {
% 	\begin{array}{c}
% 	\env,
% 	\req{k}{\pid p[\role A]}
% 	{\wtil{l.\role B}}; C
% 	\pp
% 	\prod_i
% 	\big(
% 	\genacci; C_i
% 	\big)
% 	\to
% 	\\ \qquad
% 	\env',\ 
% 	C[k'/k] \pp \prod_i\big(\ C_i[k'/k][\pids r_i /\pids q_i] \ \big)
% 	\pp
% 	\prod_i
% 	\big(
% 	\genacci; C_i
% 	\big)
% 	\end{array}
% }
% {
% 	\begin{array}c
% 	i \in \{1,\dots,n\}
% 	\quad
% 	\fresh{k'}
% 	\quad
% 	\{ \wtil{l.\role B} \} = \biguplus_i \{\wtil{l_i.\role B_i}\}
% 	\quad
% 	\fresh{\pids r}
% 	\\[2pt]
% 	\{\pids r\} = \bigcup_i \{ \pids r_i \}
% 	\quad
% 	\pid p \in \env(l)
% 	\quad
% 	\delta = \deltastart{k'}{l.\pid p[\role A],\wtil{l_1.\pid r_1[\role
% 	B_1]},\dots,\wtil{l_n.\pid r_n[\role B_n]}}
% 	\quad
% 	\renv{\env}{\delta}{\env'}
% 	\end{array}
% }
\end{array}
\end{displaymath}}
\vspace{-1em}
\caption{Applied Choreographies, semantics (selected).}
\label{fig:cc_semantics_sos}
\end{figure*}

==> figures/chor_typing_rules.tex <==
\begin{figure*}
{\footnotesize
\begin{displaymath}
\hspace{-5pt}\begin{array}{c}
% \infer[\did{T}{Cond}]
% {\Gamma \hlseq{\gencond}}
% {
% 	\Gamma \seq \pair{\pid p.e}{\tbool}
% 	&
% 	\Gamma \hlseq{C_1}
% 	&
% 	\Gamma \hlseq{C_2}
% }
% \qquad
\infer[\did{T}{Com}]
{
	\Gamma, 
	\pair{k[\role A]}{\genlsendB},
	\pair{k[\role B]}{\genlrecvPrime}
	\hlseq{
		\com{k}{\pid p[\role A].e}{\pid q[\role B].o_j(x)};C}
}
{
	j \in I
	&
	% \Gamma \seq{\com{k}{\pid p[\role A]}{\pid q[\role B]}}
	\Gamma \seq \pair{\pid p}{k[\role A]},\pair{\pid q}{k[\role B]}
	&
	\Gamma \seq \pair{\pid p.e}{U_j}
	&
	\Gamma, \pair{\pid q.x}{U_j}, 
		\pair{k[\role A]}{T_j}, 
		\pair{k[\role B]}{T'_j}
		\hlseq{C}
}
% \\[8pt]
% \infer[\did{T}{Send}]
% {
% 	\Gamma, 
% 	\pair{k[\role A]}{\genlsendB}
% 	\hlseq{\gensendj; C}
% }
% {
% 	j \in I
% 	&
% 	\Gamma \seq \pair{\pid p}{k[\role A]}
% 	% &
% 	% \Gamma \seq{\com{k}{\pid p[\role A]}{\role B}}
% 	&
% 	\Gamma \seq \pair{\pid p.e}{U_j}
% 	&
% 	\Gamma, \pair{k[\role A]}{T_j} \hlseq{C }
% }
% \\[8pt]
% \infer[\did{T}{Recv}]
% {
% 	\Gamma, 
% 		\pair{k[\role B]}{\lrecv{A}{\{o_i(U_i);T_i\}_{i \in I}}}
% 	\hlseq{\genbranchIJ}
% }
% {
% 	% \Gamma \seq{\com{k}{\role A}{\pid q[\role B]}}
% 	\Gamma \seq \pair{\pid q}{k[\role B]}
% 	&
% 	\forall j\in I. \ \Gamma, \pair{\pid q.x_j}{U_j}, 
% 	\pair{k[\role B]}{T_j}
% 	\hlseq{C_j}
% }
\\[5pt]
\infer[\did{T}{Start}]
{
	\Gamma, \til l:\initg{G}{\role A}{\til{\role B}}{\til{\role B}}
	\hlseq{\genstart ; C}
}
{
	\Gamma,\til l:\initg{G}{\role A}{\til{\role B}}{\til{\role
	B}},
	% \wtil{\pid q@l},
	\init(\ \wtil{\prc rC},k,G\ )
	\hlseq {C}
	&
	\wtil{\prc rC} = \prc pA, \wtil{\prc qB}
	&
	\til{\pid q} \not \in \Gamma
}
\qquad
\infer[\did{T}{Par}]
{\Gamma_1 \circ \Gamma_2 \hlseq {C_1 \pp C_2}}
{
	% \pn(\Gamma_1) \cap \pn(\Gamma_2) = \emptyset
	% &
	\Gamma_i \hlseq {C_i}
	&
	\Gamma_2 \hlseq {C_2}
}
% \quad
% \infer[\did{T}{Req}]
% {
% 	\Gamma \hlseq{\genreq ; C}
% }
% {
% 	\Gamma, \pid p:k[\role A], k[\role A]:\epp{G}{\role A} \hlseq{C}
% 	&
% 	\Gamma \seq \til l:\initg{G}{\role A}{\til{\role B}}{\emptyset}
% }
% \\[5pt]
% \infer[\did{T}{Call}]
% {
% 	\Gamma, \Gamma'', \pair{X\carr{\pids p}}{\Gamma'} \hlseq{X\carr{\pids p}}
% }
% {
% 	\m{end}(\Gamma)
% 	&
% 	\Gamma'' \subseteq \Gamma'
% }
% \quad
% \infer[\did{T}{Acc}]
% {
% 	\Gamma, \til l':\initg{G}{\role A}{\til{\role B}}{\til{\role C}} \hlseq{
% 		\genaccC ; C	}
% }
% {
% 	\til l \subseteq \til l'
% 	&
% 	\Gamma, \til l':\initg{G}{\role A}{\til{\role B}}{\emptyset},
% 	% \wtil{\pid q@l},
% 	\init(\ \wtil{\pid q[\role C]},k,G\) \hlseq{C}
% }
% \hfill
% \infer[\did{T}{End}]
% {\Gamma \hlseq{\inact}}
% {
% \m{end}(\Gamma)
% }
% \hfill
% \infer[\did{T}{Def}]
% {
% 	\Gamma \hlseq{\recDef{X\carr{\pids p}}{C'}{C}}
% }
% {
% 	\Gamma,\pair{X}{\Gamma'} \hlseq{C}
% 	&
% 	\Gamma', \pair{X}{\Gamma'} \hlseq C'
% 	&
% 	\Gamma' |_{\locs} \subseteq \Gamma
% 	&
% 	\pids p = \pn(C')
% }
\end{array}
\end{displaymath}}
\caption{Choreography Calculus, Typing Rules (selected).}
\label{fig:typing_rules}
\end{figure*}
% \begin{figure*}
% \begin{displaymath}
% \begin{array}{c}
% \infer[\did{O}{Com}]
% {
% 	\Gamma \seq \com{k}{\pid p[\role A]}{\pid q[\role B]}
% }
% {
% 	\Gamma \seq \pair{\pid p}{k[\role A]}
% 	&
% 	\Gamma \seq \pair{\pid q}{k[\role B]}
% }
% \qquad
% \infer[\did{O}{Send}]
% {
% 	\Gamma \seq \com{k}{\pid p[\role A]}{\role B}
% }
% {
% 	\Gamma \seq \pair{\pid p}{k[\role A]}
% }
% \qquad
% \infer[\did{O}{Recv}]
% {
% 	\Gamma \seq \com{k}{\role A}{\pid q[\role B]}
% }
% {
% 	\Gamma \seq \pair{\pid q}{k[\role B]}
% }
% \end{array}
% \end{displaymath}
% \caption{Choreography Calculus - Ownership Rules}
% \label{fig:ownership_rules}
% \end{figure*}

==> figures/chor_typing_swap.tex <==
\begin{figure}
{$$
\begin{array}c
	\infer[\did{GS}{ComCom}]{
	\begin{array}{l}
		\gcom{\role A}{\role B}{\{\op{o}_i(U_i);\gcom{\role C}{\role
			D}{\{\op{o}_j'(U_j');G_{ij}\}_{j \in J}}\}_{i \in I}}
		\\\hspace{.3\textwidth}
		\swapG \quad
		\gcom{\role C}{\role D}{\{\op{o}_j'(U_j');\gcom{\role A}{\role
			B}{\{\op{o}_i(U_i);G_{ij}\}_{i \in I}}\}_{j \in J}}
	\end{array}
}
{	\{\role A, \role B\} \cap \{\role C, \role D\} = \emptyset }
\\[20pt]
\infer[\did{GS}{ComRecv}]{
	\begin{array}c
	\gcom{\role A}{\role B}{\{\op{o}_i(U_i);\grecv{\role C}{\role D}{\op{o}(U)};G_i\}}
	\quad \swapG \quad
	\grecv{\role C}{\role D}{\op{o}(U)};\gcom{\role A}{\role B}{\{\op{o}_i(U_i);G_i\}}
	\end{array}
}
{	
	\{\role A, \role B\}  \cap \{\role D\} = \emptyset
 }
\\[15pt]
\infer[\did{GS}{RecvRecv}]{
	\begin{array}c
	\grecv{\role A}{\role B}{\op{o}(U)};\grecv{\role C}{\role D}{\op{o}'(U)};G
	\quad \swapG \quad
	\grecv{\role C}{\role D}{\op{o}'(U)};\grecv{\role A}{\role B}{\op{o}(U)};G
	\end{array}
}{
	\role B \neq \role D
}
\end{array}
$$}
	\caption{Global types --- Swap Relation $\swapG$.}
	\label{fig:cc_global_types_swap}
\end{figure}

==> figures/choreography_example.tex <==
\begin{figure*}
\begin{subfigure}{.5\textwidth}
  {\scriptsize
  \begin{displaymath}
	\ResetLN
	{\setlength\arraycolsep{2pt}
	\begin{array}l
	C_{c} = \\ \quad\left\{
	\begin{array}{rl}
		\LN & \req{k_d}{\prc cC}{l_{\role A}.\role A,
			l_{\role{DM}}.\role{DM},l_{\role L}.\role L};
		\\
		\LN & \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get};
		\\[.3em]
		\LN & \recDef{\text{STORE}}{
		\\
		\LN &	\quad \com{k_d}{\role{DM}}{\prc cC.\{
		\\
		\LN & \qquad pkt( \jpath{bb} );
		\\
		\LN & \quad\qquad \com{k_s}{\prc cU.\jpath{bb}}{
						\prc fF.append(\jpath{data})};
		\\
		\LN & \quad\qquad \recCall{\text{STORE}}\; ,
		\\
		\LN & \qquad chksum( \jpath{cs} );
		\\
		\LN & \quad\qquad \com{k_s}{\prc cU.\jpath{cs}}{
						\prc fF.check(\jpath{cs})};
		\\
		\LN & \quad\qquad \cond{\pid f.\m{check}( \jpath{fname}, \jpath{cs} )}{
		\\
		\LN & \qquad\qquad \com{k_s}{\prc fF}{\prc cU.saved}
		\\
		\LN & \quad\qquad }{
		\\
		\LN & \qquad\qquad \com{k_s}{\prc fF}{\prc cU.discarded}
		\\
		\LN & \quad }\}}
		% \\
		% \LN & \quad \}}
		\\
		\LN & }{
		\\
		\LN & \com{k_d}{\role A}{\prc cC.\{
		\\
		\LN & \quad ok;
		\\
		\LN & \qquad \start{k_s}{\prc cU}{l_{\role C}.\prc fF};
		\\
		\LN & \qquad \com{k_s}{\prc cU.\m{name}()}{\prc fF.create(\jpath{fname})};
		\\
		\LN & \qquad \recCall{\text{STORE}}\; ,
		\\
		\LN & \quad ko \ \}}
		% \\
		% \LN & \quad \}}
	}
	\end{array}
	\right.
	\end{array}
	}
  \end{displaymath}}
	% \caption{Client partial choreography}
 %  \label{fig:choreography_example_client}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\ResetLN
  {\scriptsize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\begin{array}l
	C_{s} = \\	
	\quad  \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role A}.\prc aA,
		l_{\role{DM}}.\prc {dm}{DM},l_{\role L}.\prc lL};
	\\
	\LN & \com{k_d}{\role C}{\prc aA.get(\jpath{req})};
	\\
	\LN & \cond{\pid a.isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc {dm}{DM}.ok(\jpath{rsc})};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ok};
	\\
	\LN & \quad \com{k_d}{\prc {dm}{DM}.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
	\\[.4em]
	\LN & \quad \recDef{\text{TRANSFER}}{
	\\
	\LN &
		\qquad\cond{ \pid {dm}.\m{more}(\jpath{rsc})}{
		\\
		\LN & \quad\qquad \com{k_d}{\prc {dm}{DM}.\m{next}(\jpath{rsc})}{\role C.pkt};
		\\
		\LN & \quad\qquad \recCall{\text{TRANSFER}} 
		\\ \LN &\qquad }{
		\\
		\LN & \quad\qquad \com{k_d}{\prc {dm}{DM}.\m{chksum}(\jpath{rsc})}{\role C.chksum}
		\\ \LN & \qquad}
	\\ \LN & \quad}{
	\\[.2em] \LN & \;\quad \recCall{\text{TRANSFER}}
	}
	\\ \LN & }{
	\\ 
		\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc {dm}{DM}.ko(\jpath{rsc})};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ko};
	\\
	\LN & \quad \com{k_d}{\prc {dm}{DM}.\m{logko}(\jpath{rsc})}{\prc lL.log(\jpath{log})}
	\\ \LN &
	}
	\end{array}
	\right.
	\end{array}
	}
  \end{displaymath}}
\end{subfigure}
  \caption{Choreography Example}
  \label{fig:choreography_example}
\end{figure*}

==> figures/compilation_example.tex <==
\begin{figure*}
%
%	ENCODING --- C
%
\begin{subfigure}{\textwidth}
	{\scriptsize
	\begin{displaymath}
		\overbrace{
		\jsrv{\genenc{\epp{C}{\pid f}}, \jprc{\genenc{\epp{C}{\pid c}}}{\env(\pid c).\estate}
		{\env( \pid c ).\equeues}}{l_\role C}}^{S_c}
		\; \pp \;
		\overbrace{
		\jsrv{\ \genenc{\epp{C}{\pid a}}, \inact}{l_\role A}}^{S_a}
		\; \pp \;
		\overbrace{
		\jsrv{\ \genenc{\epp{C}{\pid {dm}}}, \inact}{l_\role {DM}}}^{S_{dm}}
		\; \pp \;
		\overbrace{
		\jsrv{\ \genenc{\epp{C}{\pid l}}, \inact}{l_\role L}}^{S_l}
	\end{displaymath}}
	% \caption{Parallel composition of the compiled services of
		% $\genenc{\env,\epp{C}{}}$}
  % \label{fig:example_compilation_services}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\ResetLN
  {\scriptsize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\genenc{\epp{C}{\pid c}} =
	\left\{
	\hspace{-3pt}\begin{array}{rl}
	\LN & \jpath{kd.C.l} = l_{\role C};
	\\
	\LN & \jpath{kd.A.l} = l_{\role A};
	\\
	\LN & \jpath{kd.DM.l} = l_{\role {DM}};
	\\
	\LN & \jpath{kd.L.l} = l_{\role L};
	\\
	% \LN & \ldots
	% \\
	% \LN & \jpath{kd.A.C} = \new;
	% \\
	\LN & \cq{\jpath{kd.A.C}};
	\\
	\LN & \notify{?}{\jpath{kd.A.l}}{\jpath{kd}};
	\\
	\LN & \oneway{sync}{\jpath{kd}} \qfrom{\jpath{kd.A.C}};
	\\
	% \LN & \jpath{kd.S.C} = \new;
	% \\
	% \LN & \cq{\jpath{kd.S.C}};
	\LN & \ldots
	\\
	% \LN & \notify{?}{\jpath{kd.S.l}}{\jpath{kd}};
	\LN & \ldots
	\\
	\LN & \notify{start}{\jpath{kd.A.l}}{\jpath{kd}} \qto{\jpath{kd.C.A}};
	\\
	\LN & \notify{start}{\jpath{kd.S.l}}{\jpath{kd}} \qto{\jpath{kd.C.S}};
	\\
	\LN & \notify{start}{\jpath{kd.C.l}}{\jpath{kd}} \qto{\jpath{kd.C.L}};
	\\
	\LN & \notify{get}{\jpath{kd.A.l}}{\m{mkReq()}} \qto{\jpath{kd.C.A}};
	\\
	\LN & \ldots
	\end{array}
	\right.
	% \\\\	
	% \jsrv{\inact, \jprc{\enc{\epp{C_{c}}{\pid c}}_{\pid c}}
	% 	{\env(\pid a).\estate}{\env(\pid a).\equeues}}{l_{\role C}}
	}
  \end{displaymath}}
\end{subfigure}
%
%	ENCODING --- A
%
\begin{subfigure}{.5\textwidth}
	\ResetLN
  {\scriptsize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\genenc{\epp{C}{\pid a}} =
	\left\{
	\hspace{-3pt}\begin{array}{rl}
	\LN & \oneway{!}{\jpath{kd}};
	% \\
	% \LN & \jpath{kd.C.A} = \new;
	\\
	\LN & \cq{\jpath{kd.C.A}};
	% \\
	% \LN & \jpath{kd.S.A} = \new;
	\\
	\LN & \cq{\jpath{kd.S.A}};
	% \\
	% \LN & \jpath{kd.L.A} = \new;
	\\
	\LN & \cq{\jpath{kd.L.A}};
	\\
	\LN & \notify{sync}{\jpath{kd.C.l}}{\jpath{kd}} \qto{\jpath{kd.A.C}};
	\\
	\LN & \oneway{start}{\jpath{kd}} \qfrom{\jpath{kd.C.A}};
	\\
	\LN & \oneway{get}{\jpath{req}} \qfrom{\jpath{kd.C.A}};
	\\
	\LN & \cond{isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \notify{ok}{\jpath{kd.S.l}}{\jpath{req.rsc}} 
		\qto{\jpath{kd.A.S}};
	\\
	\LN & \quad \notify{ok}{\jpath{kd.C.l}}{} 
		\qto{\jpath{kd.A.C}}  
	\\ \LN & }{
	\\ 
	\LN & \quad \notify{ko}{\jpath{kd.S.l}}{\jpath{req.rsc}} 
		\qto{\jpath{kd.A.S}};
	\\
	\LN & \quad \notify{ko}{\jpath{kd.C.l}}{} 
		\qto{\jpath{kd.A.C}}  
	\\ \LN &
	}
	\end{array}
	\right.
	% \\\\	
	% \jsrv{\enc{\epp{C_{s}}{\pid a}}_{l_{\role A}} ,\inact}{l_{\role A}}
	}
  \end{displaymath}}
\end{subfigure}

\vspace{-10pt}

%
% ENCODING --- L
%
\begin{subfigure}{\textwidth}
	\ResetLN
  {\scriptsize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\genenc{\epp{C}{\pid l}} =
	\left\{
	\hspace{-2pt}\begin{array}{l}
	\LN \hspace{2pt} \oneway{!}{\jpath{kd}};
	% \\
	% \LN & \jpath{kd.C.L}=\new;
	\LN \hspace{2pt} \cq{\jpath{kd.C.L}};
	% \\
	% \LN & \jpath{kd.A.L}=\new;
	\LN \hspace{2pt} \cq{\jpath{kd.A.L}};
	% \\
	% \LN & \jpath{kd.S.L}=\new;	
	\LN \hspace{2pt} \cq{\jpath{kd.S.L}};
	\LN \hspace{2pt} \notify{sync}{\jpath{k.C.l}}{\jpath{kd}} \qto{\jpath{kd.L.C}};
	\\
	\LN \hspace{2pt} \oneway{start}{\jpath{kd}} \qfrom{\jpath{kd.C.L}};
	\LN \hspace{2pt} \oneway{log}{\jpath{log}} \qfrom{\jpath{kd.S.L}}
	% \\\\
	% \jsrv{\enc{\epp{C_{s}}{\pid l}}_{l_{\role L}} ,\inact}{l_{\role L}}
	\end{array}\right.
	}
  \end{displaymath}}
\end{subfigure}
	\caption{Compilation of $C = C_c \pp C_s$, behaviours of $\pid c$
	(excepts), $\pid {a}$, and $\pid l$.}
  \label{fig:example_compilation}
\end{figure*}

==> figures/eFC_semantics.tex <==
\begin{figure*}
{\footnotesize
\begin{displaymath}
\hspace{-5pt}\begin{array}{c}
\infer[\did{eFC}{Send}]
{
	\env,\ \eta; C
	\quad \to\quad
	\env',\ C
}{
	\eta = \gensend
	&
	\renv{\env}{\eta}{\env'}
}
\quad
\infer[\did{eFC}{Recv}]
{
	\env,\ \genbranchI
	\quad \to\quad
	\env',\ C_j
}{
	j \in I
	&
	\renv{\env}{\com{k}{\role A}{\pid q[\role B].o_j(x_j)}}{\env'}
}
\\[5pt]
% \infer[\did{C}{Cond}]
% {
% 	\env,\ \cond{\pid p.e}{C_1}{C_2}
% 	\quad\to\quad
% 	\env,\ C_i
% }
% {
% 	i = 1 \text{ if } \evalfn(e, \env(\pid p).\estate) = \text{ true, }
% 	i = 2 \text{ otherwise}
% }
% \\[5pt]
% \infer[\did{C}{Ctx}]
% {
% 	\env, \recDef{X}{C_2}{C_1} \to
% 	\env^\prime, \recDef{X}{C_2}{C^\prime_1}
% }
% {
% 	\env, C_1 \to \env^\prime, C^\prime_1
% }
% \\[5pt]
% \infer[\did{C}{Eq}]
% {
% 	\env, C_1 \to \env^\prime, C_2
% }
% {
% 	\ctx{R} \in \{\,\equiv\,,\,\swapC\,\}
% 	&
% 	C_1 \,\ctx{R}\, C^\prime_1
% 	&
% 	\env, C^\prime_1 \to \env^\prime, C^\prime_2
% 	&
% 	C^\prime_2 \,\ctx{R}\, C_2
% }
% \\[5pt]
% \qquad
% \infer[\did{eFC}{Par}]
% {
% 	\env, C_1\pp C_2
% 	\to
% 	\env', C'_1 \pp C_2
% }
% {
% 	\env, C_1
% 	\to
% 	\env', C'_1
% }
% \quad
% \\[5pt]
\infer[\did{eFC}{Start}]
{
	\begin{array}{l}
	\env,
	\req{k}{\pid p[\role A]}
	{\wtil{l.\role B}}; C
	\pp
	\prod_i
	\big(
	\genacci; C_i
	\big)
	\to
	\\ \hspace{100pt}
	\env',\ 
	C[k'/k] \pp \prod_i\big(\ C_i[k'/k][\pids r_i /\pids q_i] \ \big)
	\pp
	\prod_i
	\big(
	\genacci; C_i
	\big)
	\end{array}
}
{
	\begin{array}c
	i \in \{1,\dots,n\}
	\quad
	\env\fresh{k',\pids r}
	\quad
	\{ \wtil{l.\role B} \} = \biguplus_i \{\wtil{l_i.\role B_i}\}
	% \quad
	% \fresh{\pids r}
	\\[2pt]
	\{\pids r\} = \bigcup_i \{ \pids r_i \}
	\quad
	\pid p \in \env(l)
	\quad
	\delta = \deltastart{k'}{l.\pid p[\role A],\wtil{l_1.\pid r_1[\role
	B_1]},\dots,\wtil{l_n.\pid r_n[\role B_n]}}
	\quad
	\renv{\env}{\delta}{\env'}
	\end{array}
}
\end{array}
\end{displaymath}}
\vspace{-1em}
\caption{Frontend Endpoint Calculus, semantics (selected).}
\label{fig:eFC_semantics}
\end{figure*}

==> figures/eFC_syntax.tex <==
\begin{figure}
{\arraycolsep=1pt\def\arraystretch{1.3} \small
$$
\begin{array}l	
\begin{array}{rll}
C \gram &\; \gensend							\; 								& \prid{send}	
	\\
	\Div &\; \genbranchI					\;								& \prid{recv}
	\\
	\Div &\; \cond{\pid p.e}{C_1}{C_2} 							& \prid{cond}
\end{array}
\quad
\begin{array}{rll}
	\Div \quad &\; \genacc ; C					\;								& \prid{acc}
	\\
	\Div \quad &\; \genreq							\;								& \prid{req}
	\\
	\Div \quad &\; \recDef{X}{C^\prime}{C}	& \prid{def}
\end{array}
\quad 
\begin{array}{rll}
	\Div \quad & \; C_1 \pp C_2 				\;								& \prid{par}
	\\
	\Div \quad	&\; \inact																	& \prid{inact}
	\\
	\Div \quad	& \; \recCall{X}													& \prid{call}
\end{array}
\end{array}
$$
}
\vspace{-1em}
\caption{Frontend Endpoint Choreographies, syntax.}
\label{fig:eFC_syntax}
\end{figure}


==> figures/encoding_full.tex <==
\begin{figure*}
{\footnotesize	
% \begin{minipage}{.45\textwidth}
	\begin{displaymath}
	{\setlength\arraycolsep{2pt}
		\begin{array}{l}
			\genenc{
			\req{k}{\pid p[\role A]}{\wtil{l.\role B}};C}
				=\\ \qquad 
				\m{start}(k, l'.\role A, \wtil{l.\role B});
				\genenc{C} \ , \text{ where } \pid p@l' \in \Gamma
		\\[5pt]
		\genenc{\gensend;C} =\\ \qquad
			\notify{o}{\jpath{k.B.l}}{e} \qto{\jpath{k.A.B}} ; \genenc{C}
		\\[5pt]
		\genenc{\recDef{X}{C'}{C}} = \recDef{X}{\genenc{C'}}{\genenc{C}}
		\\[5pt]
		\genenc{X} = X
		\end{array}
		\quad
		\begin{array}{l}
		\genenc{\acc{k}{l.\pid q[\role B]}; C} =\\ \qquad
			\m{accept}(\ k,\ \role B, \Gamma(\til l) \ );
			\genenc{C}\ , \text{ where } l \in \til l \text{ and } \til l \in \Gamma
		\\[5pt]
		\genenc{\genbranchI} = \\ \qquad
			\sum\limits_{i \in I}\choice{\oneway{o_i}{x_i} 
				\qfrom{\jpath{k.A.B}}}{\genenc{C_i}\ }
		\\[8pt]
		\genenc{\cond{\pid p.e}{C_1}{C_2}} = \cond{e}{\genenc{C_1}\
		}{\genenc{C_2}\ }
		\\[5pt]
		\genenc{\inact} = \inact
		\end{array}}
	\end{displaymath}}
	% \begin{minipage}{\textwidth}
		\input{figures/encoding_start_accept}
	% \end{minipage}
	\vspace{-1em}
	\caption{Compiler from FC to DCC.}
	\label{fig:encoding_full}
\end{figure*}

==> figures/encoding_start_accept.tex <==
\newcommand{\notext}[1]{}
	{\footnotesize$$
	\hspace{-5pt}\begin{array}l
\m{start}(k, l_\role A.\role A, \wtil{l_\role B.\role B}) =
	\\[-5pt]
		\quad\underbrace{\Seq\limits_{\vphantom{\raisebox{-2pt}{C}}
			\substack{ \jpath{I} \in \{\role A, \til{\role B}\}}}
			\jpath{k.I.l} = l_{\role I}\ ;}_\text{\scriptsize ($s_1$) locations}
		\underbrace{			
			\Seq\limits_{\jpath{I} \in \{\til{\role B}\}}
			\Big(
				\overbrace{
					\cq{\jpath{k.I.A}}
				}^\text{\scriptsize	($s_{2.1}$) \notext{create queue}}
				;
				\overbrace{
					\notify{?}{\jpath{k.I.l}}{\jpath{k}}
				}^\text{\scriptsize ($s_{2.2}$) \notext{spawn request}}
				;
				\overbrace{
					\oneway{sync}{\jpath{k}} \qfrom \jpath{k.I.A}
				}^\text{\scriptsize ($s_{2.3}$) \notext{service response}}
			\Big);
			}_\text{\scriptsize ($s_2$) creation of correlation keys and service processes}
		%
		\underbrace{
			\Seq\limits_{\jpath{I} \in \{\til{\role B}\}}
			\notify{start}{\jpath{k.I.l}}{\jpath{k}} \qto \jpath{k.A.I}
		}_\text{\scriptsize ($s_3$) session start}
	% }
\\[35pt]
\m{accept}(k, \role B,\initg{G}{\role A}{\til{\role C}}{\roles D}) =
		\underbrace{\vphantom{\raisebox{-16pt}{C}}
			\oneway{!}{\jpath{k}}
		}_\text{\raisebox{4pt}{\scriptsize ($a_1$) \notext{spawn accept\ }}}
		;
		\underbrace{\vphantom{\raisebox{-16pt}{C}}
			\Seq\limits_{	\jpath{I} \in \{\role A,\til{\role C}\}/\{\role B\} }
				\Big( 
				\cq{\jpath{k.I.B}} \ \Big)
		}_\text{\scriptsize ($a_2$) \notext{create correlation keys and queues}}
		;
		\underbrace{\vphantom{\raisebox{-16pt}{C}}
			\notify{sync}{\jpath{k.A.l}}{\jpath{k}} \qto{\jpath{k.B.A}}
		}_\text{\raisebox{4pt}{\scriptsize ($a_3$) \notext{service response}}}
		;
		\underbrace{\vphantom{\raisebox{-16pt}{C}}
			\oneway{start}{\jpath{k}} \qfrom{\jpath{k.A.B}}
		}_\text{\raisebox{4pt}{\scriptsize ($a_4$) \notext{session start}}}
\end{array}
$$}

==> figures/jc_semantics.tex <==
\begin{figure}
\small\begin{displaymath}
\hspace{-5pt}\setlength\arraycolsep{2.5pt}\begin{array}{llll}
	\did{DCC}{Recv}
	&
	t_c = \evalfn(e, t)
	\ \wedge \
	M( t_c ) = ( o, t' ) :: \til m
	& \Rightarrow &
	\jprc{\oneway{o}{x} \qfrom{e};B}{t}{M}
	\to
	\jprc{B}{t \tcopy{x}{t'} }{M[t_c \mapsto \til m]}
	\\[2pt]
	\did{DCC}{Cq} 
	&
	\begin{array}l
		P = \jprc{\cq{x};B}{t}{M}
		\\
		\wedge \ t_c \not \in \bigcup_i \dom(M_i) \cup \m{dom}(M)
	\end{array}
	& \Rightarrow &
		\begin{array}l
		\jsrv{B_s,\ P \pp \prod_i \jprc{B_i}{t_i}{M_i}}l
			\to \\ \quad 
		\jsrv{B_s,\ \jprc{B}{t \tcopy{x}{t_c}}{M[t_c \mapsto \emptyseq]}
			\pp \prod_i \jprc{B_i}{t_i}{M_i}}l
		\end{array}
	\\[10pt]
	\did{DCC}{Send} 
	&
	\begin{array}{l}
		P = \jprc{\notify{o}{e_1}{e_2} \qto e_3; B}{t}{M}
		\\
		\wedge \ \evalfn( e_1, t ) = l'
		\ \wedge \
		\evalfn( e_3, t ) = t_c
		\\
		\wedge \ \evalfn(	e_2, t ) = t_m
		\\
		\wedge \ M'' = M'[t_c \mapsto M'(t_c) :: (o, t_m )]
	\end{array}
	& \Rightarrow &
	\begin{array}l
		\jsrv{B_s, P \pp P_1 }{l} \pp 
			\jsrv{B_s', \jprc{B'}{t'}{M'} \pp P_2}{l'}
		\to \\[2pt] \quad 
		 \jsrv{B_s, \jprc{B}{t}{M} \pp P_1 }{l} \pp 
			\jsrv{B_s', \jprc{B'}{t'}{M''} \pp P_2}{l'}
	\end{array}
	\\[20pt]
	\did{DCC}{Start}
	&
	\begin{array}l
		P_1 = \jprc{\notify{?}{e_1}{e_2};B_1}{t_1}{M_1}
		\\
		\wedge \ \evalfn( e_1, t_1 ) = l
		\\
		\wedge \ Q = \jprc{B}{t_\bot\tcopy{x}{\evalfn( e_2, t_1 )} }{\emptyset}
	\end{array}
	& \Rightarrow &
	\begin{array}l
		\jsrv{!(x);B,\ P}{l}	\pp	\jsrv{B'_s,\ P_1 \pp P_2}{l'}
		 \to \\[2pt] \quad \jsrv{!(x);B,\ Q \pp P}{l}
			\pp \jsrv{B'_s,\ \jprc{B_1}{t_1}{M_1} \pp P_2}{l'}	
		\end{array}
\end{array}
\end{displaymath}
	\vspace{-1em}
	\caption{Dynamic Correlation Calculus, semantics (selected).}
	\label{fig:js_semantics_sos}
\end{figure}

==> figures/jc_semantics_sel.tex <==
\begin{figure*}
{\footnotesize
\begin{displaymath}
\begin{array}{l}
	\did{DCC}{Recv}
		\left.\begin{array}l
			t_c = \evalfn(e, t )
			\\
			M( t_c ) = ( o, t' ) :: \til m
		\end{array}\right\}
	\then
		\jprc{\oneway{o}{x} \qfrom{e};B}{t}{M}
		\to
		\jprc{B}{t \tcopy{x}{t'} }{M[t_c \mapsto \til m]}
	\\[10pt]
	\did{DCC}{Cq}
	\left.\begin{array}l
		P = \jprc{\cq{x};B}{t}{M}
		\\
		t_c \not \in \bigcup_i \dom(M_i) \cup \m{dom}(M)
		\\
		t' = t \tcopy{x}{t_c}
	\end{array}\right\}
	\then
		\begin{array}l
		\jsrv{B_s,\ P \pp \prod_i \jprc{B_i}{t_i}{M_i}}l
			\to
		\\[4pt]
		\jsrv{B_s,\ \jprc{B}{t'}{M[t_c \mapsto \emptyseq]}
			\pp \prod_i \jprc{B_i}{t_i}{M_i}}l
		\end{array}
	\\[15pt]
	\did{DCC}{Send}
	\left.\begin{array}l
		P = \jprc{\notify{o}{e_1}{e_2} \qto e_3; B}{t}{M}
		\\
		\evalfn(e_1, t ) = l'
		\quad
		\evalfn(e_2, t ) = t_m
		\\
		\evalfn(e_3, t ) = t_c
		\\
		M'' = M'[t_c \mapsto M'(t_c) ::  (o, t_m )]
	\end{array}\right\}
	\then
		\begin{array}l
			\jsrv{B_s, P \pp P_1 }{l} \pp 
			\jsrv{B_s', \jprc{B'}{t'}{M'} \pp P_2}{l'}
		\\ \to  \quad
		\jsrv{B_s, \jprc{B}{t}{M} \pp P_1 }{l} \pp 
			\\ \;\qquad \jsrv{B_s', \jprc{B'}{t'}{M''} \pp P_2}{l'}
		\end{array}
	\\[20pt]
	\did{DCC}{Start}
		\left.\begin{array}l
			P_1 = \jprc{\notify{?}{e_1}{e_2};B_1}{t_1}{M_1}
			\\
			\evalfn( e_1, t_1 ) = l
			\\
			\evalfn( e_2, t_1 ) = t_m
			\\
			Q = \jprc{B}{t_\bot\tcopy{x}{t_m}}{\emptyset}
		\end{array}\right\}
		\then
		\begin{array}l
			\jsrv{!(x);B,\ P}{l}	\pp	\jsrv{B'_s,\ P_1 \pp P_2}{l'}
			\to\\[2pt]
			\jsrv{!(x);B,\ Q \pp P}{l} \pp \\
			\jsrv{B'_s,\ \jprc{B_1}{t_1}{M_1} \pp P_2}{l'}
		\end{array}
\end{array}
\end{displaymath}}
	\caption{Correlation Calculus, semantics (selected rules)}
	\label{fig:js_semantics}
\end{figure*}


==> figures/jc_structural_congruence.tex <==
\begin{figure}[h]
% $$
% 	\hspace{-1em}\begin{array}{c}
% 		\recDef{X}{B'}{B[X]}
% 		\equiv
% 		\recDef{X}{B'}{B[B']}
% 		\\[.5em]
% 		P \equiv P \pp \jprc{\inact}{t}{\emptyset}
% 		\qquad
% 		(P_1 \pp P_2) \pp P_3  \equiv P_1 \pp (P_2 \pp P_3)
% 		\\[.5em]
% 		P \pp P^\prime \equiv P^\prime \pp P 
% 		\qquad
% 		% \jsrv{B_s, P \pp P'}l \equiv \jsrv{B_s, P' \pp P}l
% 		S \pp S^\prime \equiv S^\prime \pp S 
% 		\\[.5em]
% 		(S_1 \pp S_2) \pp S_3  \equiv S_1 \pp (S_2 \pp S_3)
% 	\end{array}
% $$
{\footnotesize$$
	\hspace{-1em}\begin{array}{c}
		\jprc{\recDef{X}{B'}{B[X]}}{t}{M}
		\equiv
		\jprc{\recDef{X}{B'}{B[B']}}{t}{M}
		\\[.5em]
		P \equiv P \pp \jprc{\inact}{t}{\emptyset}
		\qquad
		(P_1 \pp P_2) \pp P_3 \equiv P_1 \pp (P_2 \pp P_3)
		\\[.5em]
		P \pp P' \equiv P' \pp P
		\qquad
		% \jsrv{B_s, P \pp P'}l \equiv \jsrv{B_s, P' \pp P}l
		S \pp S^\prime \equiv S^\prime \pp S 
		\\[.5em]
		(S_1 \pp S_2) \pp S_3  \equiv S_1 \pp (S_2 \pp S_3)
	\end{array}
$$}
	\caption{Dynamic Correlation Calculus, structural congruence}
	\label{fig:jc_structural_congruence}
\end{figure}

==> figures/ownership_typing_rules.tex <==
\begin{figure*}
\begin{displaymath}
\begin{array}{c}
\infer[\did{O}{Com}]
{
	\Gamma \seq \com{k}{\pid p[\role A]}{\pid q[\role B]}
}
{
	\Gamma \seq \pair{\pid p}{k[\role A]}
	&
	\Gamma \seq \pair{\pid q}{k[\role B]}
}
\qquad
\infer[\did{O}{Send}]
{
	\Gamma \seq \com{k}{\pid p[\role A]}{\role B}
}
{
	\Gamma \seq \pair{\pid p}{k[\role A]}
}
\qquad
\infer[\did{O}{Recv}]
{
	\Gamma \seq \com{k}{\role A}{\pid q[\role B]}
}
{
	\Gamma \seq \pair{\pid q}{k[\role B]}
}
\end{array}
\end{displaymath}
\caption{Choreography Calculus - Ownership Typing}
\label{fig:own_typing_rules}
\end{figure*}

==> figures/preview_example.tex <==
\begin{figure*}
\begin{subfigure}{\textwidth}
%
% PROTOCOLS
%
  \footnotesize
  \begin{displaymath}
	\begin{array}{l}
G_{d} =
 	\gcom{\role C}{\role A}{get\left(
 		\begin{array}{l}
	 		\jpath{creds}: \tstring, 
	 		\\ \jpath{rsc}: \tstring	
 		\end{array}
 		\right)};\ 
	\gcom{\role A}{\role S}{
	\left\{
	\begin{array}{l}
		ok( \tstring );
			\gcom{\role A}{\role C}{ok()};
			\gcom{\role S}{\role L}{log(\tstring)};
			\m{rec}\;\mathbf{t};
			\gcom{\role S}{\role C}{
			\left\{
				\begin{array}{l}
					pkt( \tbytes ); \mathbf{t},
					\\
					chksum( \tstring )
				\end{array}
			\right \}},
			\\
		ko(\tstring);
		\gcom{\role A}{\role C}{ko()};
		\gcom{\role S}{\role L}{log(\tstring)}
	\end{array}
	\right\}}
	\\[2em]
G_{s} =
	\gcom{\role U}{\role F}{create(\tstring)};
	\m{rec}\;\mathbf{s};
	\gcom{\role U}{\role F}{\left\{
		\begin{array}{l}
			append( \tbytes ); \mathbf{s},
			\\
			check( \tstring );
			\gcom{\role F}{\role U}{\left\{
				\begin{array}{l}
					saved(  ),
					\\
					discarded(  )
				\end{array}
			\right\}}
		\end{array}
	\right\}}
\end{array}
  \end{displaymath}
  \vspace{-2mm}
  \caption{Protocols}
  \label{fig:preview_example_protocols}
\end{subfigure}
%
% COMPLETE CHOREOGRAPHIES
%
\begin{subfigure}{.5\textwidth}
  \footnotesize
  \begin{displaymath}
	\ResetLN
	{\setlength\arraycolsep{2pt}
	C_{c} = \left\{
	\begin{array}{rl}
		\LN & \req{k_d}{\prc cC}{l_{\role A}.\role A,
			l_{\role S}.\role S,l_{\role L}.\role L};
		\\
		\LN & \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get};
		\\[.3em]
		\LN & \recDef{\m{store}}{
		\\
		\LN &	\quad \com{k_d}{\role S}{\prc cC.\{
		\\
		\LN & \qquad pkt( \jpath{bb} );
		\\
		\LN & \quad\qquad \com{k_s}{\prc cU.\jpath{bb}}{
						\prc fF.append(\jpath{data})};
		\\
		\LN & \quad\qquad \recCall{\m{store}}\; ,
		\\
		\LN & \qquad check( \jpath{cs} );
		\\
		\LN & \quad\qquad \cond{\pid f.\m{check}( \jpath{fname}, \jpath{cs} )}{
		\\
		\LN & \qquad\qquad \com{k_s}{\prc fF}{\prc cU.saved}
		\\
		\LN & \quad\qquad }{
		\\
		\LN & \qquad\qquad \com{k_s}{\prc fF}{\prc cU.discarded}
		\\
		\LN & \quad\qquad }
		\\
		\LN & \quad \}}
		\\
		\LN & }{
		\\[.3em]
		\LN & \quad \com{k_d}{\role A}{\prc cC.\{
		\\
		\LN & \qquad ok;
		\\
		\LN & \quad\qquad \start{k_s}{\prc cU}{l_{\role F}.\prc fF};
		\\
		\LN & \quad\qquad \com{k_s}{\prc cU.\m{name}()}{\prc fF.create(\jpath{fname})};
		\\
		\LN & \quad\qquad \recCall{\m{store}}\; ,
		\\
		\LN & \qquad ko
		\\
		\LN & \quad \}}
	}
	\end{array}
	\right.
	}
  \end{displaymath}
	\caption{Client partial choreography}
  \label{fig:preview_example_client}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	C_{s} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role A}.\prc aA,
		l_{\role S}.\prc sS,l_{\role L}.\prc lL};
	\\
	\LN & \com{k_d}{\role C}{\prc aA.get(\jpath{req})};
	\\
	\LN & \cond{\pid a.isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ok(\jpath{rsc})};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ok};
	\\
	\LN & \quad \com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
	\\[.4em]
	\LN & \quad \recDef{\m{stream}}{
	\\
	\LN &
		\qquad\cond{ \pid s.\m{more}(\jpath{rsc})}{
		\\
		\LN & \quad\qquad \com{k_d}{\prc sS.\m{next}(\jpath{rsc})}{\role C.pkt};
		\\
		\LN & \quad\qquad \recCall{\m{stream}} 
		\\ \LN &\qquad }{
		\\
		\LN & \quad\qquad \com{k_d}{\prc sS.\m{chksum}(\jpath{rsc})}{\role C.chksum}
		\\ \LN & \qquad}
	\\ \LN & \quad}{
	\\[.2em] \LN & \recCall{\m{stream}}
	}
	\\ \LN & }{
	\\ 
		\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ko(\jpath{rsc})};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ko};
	\\
	\LN & \quad \com{k_d}{\prc sS.\m{logko}(\jpath{rsc})}{\prc lL.log(\jpath{log})}
	\\ \LN &
	}
	\end{array}
	\right.
	}
  \end{displaymath}
	\caption{Server partial choreography}
  \label{fig:preview_example_server}
\end{subfigure}

\begin{subfigure}{\textwidth}
	\begin{displaymath}
		ENDPOINT\ PROJECTION
	\end{displaymath}
\end{subfigure}

%
%	PROJECTED CHOREOGRAPHIES --- A
%
\begin{subfigure}{.33\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C_{s}}{\pid a} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role A}.\prc aA};
	\\
	\LN & \com{k_d}{\role C}{\prc aA.get(\jpath{req})};
	\\
	\LN & \cond{\pid a.isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\role S.ok};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ok}
	\\ \LN & }{
	\\ 
		\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\role S.ko};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ko}
	\\ \LN &
	}
	\end{array}
	\right.
	}
  \end{displaymath}
	\caption{EPP of process $\pid a$}
  \label{fig:preview_example_epp_A}
\end{subfigure}
%
%	PROJECTED CHOREOGRAPHIES --- S
%
\begin{subfigure}{.4\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C_{s}}{\pid s} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role S}.\prc sS};
	\\
	\LN & \com{k_d}{\role A}{\prc sS.\{
	\\
	\LN & \quad ok( \jpath{rsc} );
	\\
	\LN & \quad \com{k_d}{\prc sS.\m{logok}(\jpath{req})}{\role L.log};
	\\
	\LN & \quad \cdots\ ,
	\\ 
	\LN & \quad ko( \jpath{rsc} );
	\\
	\LN & \quad \com{k_d}{\prc sS.\m{logko}(\jpath{req})}{\role L.log}
	\\
	\LN & \}}
	\end{array}
	\right.
	}
  \end{displaymath}
	\caption{EPP of process $\pid s$}
  \label{fig:preview_example_epp_S}
\end{subfigure}
%
% PROJECTED CHOREOGRAPHIES --- L
%
\begin{subfigure}{.2\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C_{s}}{\pid l} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role L}.\prc lL};
	\\
	\LN & \com{k_d}{\role S}{\prc lL.log(\jpath{log})};
	\end{array}
	\right.
	}
  \end{displaymath}
	\caption{EPP of process $\pid l$}
  \label{fig:preview_example_epp_L}
\end{subfigure}

\begin{subfigure}{\textwidth}
	\begin{displaymath}
		ENCODING
	\end{displaymath}
\end{subfigure}
%
%	ENCODING --- A
%
\begin{subfigure}{.41\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\begin{array}{l}
	\genenc{\epp{C_{s}}{\pid a}} = \\[5pt] 
	\qquad\left\{
	\begin{array}{rl}
	\LN & \oneway{!}{\jpath{kd}};
	\\
	\LN & \jpath{kd.C.A} = \new;
	\\
	\LN & \cq{\jpath{kd.C.A}};
	\\
	\LN & \jpath{kd.S.A} = \new;
	\\
	\LN & \cq{\jpath{kd.S.A}};
	\\
	\LN & \jpath{kd.L.A} = \new;
	\\
	\LN & \cq{\jpath{kd.L.A}};
	\\
	\LN & \notify{sync}{\jpath{kd.C.l}}{\jpath{kd}} \qto{\jpath{kd.A.C}};
	\\
	\LN & \oneway{start}{\jpath{kd}} \qfrom{\jpath{kd.C.A}};
	\\
	\LN & \oneway{get}{\jpath{req}} \qfrom{\jpath{kd.C.A}};
	\\
	\LN & \cond{isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \notify{ok}{\jpath{kd.S.l}}{\jpath{req.rsc}} 
		\qto{\jpath{kd.A.S}};
	\\
	\LN & \quad \notify{ok}{\jpath{kd.C.l}}{} 
		\qto{\jpath{kd.A.C}}  
	\\ \LN & }{
	\\ 
	\LN & \quad \notify{ko}{\jpath{kd.S.l}}{\jpath{req.rsc}} 
		\qto{\jpath{kd.A.S}};
	\\
	\LN & \quad \notify{ko}{\jpath{kd.C.l}}{} 
		\qto{\jpath{kd.A.C}}  
	\\ \LN &
	}
	\end{array}
	\right.
	% \\\\	
	% \jsrv{\enc{\epp{C_{s}}{\pid a}}_{l_{\role A}} ,\inact}{l_{\role A}}
	\end{array}
	}
  \end{displaymath}
	\caption{Compilation of service at $l_{\role A}$}
  \label{fig:preview_example_encoding_A}
\end{subfigure}
%
%	ENCODING --- C
%
\begin{subfigure}{.3\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\begin{array}{l}
	\genenc{\epp{C_{c}}{\pid c}} = \\[5pt] 
	\qquad\left\{
	\begin{array}{rl}
	\LN & \jpath{kd.C.l} = l_{\role C};
	\\
	\LN & \ldots
	\\
	\LN & \jpath{kd.A.C} = \new;
	\\
	\LN & \cq{\jpath{kd.A.C}};
	\\
	\LN & \notify{?}{\jpath{kd.A.l}}{\jpath{kd}};
	\\
	\LN & \oneway{sync}{\jpath{kd}} \qfrom{\jpath{kd.A.C}};
	\\
	\LN & \jpath{kd.S.C} = \new;
	\\
	\LN & \cq{\jpath{kd.S.C}};
	\\
	\LN & \notify{?}{\jpath{kd.S.l}}{\jpath{kd}};
	\\ 
	\LN & \ldots
	\\
	\LN & \notify{start}{\jpath{kd.A.l}}{\jpath{kd}} \qto{\jpath{kd.C.A}};
	\\
	\LN & \notify{start}{\jpath{kd.S.l}}{\jpath{kd}} \qto{\jpath{kd.C.S}};
	\\
	\LN & \notify{start}{\jpath{kd.C.l}}{\jpath{kd}} \qto{\jpath{kd.C.L}};
	\\
	\LN & \ldots
	\end{array}
	\right.
	% \\\\	
	% \jsrv{\inact, \jprc{\enc{\epp{C_{c}}{\pid c}}_{\pid c}}
	% 	{\env(\pid a).\estate}{\env(\pid a).\equeues}}{l_{\role C}}
	\end{array}
	}
  \end{displaymath}
	\caption{Compilation of service at $l_{\role C}$}
  \label{fig:preview_example_encoding_C}
\end{subfigure}
%
% ENCODING --- L
%
\begin{subfigure}{.33\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\begin{array}{l}
	\genenc{\epp{C_{s}}{\pid a}} = \\[5pt] 
	\qquad\left\{
	\begin{array}{rl}
	\LN & \oneway{!}{\jpath{kd}};
	\\
	\LN & \jpath{kd.C.L}=\new;
	\\
	\LN & \cq{\jpath{kd.C.L}};
	\\
	\LN & \jpath{kd.A.L}=\new;
	\\
	\LN & \cq{\jpath{kd.A.L}};
	\\
	\LN & \jpath{kd.S.L}=\new;	
	\\
	\LN & \cq{\jpath{kd.S.L}};
	\\
	\LN & \notify{sync}{\jpath{k.C.l}}{\jpath{kd}} \qto{\jpath{kd.L.C}};
	\\
	\LN & \oneway{start}{\jpath{kd}} \qfrom{\jpath{kd.C.L}};
	\\
	\LN & \oneway{log}{\jpath{log}} \qfrom{\jpath{kd.S.L}}
	\end{array}
	\right.
	% \\\\
	% \jsrv{\enc{\epp{C_{s}}{\pid l}}_{l_{\role L}} ,\inact}{l_{\role L}}
	\end{array}
	}
  \end{displaymath}
	\caption{Compilation of service at $l_{\role L}$}
  \label{fig:preview_example_encoding_L}
\end{subfigure}
	\caption{Example}
\end{figure*}

==> figures/projection_example.tex <==
\begin{figure*}
\begin{subfigure}{.45\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C}{\pid a} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role A}.\prc aA};
	\\
	\LN & \com{k_d}{\role C}{\prc aA.get(\jpath{req})};
	\\
	\LN & \cond{\pid a.isValid( \jpath{req} ) }{
	\\ 
	\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\role S.ok};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ok}
	\\ \LN & }{
	\\ 
		\LN & \quad \com{k_d}{\prc aA.\jpath{req.rsc}}{\role S.ko};
	\\
	\LN & \quad \com{k_d}{\prc aA}{\role C.ko}
	\\ \LN &
	}
	\end{array}
	\right.
	}
  \end{displaymath}
	% \caption{EPP of process $\pid a$}
 %  \label{fig:example_epp_A}
\end{subfigure}
%
%	PROJECTED CHOREOGRAPHIES --- S
%
\begin{subfigure}{.55\textwidth}
	\ResetLN
  \footnotesize
  \vspace{.5em}
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C}{\pid {dm}} = \left\{
	\begin{array}{rl}
	\LN & \acc{k_d}{l_{\role S}.\prc {dm}{DM}};
	\\
	\LN & \com{k_d}{\role A}{\prc {dm}{DM}.\{
	\\
	\LN & \quad ok( \jpath{rsc} );
	\\
	\LN & \qquad \com{k_d}{\prc {dm}{DM}.\m{logok}(\jpath{req})}{\role L.log};
	\\
	\LN & \quad \cdots\ ,
	\\ 
	\LN & \quad ko( \jpath{rsc} );
	\\
	\LN & \qquad \com{k_d}{\prc {dm}{DM}.\m{logko}(\jpath{req})}{\role L.log}
	\\
	\LN & \}}
	\end{array}
	\right.
	}
  \end{displaymath}
  % \vspace{5pt}
	% \caption{EPP of process $\pid {dm}$}
 %  \label{fig:example_epp_S}
\end{subfigure}
%
% PROJECTED CHOREOGRAPHIES --- L
%
\begin{subfigure}{\textwidth}
	\ResetLN
  \footnotesize
  \begin{displaymath}
	{\setlength\arraycolsep{2pt}
	\epp{C}{\pid l} = \Big\{
	\LN \; \acc{k_d}{l_{\role L}.\prc lL};
	\qquad
	\LN \; \com{k_d}{\role S}{\prc lL.log(\jpath{log})};
	}
  \end{displaymath}
\end{subfigure}	
	\vspace{-3pt}
	\caption{Endpoint Projections of $C_c \pp C_s$. Projection on $\pid a$, $\pid
	{dm}$ (excepts), and $\pid l$.}
  \label{fig:example_epp}
\end{figure*}

==> figures/projection_sel.tex <==
\begin{figure*}
{\footnotesize
$$
\genproj{\gencom ; C} = \begin{cases}
		\gensend ; \genproj{C} & 
			\mbox{if } \pid r = \pid p
		\\
		\genrecv ; \genproj{C} &
			\mbox{if } \pid r = \pid q
		\\
		\genproj{C} & \mbox{otherwise}
	\end{cases}
\qquad
\genproj{\gencond} = \begin{cases}
		\cond{\pid p.e}{\epp{C_1}{\pid r}}{\epp{C_2}{\pid r}} & \mbox{if } \pid r = \pid p
		\\
		\genproj{C_1} \sqcup \genproj{C_2} & \mbox{otherwise}
	\end{cases}
$$
}
\caption{Choreography Calculus, process projection --- selected rules}
\label{fig:cc_projection}
\end{figure*}

==> figures/protocols_example.tex <==
\begin{figure*}
  \begin{displaymath}
	\begin{array}{l}
G_{d} =
 	\gcom{\role C}{\role A}{get\left(
 		\left\{\begin{array}{l}
	 		\jpath{creds}: \tstring, 
	 		\\ \jpath{rsc}: \tstring
 		\end{array}\right\}
 		\right)};
 	\\\hspace{25pt}
	\gcom{\role A}{\role{DM}}{
	\left\{
	\begin{array}{l}
		ko(\tstring);
		\gcom{\role A}{\role C}{ko()};
		\gcom{\role{DM}}{\role L}{log(\tstring)},
		\\
		ok( \tstring );
			\gcom{\role A}{\role C}{ok()};
			\gcom{\role{DM}}{\role L}{log(\tstring)};
			\m{rec}\;\mathbf{t};
			\gcom{\role{DM}}{\role C}{
			\left\{
				\begin{array}{l}
					pkt( \tbytes ); \mathbf{t},
					\\
					chksum( \tstring )
				\end{array}
			\right \}}
	\end{array}
	\right\}}
	\\[2em]
G_{s} =
	\gcom{\role U}{\role F}{create(\tstring)};
	\m{rec}\;\mathbf{s};
	\gcom{\role U}{\role F}{\left\{
		\begin{array}{l}
			append( \tbytes ); \mathbf{s},
			\\
			check( \tstring );
			\gcom{\role F}{\role U}{\left\{
				\begin{array}{l}
					saved(  ),
					\\
					discarded(  )
				\end{array}
			\right\}}
		\end{array}
	\right\}}
\end{array}
  \end{displaymath}
  \vspace{-2mm}
  \caption{Protocols example}
  \label{fig:preview_example_protocols}
\end{figure*}

==> figures/sos_chor_seff_inline.tex <==
\begin{figure}
{\footnotesize
\setlength{\arraycolsep}{3pt}
$$
\hspace{-5pt}\begin{array}{llll}
\did{\env}{Start}
&
\env'\!=\!\env\big[\pid r \mapsto f_\bot\big]_{\pid r \in \{\pids q\}}
\big[	
	\chanto{k}{\role C}{\role E} \mapsto \emptyseq 
\big]_{\role C,\role E \in \{\role A, \roles B\}, \role C \neq \role E}
& \Rightarrow &
\renv{\env}{\genstart}{\env'} 
\\[3pt]
\did{\env}{Send}
&
\env( \chanto{k}{\role A}{\role B} ) = \til m
\ \wedge \
v = \evalfn(\; e, \env( \pid p ) \;)
& \Rightarrow &
\renv{\env}{\gensend}{\env\big[	
	\chanto{k}{\role A}{\role B} \mapsto \til m :: (o, v)
\big]}
\\[3pt]
\did{\env}{Recv}
&
\env( \chanto{k}{\role A}{\role B} ) = (o,v) :: \til m
\ \wedge \
\env' = \env\big[ \chanto{k}{\role A}{\role B} \mapsto \til m \big]  
& \Rightarrow &
\renv{\env}{\genrecv}{\env'\big[ 
	\pid q \mapsto \env( \pid q )[ x \mapsto v ] 
\big]}
	\end{array}
	$$}
	\vspace{-1em}
 	\caption{Effects on Deployment.}
	\label{fig:seff_semantics}
\end{figure}

==> preview.tex <==
%auto-ignore

In this section we introduce our model and approach through a working example. 

%
%Key elements of our choreographic model are \emph{protocols} and
%\emph{choreographies}.
%Figure~\ref{fig:preview_example_protocols} reports the specification of the
%protocols, used by the choreographies in
%Figs.~\ref{fig:preview_example_client}, and~\ref{fig:preview_example_server}.
%
%\textbf{Protocols as Global Types.} A protocol is an abstract specification of
%the structure of some communications in a system. We represent protocols with
%\emph{global types}~\cite{HYC08}, i.e., global descriptions where entities,
%abstracted as \emph{roles}, communicate following a given conversation
%structure.
%
%The first protocol, called $G_d$, describes the interaction between a Client
%$\role C$ and a system for verified file transfer. The system is composed by a
%download server process $\role S$, a download access manager $\role A$, and a
%logger $\role L$.
%
%Following $G_d$, $\role C$ asks for a file to $\role A$ through operation
%$get$. The type of the exchanged message contains two values of type
%$\tstring$: $\jpath{creds}$ for the credentials of $\role C$ and $\jpath{rsc}$
%for the resource identifier of the file (e.g., a URL). Then $\role A$ notifies
%$\role S$ whether the credentials and the resource identifier are valid or not.
%%
%If they are not valid, $\role A$ sends a message
%on operation $ko$ to $\role S$, with the outcome of the validation
%($\tstring$). Next $\role A$ sends an empty message (empty parentheses are a
%short-cut for type $\tunit$) to $\role C$ on operation $ko$ to inform it of the
%failed attempt and, finally, the protocol ends with $\role S$ forwarding to the
%logger $\role L$ the error received from $\role A$ through operation $log$.
%%
%If the validation of the request is valid, $\role A$ sends a message on
%operation $ok$ to $\role S$, with the resource identifier of the requested
%file. Next, $\role A$ sends an empty message to $\role C$ on operation $ok$ to
%acknowledge the success of the request and $\role S$ asks to $\role L$ to $log$
%the request. The protocol continues with $\m{rec}\;\mathbf{t}$. This is the
%definition of a \emph{label-guarded recursion}. Calling the label $\mathbf {t}$
%repeats the protocol that contains it, starting from the definition of $\mathbf
%{t}$. Then $\role S$ either: \emph{i}) transfers a packet of $\tbytes$ of the
%requested file to $\role C$, on operation $pkt$, continuing to the next packet
%by calling $\mathbf{t}$, or \emph{ii}) ends the protocol by sending the checksum
%($chksum$) of the file to $\role C$.
%
%The second protocol, named $G_s$, describes the interaction between a User
%$\role U$ of an operative system and a process $\role F$ that can access the
%filesystem. The protocol starts with $\role U$ asking to $\role F$ to $create$
%a new file ($\tstring$). Then, it defines the recursive procedure $\mathbf {s}$
%and proceeds with a communication between $\role U$ and $\role F$. If $\role U$
%has a new packet of $\tbytes$ to be appended to the file, it sends a message to
%$\role F$ through operation $append$ and recursively calls $\mathbf{s}$.
%Otherwise, $\role U$ ends the file transfer and forwards to $\role F$ the
%checksum string via operation $check$. Finally, $\role F$ informs $\role U$ on
%whether it $saved$ the file or $discarded$ it, based on the outcome of the
%checksum on the file.

We want to develop a system which allows the interaction between  a Client
$\role C$ and a Server $\role S$ for verified file transfer. The server is
composed by a download process $\role D$, an access manager  $\role A$ and a
logger $\role L$. The behaviour of the system can be informally described as
follows.

The client $\role C$ asks for a file transfer to $\role A$ by sending its
credentials and the identifier of the file (e.g., a URL). The access manager
$\role A$ then check whether the credentials and the  identifier are valid. If
not, $\role A$ transmit the outcome of the validation to $\role D$ and then
notifies the failure  to $\role C$. In its turn,  $\role S$ forward the error
received from $\role A$ to the logger $\role L$.
%
If the validation of the request is valid, $\role A$ sends a message to $\role
S$ containing the resource identifier of the requested file and then sends a
message to $\role C$  to acknowledge the success of the request. Hence  and
$\role D$ asks to $\role L$ to $log$ the request and start the actual transfer
by repeating, recursively, the transfer of  a packet of bytes of the requested
file to $\role C$ until the End of File is reached and  the checksum is sent to
$\role C$. In its turn $\role C$ uses a process  $\role F$ of the operative
system in order to access the file system and save the file: $\role C$ asks to
$\role F$ to $create$ a new file and then, through a recursive procedure, it
sends the packets to be appended to the file until the transfer is terminated.
At this point  the checksum is sent and finally  $\role F$, depending on the
outcome of the checksum,  notify  $\role C$ whether it $saved$ or $discarded$
the file.


It is worth noting that in this simple example two kind of interactions or, in
other terms, two protocols are involved on the client side: one for
communicating with the server in order to download the file, and another one
for saving it through the functionalities of the file system. As we will see,
our approach allows a smooth integration of this kind of different behaviours
within the same (choreographic) process.


Our first step in the development of the system introduced above is the
definition, in Figure XXX, of a suitable (applied) choreography which describes
globally the system in terms of two  (parallel) processes $C_c$ and $C_s$
representing  the client $\role C$  and the server $\role S$, respectively.
Note that is not a purely abstract description of a protocol, as one could
obtain with such formalisms as global types, but is a first, high level,
program.

Before going into the details of the code let us observe that, in general, key elements of choreographies are \emph{processes}.
and \emph{sessions} . A process represents an entity that executes a sequence of instructions, 
while a session implements the communications among the processes taking part in it (NON MI PIACE MOLTO 
QUESTA DEF DI SESSIONE).  Processes ca be dynamically created and they can create new sessions 
(SEMPRE O SOLO QUI?). 
Important in choreographies are also roles, which are used to indicate specific classes of behaviours in specific contexts: for example, the client $\role C$, the access manager $\role A$ etc. in our example are roles.  

A first distinguishing feature of our approach is the presence of specific of
deployment information which is given in terms of locations: these are used to
identify the places where deployment of processes take place or, in other
terms, where services are located. In a sense locations in our model are
similar to public channels which, in other choreographic approaches, are used
to model the creation of a new session, even though a location can support only
the behaviour of one single role. More precisely ... QUI DIRE LA RELAZIONE
PRECISA FRA SESSIONE E LOCATION. It is worth noting that the presence of
locations, rather than channels names, makes easier the link of our applied
choreographic language with real implementations. DIRE QUALCHE COSA SU
CORRELAZIONE AT THIS STAGE ??



%
%XXXXXand XXX which are very close to the real world 
%implementations.
%
%In this work, we introduce other two key-elements: the \emph{environment}
%($\env$) and the locations $l_1,\ldots,l_n$. $\env$ is a global structure
%that contains the state of the processes in a choreography. We call the
%couple $\env,C$ a \emph {running choreography}.
%
%\textbf{The Environment.}
%The reason for introducing $\env$ is threefold: \emph{i}) $\env$ allows to
%clearly define how correlation works by keeping track of the evolution of its
%companion choreography; \emph{ii}) we use $\env$ to ease the process of
%compilation from a choreography to a set of processes and
%\emph{iii}) to prove that a choreography and its compilation behave
%accordingly. Indeed we prove that, for any evolution of the choreography, the
%information (processes, states, and queues) in $\env$ is the same as the
%union of the local information in the compilation.
%
%Figure~\ref {fig:E} depicts the structure of $\env$. For each process in a
%choreography $C$, $\env$ contains the location of all processes $\pid
%p_1\,\ldots,\pid p_n$ in $C$, their state ($\estate$) and their set of queues
%($\equeues$). $\env$ identifies a specific queue of a process with a set of
%values, i.e., let $\pid p$ be a process in $\env$, $\env(\pid p).\equeues$ is
%a partial function that given a set of values $t$ ($t \in
%\m{dom}(\env(\pid p).\equeues)$) returns a queue of messages $\til m$.
%
%\textbf{Locations and Public Channels}
%
%\textbf{BOZZA, SCRIVERE MEGLIO!!!}
%
%A standard practice of Choreography Programming and Session Types is to model the creation of a new session between different processes via \emph{public channels} typed by a global type. Locations in our model are similar to public channels, but they only support one local type, i.e., the behaviour of one of the roles of a global type. However, the (lexicographic) union of a set of locations can be typed by a global type.
%
%Given a typing environment $\Gamma$, a global type $G$, and sequence of
%locations $\til l$, $\til l$ has type $G$ in $\Gamma$ if, for all roles in $G$, there exists $l \in \til l$ whose local type is the type of role $\role R$ in $G$.
%
%Let $C = C_c \pp C_s$ parallel composition of the two partial choreographies $C_c$ and $C_s$, resp. in Figs.~\ref{fig:preview_example_client} and~\ref{fig:preview_example_server}. Let $l_{\role C}$ be the location of process $\pid c$ in Figure~\ref{fig:preview_example_client}. The sequence of locations $l_{\role C},l_{\role A},l_{\role S},l_{\role L}$ and $l_{\role C}, l_{\role F}$ respectively implement the global types $G_d$ and $G_s$.
%
%Below we comment the salient runtime behaviours of $\env,C$.
%
%\textbf{Starting of a new session: correlation and queues.}
%

CAMBIARE NEL CODICE RUOLO S IN RUOLO D

Below we comment the behaviour of a choreography that implements the
interaction described above. In order to explain the benefits of our approach,
we first describe one of the key element of our model: the \emph {environment}
($\env$). $\env$ is a global structure that contains the state of the processes
in a choreography. Given a choreography $C$, we call the couple $\env,C$ a
\emph {running choreography}. The reason we introduced $\env$ is that we need
it to model message passing based on data (rather than names). At runtime
$\env$ keeps track of the evolution of a choreography.

Figs.\ref{fig:preview_example_client} and~\ref{fig:preview_example_server} with
respectively the code of choreographies $C_c$ and $C_s$. In the code, the
behaviours of our components are represented by the roles appearing in the
choreographies with the same notation indicated above ($\role C$ for the
Client, etc.).

Let us run some salient parts of the parallel composition of $C_c$ and $C_s$
along with environment $\env$, written $\env,C_c \pp C_s$.

The interaction between the first two statements (Line 1) of $C_c$ and $C_s$
spawns a new session named $k_d$. At Line 1 of $C_c$ process $\pid c$, playing
role $\role C$, requests to create a new session with some new processes at
locations $l_{\role A}$, $l_{\role S}$, and $l_{\role L}$. Line 1 of $C_s$
matches the request with the newly created processes $\pid a$ (playing $\role
A$, running at location $l_{\role A}$), $\pid s$ (playing $\role S$, running at
$l_{\role S}$), and $\pid l$ (playing $\role L$, running at $l_{\role L}$).

Let $\wtil{l.\prc qB} = l_{\role A}.\prc aA,l_{\role S}.\prc sS,l_{\role
L}.\prc lL$, and $C_c'$ and $C_s'$ continuation of respectively $C_c$ and $C_s$
after Line 1. $E,C$ reduces to
%
$$
\hspace{-.5em}\begin{array}{l}
\env,
\req{k_d}{\prc cC}{\wtil{l.\prc qB}}; C_c' 
	\pp
	\acc{k_d}{\wtil{l.\prc qB}}; C_s'		
\to
\\
\env \seff (\ \start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}}\ ), C_c' \pp C_s'
\end{array}	
$$
%
The writing $\env \seff ( \start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}} )$
means that $\env$ records the effect of the start. As a result, the new state
of $\env$ is ready to handle message passing in session $k_d$.

\textbf{Message passing.}
%

\textbf{METTERE UN RIFERIMENTO AL TIPO!!!}

Line 2 of $C_c$ and $C_s$ respectively represent send and receive (partial)
operations. At Line 2 of $C_c$, $\com{k_d}{\prc cC.\m{mkReq()}}{\role A.get}$,
means that through session $k_d$, $\pid c$ (playing role $\role C$), sends the
result of the evaluation of function $\m{mkReq()}$ on operation $get$ to the
external process that plays role $\role A$. Note that $C_c$ does not specify
the name of the process playing $\role A$. The name has to be defined by the
complementary partial choreography that implements the process playing
$\role A$ ($C_s$). Below we report the reduction steps of the communication
($C_c'$ and $C_s'$ continuations of resp. $C_c$ and $C_s$ after Line 2).
%
{\scriptsize
$$
\hspace{-.5em}\begin{array}{l}
	\env,\ \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get};C_c' \pp
			 \com{k_d}{\role C}{\prc aA.get(\jpath{req})};C_s'
	\to
	\\
	\env\ \seff \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get},\ C_c' \pp
			 \com{k_d}{\role C}{\prc aA.get(\jpath{req})};C_s'
	\to
	\\
	\env' \seff \com{k_d}{\role C}{\prc aA.get(\jpath{req})},\ C_c' \pp C_s'
\end{array}
$$
}
%
First $\pid c$ sends the message to the process playing $\role A$. The effect
of $\env' = \env\ \seff \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get}$ is that
$\env'$ stored a new message in the queue pointed by $\jpath {kd.C.A.c}$ of
process $\pid a$. The content of the message is the evaluation of $\m{mkReq
()}$ on the state of $\pid c$. We remark that the effect does not need to
carry the identity of $\pid a$ in $C$. $\env$ can guess it from the
correlation data used by $\pid c$. The intention behind this choice is that
it will ease the process of compilation, as it exploits the same technique
used to route messages in the target language of compilation.

Then process $\pid a$ reads the message from $\role C$ for operation $get$,
in the queue pointed by $\jpath {kd.C.A}$. The effect of $\env' \seff
\com{k_d}{\role C}{\prc aA.get(\jpath{req})}$ removes the message from the
queue and assigns its content to variable $\jpath{req}$ in the state of $\pid
a$.

\textbf{Asynchrony.}
%
One of the benefits of including the environment in our model is that it
makes message passing inherently asynchronous. Indeed, in the example above
the two instructions at Line 2 of $C_c$ and $C_s$ are asynchronous. E.g.,
$\pid c$ may have already delivered the message and passed to the next
instruction, whilst $\pid a$ still had to reach Line 2 and read the message.
This holds also for complete operations in our semantics. They first reduce
to a send and then execute a reception.

This means that, even if a choreography defines a certain order in which its
processes shall receive (read) their messages, this order can change at
runtime. This is actually what happens in real-world distributed system.
Messages (data) are consumed according to the state of computation of each
process. Our model naturally matches this feature.

The execution of Lines 4-5 of $C_s$ show this concept (we omit
effects on $\env$ for brevity, $C_s'$ continuation of $C_s$ after Line 5):
%
{\footnotesize
$$
\hspace{-.5em}\begin{array}{l}
 \env, \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ok(\jpath{rsc})};
\com{k_d}{\prc aA}{\role C.ok};C_s'\pp C_c
\to
\\ \env', \com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};
\com{k_d}{\prc aA}{\role C.ok};C_s'\pp C_c
\swapC
\\ \env', \com{k_d}{\prc aA}{\role C.ok};\com{k_d}{\role A}{\prc
sS.ok(\jpath{rsc})};C_s'\pp C_c
\to
\\ \env'', \com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};C_s'\pp C_c
\end{array}
$$
}
%
After $\pid a$ sent its message to $\pid s$, it is possible
that $\pid s$ is not ready to read it (e.g., due to scheduling). In our
model, we allow two operations to swap if they have no process in common.
Operations $\com{k_d}{\role A}{\prc sS.ok}$ and $\com{k_d}{\prc aA}{\role
C.ok}$ regard resp. $\pid s$ and $\pid a$ and can swap. We indicate swapping
with $\swapC$. After the swap, $\pid a$ delivers its message to $\role C$.

Another example of asynchrony are Lines 9-10 of $C_s$. $\pid s$ can send all
the sequence of packets of the file to $\pid c$, whilst $\pid c$ might have
read none of them yet. The queue between them works as a buffer.

Remarkably, although allowing for asynchrony, our type system guarantees to
preserve the order of interactions, i.e., the order two processes
send and receive messages to and from each other.

\textbf{Parallelism.}
%
Our model also automatically achieves the maximum degree of parallelism among
different processes.

Lines 4-6 of $C_s$ show an example of that. 
%Above, we commented that receptions
%and reads are asynchronous. E.g., the read at Line 4 ($\pid s$ reads the
%message for operation $ok$) can execute later than the read at Line 5 ($\role
%C$ reads the message for $ok$). 
The instructions at Lines 5-6 concern a disjoint set of processes (resp. $\pid
a$, $\pid s$, and $\pid l$). According to our model the two instructions can
swap, thus their order of execution is non-deterministic. A possible reduction
is (effect on $\env$ omitted for brevity, $C_s'$ continuation of $C_s$ after
Line 6):
%
{\scriptsize
$$
\hspace{-.5em}\begin{array}{ll}
\hspace{-.5em}\begin{array}{l}
	\env, \begin{array}{l}
		\com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ok(\jpath{rsc})};
	  \com{k_d}{\prc aA}{\role C.ok};
	  \\
		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
		C_s' \pp C_c	
	\end{array}
\end{array}
\to
\\[7pt]
\hspace{-.5em}\begin{array}{l}
	\env', \begin{array}{l}
		\com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};
	  \com{k_d}{\prc aA}{\role C.ok};
	  \\
		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
		C_s' \pp C_c	
	\end{array}
\end{array}
\to
\\[7pt]
\env'',
	  \com{k_d}{\prc aA}{\role C.ok};
		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
		C_s' \pp C_c	
\swapC
\\[3pt]
\env'',
		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
	  \com{k_d}{\prc aA}{\role C.ok};
		C_s' \pp C_c	
\to
\\[3pt]
\env''',
		\com{k_d}{\role S}{\prc lL.log(\jpath{log})};
	  \com{k_d}{\prc aA}{\role C.ok};
		C_s' \pp C_c	
\swapC
\\[3pt]
\env''',
	  \com{k_d}{\prc aA}{\role C.ok};
		\com{k_d}{\role S}{\prc lL.log(\jpath{log})};
		C_s' \pp C_c	
\to \ldots
\end{array}
$$
}

After $\pid a$ sent its message, let us suppose that $\pid s$ reads it. Then,
since no process is shared between the instructions at Lines 5 and 6, it is
possible to swap them. Then $\pid s$ sends its message to $\pid l$, the two
Lines can swap again, and proceed with e.g., $\pid a$ delivering its message.
Indeed, there are other possible execution scenarios, all permitted by our
model.

\textbf{Endpoint Projection.}
%
In order to execute a choreography, we need to compile (translate) it to a
set of running processes that, run in parallel, enact the behaviour it
describes. Our procedure of compilation consists in two steps. The first
\emph{projects} the original choreography into a parallel composition of
partial single-process choreographies. The goal of this step is to have a set
of partial choreographies whose parallel composition behaves exactly as the
original one. Partial single-process choreographies will later ease the process
of compilation to a running language. Figs.~\ref{fig:preview_example_epp_A},
~\ref{fig:preview_example_epp_S}, and~\ref{fig:preview_example_epp_L}
respectively show the projection of the choreography in the example above ($C$)
on processes $\pid a$ ($\epp {C}{\pid a}$), $\pid s$ ($\epp{C}{\pid s}$), and
$\pid l$($\epp{C}{\pid l}$)\footnote{Processes $\pid a$, $\pid s$, and $\pid l$
all belong to $C_s$, therefore $\epp{C}{\pid a} =
\epp{C_s}{\pid a}$, $\epp{C_s}{\pid s} = \epp{C}{\pid s}$, and $\epp{C_s} {\pid
l} = \epp{C}{\pid l}$.}.

The EPP of $C$, $\epp{C}{} = \epp{C}{\pid c} \pp \epp{C}{\pid f} \pp \epp{C}
{\pid a} \pp \epp{C}{\pid s} \pp \epp{C}{\pid l}$, behaves exactly as $C$. This
results from the definition of the semantics of our model in which all complete
operations break into partials.

Below we highlight some salient parts of the projection and show that $C$ and
$\epp{C}{}$ behave accordingly.

Let $\wtil{l.\prc qB} = l_{\role A}.\prc aA,l_{\role S}.\prc sS,l_{\role
L}.\prc lL$, $\pid p \in \{\pid a, \pid s, \pid l\}$ and $\epp{C}{\pid p}'$
continuation of $\epp {C} {\pid p}$ after Line 1. The effect of the execution
of Line 1 of $\epp {C} {}$ is
%
{\footnotesize
$$
\hspace{-5pt}\begin{array}{l}
\env,\begin{array}{l}
\req{k_d}{\prc cC}{\wtil{l.\prc qB}}; \epp{C}{\pid c}' \pp %
\acc{k_d}{l_{\role A}.\prc aA}; \epp{C}{\pid a}' \pp \\
\acc{k_d}{l_{\role S}.\prc sS}; \epp{C}{\pid s}' \pp %
\acc{k_d}{l_{\role L}.\prc lL}; \epp{C}{\pid l}'		
\end{array}
\to
\\[10pt]
\env \seff \start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}},\ 
\epp{C}{\pid c}' \pp \epp{C}{\pid a}' \pp \epp{C}{\pid s}' \pp 
\epp{C}{\pid l}'		
\end{array} 
$$
}
%
Which is the same effect of the execution of Line 1 of $C$.

Complete communications project as partial sends and receives
between the two processes taking part in it. E.g., at Line 6 of $C_s$, $\pid s$
sends a message to $\pid l$ on operation $log$. The EPP of Line 6 of $C_s$
projects to the send at Line 4 of $\epp{C_s}{\pid s}$ and the reception at Line
2 of $\epp{C_s}{\pid l}$. As we already commented, the effect, at runtime, of
Line 6 of $C_s$ is that first $\pid s$ delivers its message to $\pid l$ and,
later on, $\pid l$ reads it. Line 4 of $\epp{C_s}{\pid s}$ and Line 2 of
$\epp{C_s}{\pid l}$ enact the same behaviour: first Line 4 executes
 and after the deliver Line 2 can execute.

The EPP preserves conditionals on the process evaluating it. For all the
other processes involved in the body of the conditional, the EPP projects a
branched reception. E.g., at Line 3 of $C_s$, process $\pid a$ evaluates a
condition that either branches in the behaviour at Lines 4-15 or Lines 17-19.
The condition evaluated at Line 3 of $C_s$ by process $\pid a$ is projected
verbatim at Line 3 of $\epp{C_s}{\pid a}$. The EPP of $\pid s$ projects a
branched communication on either operation $ok$ (Line 3) or $ko$ (Line 6 of
$\epp {C_s} {\pid s}$). The EPP of $\pid l$ projects only one branch (Line 2
of $\epp{C_s}{\pid l}$) as $\pid l$ receives on operation $log$ in either cases.

\textbf{Compilation.}
%
Once projected, we can compile the EPP of each process in the choreography to
a process of an executable language. To prove our translation sound we chose,
as target language of the compilation, an extended version of the Correlation
Calculus~\cite{MC11} (CC), the theoretical model behind the Jolie
language~\cite{jolie:website}.

Key elements of CC are \emph{services} and \emph{processes}. A service acts
as a deployment container. Each service is associated with a location,
contains a set of processes running in parallel, and can spawn new processes
at runtime on request. The form of a service is $S =\jsrv {B, P} {l}$, where
$B$ is the behaviour of spawnable processes, $P$ the parallel composition of
the running processes, and $l$ the deployment location. A process, with form
$\jprc{B}{t}{M}$, is associated with a behaviour $B$, a state $t$, and a set
of queues $M$.

CC handles communication via message passing. Messages are routed to
processes by means of correlation (matching) between a set of values
contained in the message and the values that identify a queue (just like
queues are identified by values in our choreographic model). In~\cite{MC11}
queues are static and assigned when a new process is created. To support the
runtime creation of new session, we present in this paper an extension of CC
that enables processes to create new queues at runtime.

In this way, we can translate the interactions on a session (in the original
choreography) into a set of message exchanges routed on the carried data. When
in the choreography a running process requests the creation of a new session,
we encode the request as the creation of a new set of data for correlation and
the relative queues pointed by that data. The result of our approach is that
the global knowledge on the state of the choreography, kept by the environment
$\env$, is distributed among the processes that result form the compilation of
the choreography.

\textbf{DIRE PERCHE' SERVE $\Gamma$ ALL'ENCODING} 

We write the encoding of a running choreography $\env,C$ as $\genenc{\env,C}{}$.
Informally, $\genenc{\env,C}{}$ compiles to a parallel composition services, one
for
each location in $C$. For each service $S = \jsrv{B,P}l$:
\emph{i}) let $\pid p$ be the process that offers to accept ($\textbf {acc}$)
a new session on $l$ in $C$, $$S = \jsrv{\genenc{\epp{C}{\pid p}},P}l$$. E.g.,
Figure~\ref{fig:preview_example_encoding_A} shows the encoding of the service
at $l_{\role A}$ and it exposes $\genenc{\epp{C_{s}}{\pid a}}$
to spawn new processes. A similar service is the one at $l_{\role L}$ in
Figure~\ref{fig:preview_example_encoding_L}.
\emph{ii}) for all running processes $\pid p_1, \ldots, \pid p_n$ located at
$l$ in $C$, $$S = \jsrv{B, \genenc{\epp{C}{\pid p_1}} \pp \ldots \pp
\genenc{\epp{C}{\pid p_n}}}{l}$$, i.e., it contains the parallel composition of
the compilation of the projection of $C$ on each process. E.g., let process
$\pid c$ in $C$ be located at $l_{\role C}$, the encoding of $C$ for $S$
located at $l_{\role C}$ is $S = \jsrv{B,P}{l_{\role C}}$ where $P =
\jprc{\genenc{\epp{C_{c}}{\pid c}}} {\env(\pid a).\estate}{\env(\pid
a).\equeues}$, i.e., $P$ is the encoding of the projection $\epp{C}{\pid c}$.
Note that the state and set of queues of $P$ are exactly the ones defined by
the environment $\env$ for $\pid a$.
Figure~\ref{fig:preview_example_encoding_C} shows an excerpt of the compilation
of the service at $l_{\role C}$.
%

Below we comment some salient parts of the compilation and show how $\genenc{C}
{}$ implements the runtime behaviour of $C$.

$\env' = \env \seff \start {k_d} {\pid c [\role C]} {\wtil {l.\prc qB}}$ is
the effect of starting a new session and it modifies $\env$ in such a way
that all involved processes in the start have the proper values set for
process-to-process communication (correlation) on $k_d$ along with the
corresponding queues. In $\genenc{C}{}$ we need to ensure the same behaviour in
a distributed setting. To do this, we compile the start of a new session to a
centralised synchronisation procedure. As a convention, we put in charge the
process running the $\textbf{req}$ for a new session of setting the values
and to work as the synchronisation point.

Figure~\ref{fig:preview_example_encoding_C} shows an excerpt of the compilation
of $\textbf{req}$: \emph{i}) Lines 1-2 set the location of the involved
processes. This data will be used later in send operations to address the
service of the receiver. \emph{ii}) Lines 3-5 assign fresh values ($\new$) to
the variables for correlation, following the convention
$\jpath{Session.Sender.Receiver}$. \emph{iii}) Lines 6-11 spawn the new
processes, one for each role (except the one played by the requester) in the
choreography. Lines 6-8 show the instructions for the process playing role
$\role A$. Line 6 sets the queue of the requester to receive messages from
$\role A$. Line 7 requests to the service at $l_{\role A}$ to spawn a new
process. Line 8 waits to receive a message on operation $sync$ from the new
process playing role $\role A$, i.e., on its queue pointed by
$\jpath{kd.A.C}$. \emph{iv}) Finally, Lines 12-14 notify all (new) processes
to start running the session.

The compilation of $\textbf{acc}$ is the complementary to
$\textbf{req}$. Let us look at the compilation of Line 1 of $\epp{C_s}{\pid
a}$ (Figure~\ref{fig:preview_example_epp_A}) shown at Lines 1-6 of
Figure~\ref{fig:preview_example_encoding_A}. At Line 1 $\oneway{!}{\jpath{kd}}$
accepts the request to spawn a new process. Then (Lines 2-4) the process sets
its queues to receive, on session $k_d$, from resp. $\role C$, $\role S$, and
$\role L$. Finally, it notifies the starter (at $\jpath{kd.C.l}$) it is
ready to begin the session (Line 5) and waits to be notified on operation
$start$ (Line 6).

Apart from the start procedure, the code of a compiled process and its EPP
are very similar. Indeed, the main difference between the EPP and the
compilation is that, whilst in the choreography communications happen through
a session, in the compiled code we make explicit reference to the
data-structures used to address services and communicate on queues. E.g., let
us compare Figs.~\ref{fig:preview_example_epp_A}
and~\ref{fig:preview_example_encoding_A}, below respectively addressed as the
EPP and compilation of $\pid a$. Lines 3-9 of the EPP translate, one-by-one,
to Lines 7-14 of the compilation. We briefly comment a reception and a send
operation. The reception at Line 2 of the EPP compiles to Line 7 of
Figure~\ref{fig:preview_example_encoding_A}. $\oneway{get}{\jpath{req}}
\qfrom{\jpath{kd.C.A}}$ reads a message for operation $get$
from the queue pointed by $\jpath{kd.C.A}$ and assigns its content to
variable $\jpath{req}$. The send operation at Line 4 of the EPP translates to
$\notify{ok}{\jpath{kd.S.l}}{\jpath{req.rsc}} \qto{\jpath{kd.A.S}}$ (Line 9
of the compilation) which sends the content of $\jpath{req.rsc}$ to the
process located at $\jpath{kd.S.l}$ that correlates with $\jpath{kd.A.S}$.

% \begin{itemize}
% 	\item e' il linguaggio eseguibile
% 	\item richiede piu' passi
%   \item le session sono state tradotte in code e correlazione;
% 	\item e' importante far notare che ogni processo nei servizi non fa altro che
% 	contenere un pezzo dell'environment.
% 	\item far vedere che la start crea le stesse code e gli stessi dati
% 	dell'environment ma in servizi e processi diversi
% \end{itemize}
%
%\textbf{Implementations as Applied Choreographies.}
%%
%Choreography programming[CITATION NEEDED] is a development model to implement
%protocols from a global point of view. Key elements of choreographies are
%\emph{sessions} and \emph{processes}. A session is an instance of a protocol.
%It implements the communications among the processes taking part in it. A
%process represents an entity that executes a sequence of instructions.
%Processes can be programmed as already running or dynamically created at
%runtime. Processes can create new sessions.
%
%In this work, we introduce other two key-elements: the \emph{environment}
%($\env$) and the locations $l_1,\ldots,l_n$. $\env$ is a global structure
%that contains the state of the processes in a choreography. We call the
%couple $\env,C$ a \emph {running choreography}.
%
%\textbf{The Environment.}
%The reason for introducing $\env$ is threefold: \emph{i}) $\env$ allows to
%clearly define how correlation works by keeping track of the evolution of its
%companion choreography; \emph{ii}) we use $\env$ to ease the process of
%compilation from a choreography to a set of processes and
%\emph{iii}) to prove that a choreography and its compilation behave
%accordingly. Indeed we prove that, for any evolution of the choreography, the
%information (processes, states, and queues) in $\env$ is the same as the
%union of the local information in the compilation.
%
%Figure~\ref {fig:E} depicts the structure of $\env$. For each process in a
%choreography $C$, $\env$ contains the location of all processes $\pid
%p_1\,\ldots,\pid p_n$ in $C$, their state ($\estate$) and their set of queues
%($\equeues$). $\env$ identifies a specific queue of a process with a set of
%values, i.e., let $\pid p$ be a process in $\env$, $\env(\pid p).\equeues$ is
%a partial function that given a set of values $t$ ($t \in
%\m{dom}(\env(\pid p).\equeues)$) returns a queue of messages $\til m$.
%
%\textbf{Locations and Public Channels}
%
%\textbf{BOZZA, SCRIVERE MEGLIO!!!}
%
%A standard practice of Choreography Programming and Session Types is to model the creation of a new session between different processes via \emph{public channels} typed by a global type. Locations in our model are similar to public channels, but they only support one local type, i.e., the behaviour of one of the roles of a global type. However, the (lexicographic) union of a set of locations can be typed by a global type.
%
%Given a typing environment $\Gamma$, a global type $G$, and sequence of
%locations $\til l$, $\til l$ has type $G$ in $\Gamma$ if, for all roles in $G$, there exists $l \in \til l$ whose local type is the type of role $\role R$ in $G$.
%
%Let $C = C_c \pp C_s$ parallel composition of the two partial choreographies $C_c$ and $C_s$, resp. in Figs.~\ref{fig:preview_example_client} and~\ref{fig:preview_example_server}. Let $l_{\role C}$ be the location of process $\pid c$ in Figure~\ref{fig:preview_example_client}. The sequence of locations $l_{\role C},l_{\role A},l_{\role S},l_{\role L}$ and $l_{\role C}, l_{\role F}$ respectively implement the global types $G_d$ and $G_s$.
%
%Below we comment the salient runtime behaviours of $\env,C$.
%
%\textbf{Starting of a new session: correlation and queues.}
%%
%The interaction between of the first two statements (Line 1) of $C_c$ and
%$C_s$ spawns a new session (we named the session $k_d$ for convenience). At
%Line 1 of $C_c$ process $\pid c$, playing role $\role C$, requests to create
%a new session with some new processes at locations $l_{\role A}$, $l_{\role
%S}$, and $l_{\role L}$. Line 1 of $C_s$ matches the request with the newly
%created processes $\pid a$ (playing $\role A$, running at $l_{\role A}$),
%$\pid s$ (playing $\role S$, running at $l_{\role S}$), and $\pid l$ (playing
%$\role L$, running at $l_{\role L}$). Let $\wtil{l.\prc qB} = l_{\role
%A}.\prc aA,l_{\role S}.\prc sS,l_{\role L}.\prc lL$, and $C_c'$ and $C_s'$
%continuation of respectively $C_c$ and $C_s$ after Line 1. $E,C$ reduces to
%%
%$$
%\hspace{-.5em}\begin{array}{l}
%\env,
%\req{k_d}{\prc cC}{\wtil{l.\prc qB}}; C_c' 
%	\pp
%	\acc{k_d}{\wtil{l.\prc qB}}; C_s'		
%\to
%\\
%\env \seff 
%\start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}}, C_c' \pp C_s'		
%\end{array}	
%$$
%%
%$\env' = \env \seff \start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}}$ means
%that $\env$ records the effect of the interaction:
%
%\emph{i}) $\env'$ stored the new processes $\pid a$, $\pid s$, and $\pid l$ with
%no queues
%%
%$$\env'(\pid a).\equeues = \env'(\pid s).\equeues = \env'(\pid l).\equeues =
%\emptyset$$
%%
%and empty states
%%
%$$\env'(\pid a).\estate = \env'(\pid s).\estate = \env'(\pid l).\estate = t_\bot$$
%%
%$t_\bot$ being the empty state.
%\emph{ii}) The state of all processes in the session is updated with the
%values used for correlation. Each couple of processes in the session owns a
%couple of values used to send and receive messages. By convention, we store
%correlating values following the syntax $\jpath{Session.Sender.Receiver}$.
%E.g, process $\pid a$ and $\pid c$, respectively playing roles $\role A$ and
%$\role C$ in session $k_d$, use the correlation data in $\jpath{kd.A.C}$ to
%send (resp. receive) messages. Indeed, the value of $\jpath{kd.A.C}$ is the
%same, both evaluated against the state of $\pid a$ and $\pid c$. Let $t =
%\env'(\pid a).\estate$, $t' = \env'(\pid c).\estate$, resp. states of $\pid a$ and
%$\pid c$, $\jpath{kd.A.C}(t) = \jpath{kd.A.C}(t')$. 
%%
%The same holds also for $\jpath {kd.C.A}$ and for every couple of processes
%(roles) in session $k_d$.
%\emph{iii}) For each correlation value of the kind
%$\jpath{Session.Sender.Receiver}$, the process playing role $\jpath
%{Receiver}$ has in $\env'$ an empty queue pointed by that value. E.g., $\pid a$
%(playing $\role A$) has three new empty queues mapped by $\jpath{kd.C.A}$,
%$\jpath {kd.S.A}$, and $\jpath{kd.L.A}$.
%
%\textbf{Message passing.}
%%
%
%\textbf{METTERE UN RIFERIMENTO AL TIPO!!!}
%
%Line 2 of $C_c$ and $C_s$ respectively represent send and receive (partial)
%operations. At Line 2 of $C_c$, $\com{k_d}{\prc cC.\m{mkReq()}}{\role A.get}$,
%means that through session $k_d$, $\pid c$ (playing role $\role C$), sends the
%result of the evaluation of function $\m{mkReq()}$ on operation $get$ to the
%external process that plays role $\role A$. Note that $C_c$ does not specify
%the name of the process playing $\role A$. The name has to be defined by the
%complementary partial choreography that implements the process playing
%$\role A$ ($C_s$). Below we report the reduction steps of the communication
%($C_c'$ and $C_s'$ continuations of resp. $C_c$ and $C_s$ after Line 2).
%%
%{\scriptsize
%$$
%\hspace{-.5em}\begin{array}{l}
%	\env,\ \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get};C_c' \pp
%			 \com{k_d}{\role C}{\prc aA.get(\jpath{req})};C_s'
%	\to
%	\\
%	\env\ \seff \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get},\ C_c' \pp
%			 \com{k_d}{\role C}{\prc aA.get(\jpath{req})};C_s'
%	\to
%	\\
%	\env' \seff \com{k_d}{\role C}{\prc aA.get(\jpath{req})},\ C_c' \pp C_s'
%\end{array}
%$$
%}
%%
%First $\pid c$ sends the message to the process playing $\role A$. The effect
%of $\env' = \env\ \seff \com{k_d}{\prc cC.\m{mkReq()}}{\role A.get}$ is that
%$\env'$ stored a new message in the queue pointed by $\jpath {kd.C.A.c}$ of
%process $\pid a$. The content of the message is the evaluation of $\m{mkReq
%()}$ on the state of $\pid c$. We remark that the effect does not need to
%carry the identity of $\pid a$ in $C$. $\env$ can guess it from the
%correlation data used by $\pid c$. The intention behind this choice is that
%it will ease the process of compilation, as it exploits the same technique
%used to route messages in the target language of compilation.
%
%Then process $\pid a$ reads the message from $\role C$ for operation $get$,
%in the queue pointed by $\jpath {kd.C.A}$. The effect of $\env' \seff
%\com{k_d}{\role C}{\prc aA.get(\jpath{req})}$ removes the message from the
%queue and assigns its content to variable $\jpath{req}$ in the state of $\pid
%a$.
%
%\textbf{Asynchrony.}
%%
%One of the benefits of including the environment in our model is that it
%makes message passing inherently asynchronous. Indeed, in the example above
%the two instructions at Line 2 of $C_c$ and $C_s$ are asynchronous. E.g.,
%$\pid c$ may have already delivered the message and passed to the next
%instruction, whilst $\pid a$ still had to reach Line 2 and read the message.
%This holds also for complete operations in our semantics. They first reduce
%to a send and then execute a reception.
%
%This means that, even if a choreography defines a certain order in which its
%processes shall receive (read) their messages, this order can change at
%runtime. This is actually what happens in real-world distributed system.
%Messages (data) are consumed according to the state of computation of each
%process. Our model naturally matches this feature.
%
%The execution of Lines 4-5 of $C_s$ show this concept (we omit
%effects on $\env$ for brevity, $C_s'$ continuation of $C_s$ after Line 5):
%%
%{\footnotesize
%$$
%\hspace{-.5em}\begin{array}{l}
% \env, \com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ok(\jpath{rsc})};
%\com{k_d}{\prc aA}{\role C.ok};C_s'\pp C_c
%\to
%\\ \env', \com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};
%\com{k_d}{\prc aA}{\role C.ok};C_s'\pp C_c
%\swapC
%\\ \env', \com{k_d}{\prc aA}{\role C.ok};\com{k_d}{\role A}{\prc
%sS.ok(\jpath{rsc})};C_s'\pp C_c
%\to
%\\ \env'', \com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};C_s'\pp C_c
%\end{array}
%$$
%}
%%
%After $\pid a$ sent its message to $\pid s$, it is possible
%that $\pid s$ is not ready to read it (e.g., due to scheduling). In our
%model, we allow two operations to swap if they have no process in common.
%Operations $\com{k_d}{\role A}{\prc sS.ok}$ and $\com{k_d}{\prc aA}{\role
%C.ok}$ regard resp. $\pid s$ and $\pid a$ and can swap. We indicate swapping
%with $\swapC$. After the swap, $\pid a$ delivers its message to $\role C$.
%
%Another example of asynchrony are Lines 9-10 of $C_s$. $\pid s$ can send all
%the sequence of packets of the file to $\pid c$, whilst $\pid c$ might have
%read none of them yet. The queue between them works as a buffer.
%
%Remarkably, although allowing for asynchrony, our type system guarantees to
%preserve the order of interactions, i.e., the order two processes
%send and receive messages to and from each other.
%
%\textbf{Parallelism.}
%%
%Our model also automatically achieves the maximum degree of parallelism among
%different processes.
%
%Lines 4-6 of $C_s$ show an example of that. 
%%Above, we commented that receptions
%%and reads are asynchronous. E.g., the read at Line 4 ($\pid s$ reads the
%%message for operation $ok$) can execute later than the read at Line 5 ($\role
%%C$ reads the message for $ok$). 
%The instructions at Lines 5-6 concern a disjoint set of processes (resp. $\pid
%a$, $\pid s$, and $\pid l$). According to our model the two instructions can
%swap, thus their order of execution is non-deterministic. A possible reduction
%is (effect on $\env$ omitted for brevity, $C_s'$ continuation of $C_s$ after
%Line 6):
%%
%{\scriptsize
%$$
%\hspace{-.5em}\begin{array}{ll}
%\hspace{-.5em}\begin{array}{l}
%	\env, \begin{array}{l}
%		\com{k_d}{\prc aA.\jpath{req.rsc}}{\prc sS.ok(\jpath{rsc})};
%	  \com{k_d}{\prc aA}{\role C.ok};
%	  \\
%		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
%		C_s' \pp C_c	
%	\end{array}
%\end{array}
%\to
%\\[7pt]
%\hspace{-.5em}\begin{array}{l}
%	\env', \begin{array}{l}
%		\com{k_d}{\role A}{\prc sS.ok(\jpath{rsc})};
%	  \com{k_d}{\prc aA}{\role C.ok};
%	  \\
%		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
%		C_s' \pp C_c	
%	\end{array}
%\end{array}
%\to
%\\[7pt]
%\env'',
%	  \com{k_d}{\prc aA}{\role C.ok};
%		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
%		C_s' \pp C_c	
%\swapC
%\\[3pt]
%\env'',
%		\com{k_d}{\prc sS.\m{logok}(\jpath{rsc})}{\prc lL.log(\jpath{log})};
%	  \com{k_d}{\prc aA}{\role C.ok};
%		C_s' \pp C_c	
%\to
%\\[3pt]
%\env''',
%		\com{k_d}{\role S}{\prc lL.log(\jpath{log})};
%	  \com{k_d}{\prc aA}{\role C.ok};
%		C_s' \pp C_c	
%\swapC
%\\[3pt]
%\env''',
%	  \com{k_d}{\prc aA}{\role C.ok};
%		\com{k_d}{\role S}{\prc lL.log(\jpath{log})};
%		C_s' \pp C_c	
%\to \ldots
%\end{array}
%$$
%}
%
%After $\pid a$ sent its message, let us suppose that $\pid s$ reads it. Then,
%since no process is shared between the instructions at Lines 5 and 6, it is
%possible to swap them. Then $\pid s$ sends its message to $\pid l$, the two
%Lines can swap again, and proceed with e.g., $\pid a$ delivering its message.
%Indeed, there are other possible execution scenarios, all permitted by our
%model.
%
%\textbf{Endpoint Projection.}
%%
%In order to execute a choreography, we need to compile (translate) it to a
%set of running processes that, run in parallel, enact the behaviour it
%describes. Our procedure of compilation consists in two steps. The first
%\emph{projects} the original choreography into a parallel composition of
%partial single-process choreographies. The goal of this step is to have a set
%of partial choreographies whose parallel composition behaves exactly as the
%original one. Partial single-process choreographies will later ease the
%process of compilation to a running language.
%Figs.~\ref{fig:preview_example_epp_A}, ~\ref{fig:preview_example_epp_S},
%and~\ref{fig:preview_example_epp_L} respectively show the projection of the
%choreography in the example above ($C$) on processes $\pid a$ ($\epp {C}{\pid
%a}$), $\pid s$ ($\epp{C}{\pid s}$), and $\pid l$($\epp{C}{\pid
%l}$)\footnote{Processes $\pid a$, $\pid s$, and $\pid l$ all belong to $C_s$,
%therefore $\epp{C}{\pid a} =
%\epp{C_s}{\pid a}$, $\epp{C_s}{\pid s} = \epp{C}{\pid s}$, and $\epp{C_s} {\pid
%l} = \epp{C}{\pid l}$.}.
%
%The EPP of $C$, $\epp{C}{} =
%\epp{C}{\pid c} \pp \epp{C}{\pid f} \pp \epp{C}{\pid a} \pp \epp{C}{\pid s}
%\pp \epp{C}{\pid l}$, behaves exactly as $C$. This results from the
%definition of the semantics of our model in which all complete
%operations break into partials.
%
%Below we highlight some salient parts of the projection and show that $C$ and
%$\epp{C}{}$ behave accordingly.
%
%Let $\wtil{l.\prc qB} = l_{\role A}.\prc aA,l_{\role S}.\prc sS,l_{\role
%L}.\prc lL$, $\pid p \in \{\pid a, \pid s, \pid l\}$ and $\epp{C}{\pid p}'$
%continuation of $\epp {C} {\pid p}$ after Line 1. The effect of the execution
%of Line 1 of $\epp {C} {}$ is
%%
%{\footnotesize
%$$
%\hspace{-5pt}\begin{array}{l}
%\env,\begin{array}{l}
%\req{k_d}{\prc cC}{\wtil{l.\prc qB}}; \epp{C}{\pid c}' \pp %
%\acc{k_d}{l_{\role A}.\prc aA}; \epp{C}{\pid a}' \pp \\
%\acc{k_d}{l_{\role S}.\prc sS}; \epp{C}{\pid s}' \pp %
%\acc{k_d}{l_{\role L}.\prc lL}; \epp{C}{\pid l}'		
%\end{array}
%\to
%\\[10pt]
%\env \seff \start{k_d}{\pid c[\role C]}{\wtil{l.\prc qB}},\ 
%\epp{C}{\pid c}' \pp \epp{C}{\pid a}' \pp \epp{C}{\pid s}' \pp 
%\epp{C}{\pid l}'		
%\end{array} 
%$$
%}
%%
%Which is the same effect of the execution of Line 1 of $C$.
%
%Complete communications project as partial sends and receives
%between the two processes taking part in it. E.g., at Line 6 of $C_s$, $\pid s$
%sends a message to $\pid l$ on operation $log$. The EPP of Line 6 of $C_s$
%projects to the send at Line 4 of $\epp{C_s}{\pid s}$ and the reception at Line
%2 of $\epp{C_s}{\pid l}$. As we already commented, the effect, at runtime, of
%Line 6 of $C_s$ is that first $\pid s$ delivers its message to $\pid l$ and,
%later on, $\pid l$ reads it. Line 4 of $\epp{C_s}{\pid s}$ and Line 2 of
%$\epp{C_s}{\pid l}$ enact the same behaviour: first Line 4 executes
% and after the deliver Line 2 can execute.
%
%The EPP preserves conditionals on the process evaluating it. For all the
%other processes involved in the body of the conditional, the EPP projects a
%branched reception. E.g., at Line 3 of $C_s$, process $\pid a$ evaluates a
%condition that either branches in the behaviour at Lines 4-15 or Lines 17-19.
%The condition evaluated at Line 3 of $C_s$ by process $\pid a$ is projected
%verbatim at Line 3 of $\epp{C_s}{\pid a}$. The EPP of $\pid s$ projects a
%branched communication on either operation $ok$ (Line 3) or $ko$ (Line 6 of
%$\epp {C_s} {\pid s}$). The EPP of $\pid l$ projects only one branch (Line 2
%of $\epp{C_s}{\pid l}$) as $\pid l$ receives on operation $log$ in either cases.
%
%\textbf{Compilation.}
%%
%Once projected, we can compile the EPP of each process in the choreography to
%a process of an executable language. To prove our translation sound we chose,
%as target language of the compilation, an extended version of the Correlation
%Calculus~\cite{MC11} (CC), the theoretical model behind the Jolie
%language~\cite{jolie:website}.
%
%Key elements of CC are \emph{services} and \emph{processes}. A service acts
%as a deployment container. Each service is associated with a location,
%contains a set of processes running in parallel, and can spawn new processes
%at runtime on request. The form of a service is $S =\jsrv {B, P} {l}$, where
%$B$ is the behaviour of spawnable processes, $P$ the parallel composition of
%the running processes, and $l$ the deployment location. A process, with form
%$\jprc{B}{t}{M}$, is associated with a behaviour $B$, a state $t$, and a set
%of queues $M$.
%
%CC handles communication via message passing. Messages are routed to
%processes by means of correlation (matching) between a set of values
%contained in the message and the values that identify a queue (just like
%queues are identified by values in our choreographic model). In~\cite{MC11}
%queues are static and assigned when a new process is created. To support the
%runtime creation of new session, we present in this paper an extension of CC
%that enables processes to create new queues at runtime.
%
%In this way, we can translate the interactions on a session (in the original
%choreography) into a set of message exchanges routed on the carried data. When
%in the choreography a running process requests the creation of a new session,
%we encode the request as the creation of a new set of data for correlation and
%the relative queues pointed by that data. The result of our approach is that
%the global knowledge on the state of the choreography, kept by the environment
%$\env$, is distributed among the processes that result form the compilation of
%the choreography.
%
%\textbf{DIRE PERCHE' SERVE $\Gamma$ ALL'ENCODING} 
%
%We write the encoding of a running choreography $\env,C$ as $\genenc{\env,C}{}$.
%Informally, $\genenc{\env,C}{}$ compiles to a parallel composition services, one
%for
%each location in $C$. For each service $S = \jsrv{B,P}l$:
%\emph{i}) let $\pid p$ be the process that offers to accept ($\textbf {acc}$)
%a new session on $l$ in $C$, $$S = \jsrv{\genenc{\epp{C}{\pid p}},P}l$$. E.g.,
%Figure~\ref{fig:preview_example_encoding_A} shows the encoding of the service
%at $l_{\role A}$ and it exposes $\genenc{\epp{C_{s}}{\pid a}}$
%to spawn new processes. A similar service is the one at $l_{\role L}$ in
%Figure~\ref{fig:preview_example_encoding_L}.
%\emph{ii}) for all running processes $\pid p_1, \ldots, \pid p_n$ located at
%$l$ in $C$, $$S = \jsrv{B, \genenc{\epp{C}{\pid p_1}} \pp \ldots \pp
%\genenc{\epp{C}{\pid p_n}}}{l}$$, i.e., it contains the parallel composition of
%the compilation of the projection of $C$ on each process. E.g., let process
%$\pid c$ in $C$ be located at $l_{\role C}$, the encoding of $C$ for $S$
%located at $l_{\role C}$ is $S = \jsrv{B,P}{l_{\role C}}$ where $P =
%\jprc{\genenc{\epp{C_{c}}{\pid c}}} {\env(\pid a).\estate}{\env(\pid
%a).\equeues}$, i.e., $P$ is the encoding of the projection $\epp{C}{\pid c}$.
%Note that the state and set of queues of $P$ are exactly the ones defined by
%the environment $\env$ for $\pid a$.
%Figure~\ref{fig:preview_example_encoding_C} shows an excerpt of the compilation
%of the service at $l_{\role C}$.
%%
%
%Below we comment some salient parts of the compilation and show how $\genenc{C}
%{}$ implements the runtime behaviour of $C$.
%
%$\env' = \env \seff \start {k_d} {\pid c [\role C]} {\wtil {l.\prc qB}}$ is
%the effect of starting a new session and it modifies $\env$ in such a way
%that all involved processes in the start have the proper values set for
%process-to-process communication (correlation) on $k_d$ along with the
%corresponding queues. In $\genenc{C}{}$ we need to ensure the same behaviour in
%a distributed setting. To do this, we compile the start of a new session to a
%centralised synchronisation procedure. As a convention, we put in charge the
%process running the $\textbf{req}$ for a new session of setting the values
%and to work as the synchronisation point.
%
%Figure~\ref{fig:preview_example_encoding_C} shows an excerpt of the compilation
%of $\textbf{req}$: \emph{i}) Lines 1-2 set the location of the involved
%processes. This data will be used later in send operations to address the
%service of the receiver. \emph{ii}) Lines 3-5 assign fresh values ($\new$) to
%the variables for correlation, following the convention
%$\jpath{Session.Sender.Receiver}$. \emph{iii}) Lines 6-11 spawn the new
%processes, one for each role (except the one played by the requester) in the
%choreography. Lines 6-8 show the instructions for the process playing role
%$\role A$. Line 6 sets the queue of the requester to receive messages from
%$\role A$. Line 7 requests to the service at $l_{\role A}$ to spawn a new
%process. Line 8 waits to receive a message on operation $sync$ from the new
%process playing role $\role A$, i.e., on its queue pointed by
%$\jpath{kd.A.C}$. \emph{iv}) Finally, Lines 12-14 notify all (new) processes
%to start running the session.
%
%The compilation of $\textbf{acc}$ is the complementary to
%$\textbf{req}$. Let us look at the compilation of Line 1 of $\epp{C_s}{\pid
%a}$ (Figure~\ref{fig:preview_example_epp_A}) shown at Lines 1-6 of
%Figure~\ref{fig:preview_example_encoding_A}. At Line 1 $\oneway{!}{\jpath{kd}}$
%accepts the request to spawn a new process. Then (Lines 2-4) the process sets
%its queues to receive, on session $k_d$, from resp. $\role C$, $\role S$, and
%$\role L$. Finally, it notifies the starter (at $\jpath{kd.C.l}$) it is
%ready to begin the session (Line 5) and waits to be notified on operation
%$start$ (Line 6).
%
%Apart from the start procedure, the code of a compiled process and its EPP
%are very similar. Indeed, the main difference between the EPP and the
%compilation is that, whilst in the choreography communications happen through
%a session, in the compiled code we make explicit reference to the
%data-structures used to address services and communicate on queues. E.g., let
%us compare Figs.~\ref{fig:preview_example_epp_A}
%and~\ref{fig:preview_example_encoding_A}, below respectively addressed as the
%EPP and compilation of $\pid a$. Lines 3-9 of the EPP translate, one-by-one,
%to Lines 7-14 of the compilation. We briefly comment a reception and a send
%operation. The reception at Line 2 of the EPP compiles to Line 7 of
%Figure~\ref{fig:preview_example_encoding_A}. $\oneway{get}{\jpath{req}}
%\qfrom{\jpath{kd.C.A}}$ reads a message for operation $get$
%from the queue pointed by $\jpath{kd.C.A}$ and assigns its content to
%variable $\jpath{req}$. The send operation at Line 4 of the EPP translates to
%$\notify{ok}{\jpath{kd.S.l}}{\jpath{req.rsc}} \qto{\jpath{kd.A.S}}$ (Line 9
%of the compilation) which sends the content of $\jpath{req.rsc}$ to the
%process located at $\jpath{kd.S.l}$ that correlates with $\jpath{kd.A.S}$.
%
% \begin{itemize}
% 	\item e' il linguaggio eseguibile
% 	\item richiede piu' passi
%   \item le session sono state tradotte in code e correlazione;
% 	\item e' importante far notare che ogni processo nei servizi non fa altro che
% 	contenere un pezzo dell'environment.
% 	\item far vedere che la start crea le stesse code e gli stessi dati
% 	dell'environment ma in servizi e processi diversi
% \end{itemize}



==> projection.tex <==
%auto-ignore
We now present the Endpoint Projection and its properties.
%
The EPP returns a correct composition\footnote{Here and in the following
``composition'' means ``parallel composition''.} of endpoint choreographies
that implements the behaviour of a given choreography. Intuitively, an endpoint
choreography is a choreography that does not contain complete actions.
Formally, let $\fp(C)$ return the set of free processes in a choreography
$C$:
%
\begin{definition}[Endpoint Choreography] We say that a
choreography $C$ is an endpoint choreography if $C$ does not contain complete
actions and one of the two following conditions holds:
$i)\ C = \acc{k}{{l.\pid q[\role B]}}; C' \wedge \{ \pid q \} = \fp(C');$
$ii)\ \fp(C) = \{\pid p\}$.
\end{definition}

\input{figures/projection}

An endpoint choreography defines the identity of only one process: either $i)$
a service process or $ii)$ an active process. Notably, our definition of EPP
captures the description of the behaviour of single endpoints up to complete
choreographies.
%
To give the definition of the EPP of a choreography, we first define the
notion of \emph{process projection}, which defines the behaviour of a single
process $\pid p$ in a choreography $C$, written $\epp{C}{\pid p}^{\mathbb{X}}$.
%
Intuitively, the process projection follows the structure of the originating
choreography, where $\mathbb{X}$, often omitted, is an auxiliary structure to
keep track of the procedure names where the process $\pid p$, on which we are
performing the projection, takes part.

%
A $\prid{start}$ projects to a $\prid{req}$ on the active process and a set of
$\prid{acc}$ terms on the service processes. Likewise, a $\prid {com}$
projects to a partial $\prid{send}$ for the sender and a partial $\prid{recv}$
for the receiver. Any partial term is projected as it is for its respective
process, following the structure of the choreography. We report in
\cref{fig:cc_projection} the rules for process projection. Note in
particular the projections of $\prid {recv}$ and $\prid{cond}$ terms, which
use the \emph{merging} partial operator $\sqcup$~\cite{CHY12} to merge the
behaviour of all processes in their branches.

% \noindent{\footnotesize$
% \begin{array}l
% \genproj{\gencom ; C} = \\ \qquad
% \begin{cases}
% 	\gensend ; \genproj{C} &
% 		\mbox{if } \pid r = \pid p
% 	\\
% 	\genrecv ; \genproj{C} &
% 		\mbox{if } \pid r = \pid q
% 	\\
% 	\genproj{C} & \mbox{otherwise}
% \end{cases}
% \end{array}
% \qquad
% \begin{array}l
% \genproj{\gencond} = \\ \qquad 
% \begin{cases}
% 		\cond{\pid p.e}{\epp{C_1}{\pid r}}{\epp{C_2}{\pid r}} & 
% 		\mbox{if } \pid r =	\pid p
% 		\\
% 		\genproj{C_1} \sqcup \genproj{C_2} & \mbox{otherwise}
% 	\end{cases}
% 	\\ \vphantom{-}
% \end{array}
% $}\smallskip

$C \sqcup C'$ is defined, in \cref{fig:merging_function}, only for
endpoint choreographies and returns an endpoint choreography
isomorphic to $C$ and $C'$ up to branching, i.e., with all branches on distinct
operations.
 
\input{figures/merging_function}

% \smallskip\noindent{\footnotesize
% $
% \hspace{-5pt}
% \begin{array}l
% 	\com{k}{\role A}{\prc{p}{B}.\left\{ o_i(x_i); C_i \right\}_{i \in I} }
% 		\; \sqcup \\ \qquad
% 	\com{k}{\role A}{\prc{q}{B}.\left\{ o_j(x_j); C'_j \right\}_{j \in J} }
% \end{array}
% 	= \quad
% 	\com{k}{\role A}{\prc{p}{B}.
% 		\left\{
% 			\begin{array}c
% 				\{\ o_i(x_i) ; C_i\ \}_{i \in I/J}\quad \cup \quad
% 				\{\ o_i(x_i) ; C'_i\ \}_{i \in J/I}\\[5pt]
% 				\cup \quad \{o_i(x_i) ; C_i \sqcup C'_i\}_{i \in I\cap J}
% 			\end{array}
% 		\right\}
% 	}
% $}\smallskip

%
On the definition of process projection, we define the EPP of a whole system.
Here, and in the following, $\group{C}{l}$ is the grouping operator that
returns the set of grouped (bound) service processes at the same location. We
report the definition of the grouping function in \cref{fig:grouping}.

% We
% show only the rules of $\group{C}{l}$ for $\prid {start}$ and $\prid{acc}$ as
% the other rules are trivially recursive applications.

\input{figures/grouping}


% \noindent{\footnotesize
% $
% \group{\start{k}{\pid p[\role D]}{\wtil{l.\pid q[\role B]}};C}{l} =
% \group{\genacc;C}{l}
% \quad\;
% \group{ \genacc;C }{l} =
% 	\begin{cases}
% 		\{\pid r\} \cup \group{C}{l}
% 			& \mbox{if } l.\pid r[\role A] \in \wtil{l.\pid q[\role B]}
% 		\\
% 		\group{C}{l} & \mbox{otherwise}
% 	\end{cases}
% $
% }

%
\begin{definition}[Endpoint Projection\label{def:epp}] Let $C$ be a term of AC.
The endpoint projection of $C$, denoted by $\proj{C}{}$, is defined as:
$
\proj{C}{} =
	\prod\limits_{\pid p \ \in \ \fp(C)} \proj{C}{\pid p }^{\emptyset} \pp
	\prod\limits_{l} \left( \bigsqcup\limits_{\pid p \ \in \ \group{C}{l}}
		\proj{C}{\pid p}^{\emptyset} \right)
$.
\end{definition}
%
The EPP of a choreography $C$ is the composition of the projections
of all active processes and the merged projections of the service
processes in $C$.

% \input{examples/projection_example}

\smallpar{Properties of EPP.}
\label{sub:epp_properies}
%
We give an extended presentation of the properties of EPP presented in
\cref{sec:compiler}, in particular we separate the properties of
\cref{thm:epp} in \cref{thm:EPP_typing_preservation} for a
simpler treatment.

We prove that the EPP implements the same behaviour of its originating
choreography, we build on the foundation that the EPP of a choreography is
still typable and then we establish a bisimilarity relation between the
semantics of the EPP and the originating choreography.

First we state our type preservation result using the \emph{minimal typing} of
choreographies $\seq_{\m{min}}$, which types the branches in rules $\did{T}
{Send}$ and $\did{T}{Recv}$ using the respective minimal branch types (reported
in \cref{fig:minimal_typing}). As in~\cite{CM13}, $\seq_{\m{min}}$ takes
into account that, due to merging, the EPP of a complete choreography may still
offer branches that the originating choreography discarded with a conditional.
Thus we have:
%
\begin{theorem}[EPP Typing Preservation\label{thm:EPP_typing_preservation}]
$\Gamma \hlseqmin{\env,C} \mbox{ implies } \epp{\Gamma}{} \hlseqmin{\env,\epp
{C}{}}$.
\end{theorem}
%
Where $\epp{\Gamma}{}$ replaces the typings of recursive procedures in $\Gamma$
with the typing of each procedure for each endpoint process taking part in it.

Combining the above Theorem with \cref{thm:session_fidelity} we can
prove:
%
\begin{theorem}[EPP Operational Correspondence\label{thm:epp_appendix}]
Let $\env,C$ be well-typed. Then,
\begin{enumerate}
\item (Completeness) $\env,C \to \env',C'$ implies $\env,\epp{C}{} \to
	\env',C''$ and $\epp{C'}{} \prec C''$.
\item (Soundness) $\env,\epp{C}{} \to \env',C'$ implies $\env,C \to \env',C''$
	and $\epp{C''}{} \prec C'$.
\end{enumerate}
\end{theorem}
In the theorem above $C \prec C'$ is the \emph{pruning relation}, a strong
typed bisimilarity~\cite{CHY12} such that $C$ has some unused branches
and always-available accepts.

==> proofs.tex <==
%auto-ignore

Below, we report proof sketches of our theorems.

Full proofs of Endpoint Projection and Compilation are reported
in~\cite{AC:tr}. The proof the typing system follows that of the choreography
calculus reported in \cite{AC:tr}, from which we took inspiration for the typing system for FC.

\subsubsection{Proofs of Subject Reduction and Session Fidelity}

To prove Subject Reduction and Session Fidelity, we use an annotated semantics
for FCs, ranging over labels with $\beta$, to mark transitions with the name
of the session whose term has reduced and with $\tau$ all other actions. We
also annotate the semantics of Global Types, ranging over label with $\gamma$,
to mark if the reduction happens on a ``send'' $\gcom{\role A}{\role B}{o}$ or
an a reception $\grecv {\role A} {\role B} {o}$.

Then we define a subtyping relation on local types
following~\cite{CHY12,MY13}. We write the subtyping relation as $T
\prec T'$, which intuitively indicates that $T$ is more constrained than $T'$
in its behaviour.

On Typing Environments we also define:

\begin{itemize}
	\item a subtyping relation where $\Gamma \prec \Gamma'$ means that $\Gamma$
	and $\Gamma'$ are identical Typing Environments up to some local types that
	are more constrained in $\Gamma$ --- i.e., subtypes of a correspondent local
	type --- than in $\Gamma'$;
	
	\item an annotated reduction relation of the form $\Gamma \lto{\beta} \Gamma'$
	where the annotation labels are a subset of the labels $\beta$ used to
	annotate the semantics of AC;

	\item a correspondence operator on labels to match reductions on Types and
	on FCs.
\end{itemize}

Finally we prove Subject Reduction (Theorem~\ref{thm:paper_subj_red}) by
proving the stronger result below.

\def\thmSR{\Thm\ref{thm:sub_red}}
\begin{theorem}[Typing Soundness\label{thm:sub_red}]
	Let $\env,C$ be an annotated FC and $\Gamma \hlseq {\env,C}$ for some
	$\Gamma$:
	
	\begin{description}
	
		\item if $\beta \neq \tau$ and $\env,C \lto{\beta}
			\env',C'$\, then $\Gamma \lto \beta \Gamma'$ and $\Gamma' \hlseq
			{\env',C'}$;
	
		\item if $\env,C \lto{\tau}  \env',C'$ then, for some
		$\Gamma'$, $\Gamma' \hlseq {\env',C'}$.

	\end{description}
\end{theorem}

\begin{proof}
The proof is by induction on the derivation of $\env,C \lto{\beta} \env',C'$.
\end{proof}

To prove Session Fidelity (Theorem~\ref{thm:session_fidelity}) we prove the
Lemma below for which, if a typing environment $\Gamma$ includes local types
that are projection of a global type $G$, then if the global type can reduce,
also the typing environment can reduce and the reduction preserves the
correspondence between the reduced global type and the reduced local types in
$\Gamma$.

\begin{lemma}[Type-Environment Fidelity\label{lemma:session_fidelity}]
	Let $\Gamma = \Gamma_*,\epp{G}{k}$ for some $\Gamma_*$, $k \not \in
	\Gamma_*$, and $G \lto{G_\m{act}(\beta)} G'$ then $\Gamma \lto \beta
	\Gamma'$ and for some $\Gamma_*'$, $k \not \in \Gamma_*'$, $\Gamma' =
	\Gamma_*',\epp{G'}{k}$.
\end{lemma}

\begin{proof}
	Direct by cases on the derivation of $\Gamma$.
\end{proof}

The proof of Theorem~\ref{thm:session_fidelity} follows directly from
Theorem~\ref{thm:sub_red} and Lemma~\ref{lemma:session_fidelity}.

\subsubsection{Proof of Deadlock Freedom}

Like in \cite{CM13,MY13}, our choreographies enjoy deadlock-freedom provided
that they \emph{i}) do not contain free variable names and \emph{ii}) are
\emph{well-sorted}, i.e., they have no undefined procedure calls. 

The proof of Theorem~\ref{thm:deadlock-freedom} is by induction on the
structure of $C$.

\subsubsection{Proof of FC to BC Encoding}

To prove Theorem~\ref{thm:encoding_operational_correspondence}, we analyse its
parts: \emph{(Completeness)} and \emph{(Soundness)}

The proof of Completeness is by induction on the derivation of $\env,C$. The
main observation is that the encoded system $\geneenc{\env},C$ enacts the
same semantic rule applied by $\env,C$. The only interesting case is for the
starting of a new session, where $\aenv$ and $\eenc{\env'}{\Gamma'}$ can differ
only on the correlation keys (note, their values, not their paths) used in the
newly created session to identify the related queues, which holds by the definition of $\did{\aenv}{Start}$, Definition~\ref{def:session_descriptor}, and the algorithm of encoding (Definition~\ref{fig:algo_encoding_deployment}). For this reason, we can replace $\aenv$ with $\eenc{\env'}{\Gamma'}$ preserving the same semantics of the choreography.

We can extend the same observation also for Soundness, which is proved by
induction on the derivation of $\geneenc{\env},C$.

\subsubsection{Proofs of Endpoint Projection}

To prove our result on the Endpoint Projection we first define the minimal
typing system $\hlseqmin{}$ for AC, reported in
Figure~\ref{fig:minimal_typing}. In the definition of minimal typing, we use
the definition of subtyping for global types $G \prec G'$.

\begin{definition}[Global and Local Subtyping]
	$G \prec G'$ is the smallest relation over closed and unfolded global types
	satisfying the rules below

	$$
		\begin{array}c
			
		\infer[\did{SubG}{Com}]
		{
			\gcom{\role A}{\role B}{\{o_i(U_i);G_i\}_{i \in I}} \prec
			\gcom{\role A}{\role B}{\{o_j(U'_j);G'_j\}_{j \in J}}
		}
		{
			I \subseteq J
			&
			\forall\ i \in I,\ G_i \prec G'_i \ \wedge U_i \prec U_i'
		}
		\\[10pt]
		\infer[\did{SubG}{Recv}]
		{
			\grecv{\role A}{\role B}{o(U);G} \prec
			\grecv{\role A}{\role B}{o(U');G'}
		}
		{
			U \prec U'
			&
			G \prec G'
		}
		\\[10pt]
		\infer[\did{SubG}{Eq}]
		{
			G \prec G'
		}
		{
			G'' \prec G'
			&
			( G'' \approx G \ \vee \ G'' \swapG G )
		}
		\qquad
		\infer[\did{SubG}{End}]
		{ \gend \prec G }
		{ \gend \approx G }
		\end{array}
	$$

\end{definition}

We extend the subtyping relations for local and global types to set inclusion
and point-wise to \emph{i}) the typing of services (i.e., of kind $\pair{\til
l} {\serviceTyping{G} {\role A}{\til{\role B}}{\til{\role C}}}$) and \emph{ii})
the typing of sessions, respectively. Given two types $G$ and $G'$, we denote
their least upper bound wrt $\prec$ with $G \lub G'$ (the same for local types
and typing environments). Our definition of subtyping for global types
follows~\cite{MY13}.

\input{figures/minimal_typing}

Like in~\cite{MY13} our EPP projects recursive definitions of the same
procedure from the point of view of different processes, therefore the same
definition has different types according to the process on which it has been
projected. Similarly to~\cite{MY13}, to deal with this discrepancy we define
the projection of typing environments. 

To give such definition, we slightly enrich the typing system such that the
judgement for procedures $\pair{X}{\Gamma}$ carries also the set of processes
that take part in it, written $\pair{X}{(\Gamma, \mathbb{P})}$ where if process
$\pid p \in \mathbb{P}$ then $\pid p$ takes part into procedure $X$. When we
write the typing $\pair{X}{\Gamma}$ in which $\mathbb{P}$ is omitted, we mean
$\pair{X}{(\Gamma, \emptyset)}$.

We also report the modified rules $\did{T}{Def}$ and $\did{T}{Call}$:

$$\infer[\did{T}{Def}]
{
	\Gamma \hlseq{\recDef{X}{C'}{C}}
}
{
	\Gamma,\pair{X}{(\Gamma',\pn(C'))} \hlseq{C}
	&
	\Gamma', \pair{X}{(\Gamma',\pn(C'))} \hlseq C'
	&
	\Gamma' |_{\locs} \subseteq \Gamma
}$$

$$\infer[\did{T}{Call}]
{
	\Gamma, \Gamma'', \pair{X}{(\Gamma', \mathbb{P})} \hlseqmin{X}
}
{
	\m{end}(\Gamma)
	&
	\Gamma'' \subseteq \Gamma'
}$$

% Note that we give the definition of $\epp{\Gamma}{}$ over annotated ACs,
% i.e., ACs where any procedure $X$ is annotated, e.g., $X\carr{\pids p}$,
% where $\pids p$ are the process identifiers of the active processes in the
% body of $X$. Formally, given a choreography $C$, it is always possible to
% have its annotated version with operator $@C$, defined following the rules in
% Figure~\ref{fig:cc_annotation}.

In the reminder of this section, we refer to $\Gamma$ as this enriched version.

Now, we define the typing projection for $\Gamma$:

\begin{definition}[Typing Projection\label{def:typing_projection}]
Let $\Gamma = \Gamma',\Gamma_\m{def}$ where $\nexists\ \pair{X}{\Gamma^*} \in
\Gamma'$ and $\Gamma_\m{def} = \Gamma \setminus \Gamma'$ ($\Gamma_\m{def}$ contains
only typings of recursive procedures). The projection of $\Gamma$, written
$\epp{\Gamma}{}$, is defined as:
%
$$
\epp{\Gamma}{} = \Gamma',\left\{\ 
		\pair{X}{\epp{\Gamma_x}{\pid p}} \ | 
		\ \pair{X}{(\Gamma_x, \mathbb{P})} \ \in \ \Gamma
		\ \wedge \
		\pid p \in \mathbb{P}
	\ \right\}
$$
%
where
%
$$
\epp{\Gamma}{\pid p} =
	\begin{array}l
	\big\{\
		\pair{\pid p.x}{U} \ | \ \pair{\pid p.x}{U} \in \Gamma
	\ \big\} \ \cup 
	\\[5pt]
	\big\{\
		\pair{\pid p}{k[\role A]}, \pair{k[\role A]}{T} \ | \
		\{ \pair{\pid p}{k[\role A]}, \pair{k[\role A]}{T} \} \subseteq \Gamma
	\ \big\} \ \cup
	\\[5pt]
		\big\{\
		\pair{ X }{ \epp{\Gamma'}{\pid p} } \ | \
			\pair{X}{(\Gamma',\mathbb{P})} \in \Gamma \ \wedge \
			\pid p \in \mathbb{P}
	\ \big\} \ \cup
	\\[5pt]
	\big\{
	\pair{l}{\serviceTyping{G}{\role A}{\roles B}{\roles C}} \ | \
	\pair{l}{\serviceTyping{G}{\role A}{\roles B}{\roles C}} \in \Gamma
	\big\}
	% \
	% \big\{\
	% 	\pair{\btype[k]^\role B_{\role A}}{T} \ | \ \{\pair{\pid p}{k[\role
	% 	A]},\pair{\btype [k]^\role B_\role A}{T}\} \subseteq \Gamma
	% \ \big\}
	\end{array}
$$

\end{definition}

% \input{figures/annotation}

% To proceed in the proof of Theorem~\ref{thm:epp}, we define well-annotated
% (Applied) Choreographies as ACs where annotated procedures report the names
% of the active processes in their bodies.

We proceed to prove Lemma~\ref{lemma:chor_EPP_typing_preservation} that states
that given a choreography $C$ and a typing environment $\Gamma$ for which
$\Gamma \hlseqmin{C}$ then $\epp{\Gamma}{}$, the projection of $\Gamma$, types
minimally the projection of $C$, $\epp{C}{}$.

\begin{lemma}[Choreography EPP Typing
	Preservation\label{lemma:chor_EPP_typing_preservation}] Let $C$ be a
	choreography and let $\Gamma \hlseqmin C$ then $\epp {\Gamma} {} \hlseqmin
	{\epp {C} {}}$.
\end{lemma}

\begin{proof}
The proof is by induction on the typing derivation of $\Gamma \hlseqmin{C}$.
\end{proof}


\noindent We finally prove Theorem~\ref{thm:EPP_typing_preservation}.

\noindent\textbf{Theorem~\ref{thm:EPP_typing_preservation}} (EPP Type
Preservation) Let $\Gamma \hlseqmin {\env,C}$ then $\epp{\Gamma}{}
\hlseqmin {\env,\epp {C} {}}$.

\begin{proof}
	To prove Theorem~\ref{thm:EPP_typing_preservation} we need to prove that we
	can apply Rule $\did{Min}{\env C}$ on $\epp{\Gamma}{} \hlseqmin {\env, \epp
	{C}{}}$

	$$
	\infer[\did{Min}{DC}]
	{\epp{\Gamma}{} \hlseqmin { \env, \epp{C}{} } }
	{
		\pco( \epp{\Gamma}{} )
		&
		\epp{\Gamma}{} \hlseqmin { \env }	
		&
		\epp{\Gamma}{} \hlseqmin { \epp{C}{} }
	}
	$$
	
	where
	\begin{itemize}
		\item $\pco(\epp{\Gamma}{})$ and $\epp{\Gamma}{} \hlseqmin{ \env }$ hold
		because $\epp{\Gamma}{}$ alters only procedure definitions in $\Gamma$;
		\item $\epp{\Gamma}{} \hlseqmin{ \epp{C}{} }$ holds from
		Lemma~\ref{lemma:chor_EPP_typing_preservation} and the assumption of
		well-sortedness on $C$ (if $C$ is well-sorted also $\epp{C}{}$ is
		well-sorted and typable by $\Gamma$).
	\end{itemize}

\end{proof}


Before proving Theorem~\ref{thm:epp_appendix} we define some auxiliary concepts
to establish a correspondence between a choreography and its projection.

Following our definition of EPP, the projection of $\prid{start}$ terms on
service processes yield a parallel composition of $\prid{acc}$ terms on the
locations subject of the $\prid{start}$. However, the reduction of a
$\prid{start}$ term might remove the availability to start new processes on the
locations subject of the $\prid{start}$ (i.e., if the reductum does not contain
another $\prid{start}$ term on the same locations). Contrarily, $\prid{acc}$
terms remain always available.

A similar observation can be drawn between conditional branches that contain
$\prid{com}$ terms whose projection merges all possible communications into
$\prid{recv}$ and $\prid{send}$ terms. Also in this case, reducing the
condition and projecting the result yields a subset of all possible branches
for the considered communication.

Similarly to~\cite{MY13} and~\cite{CHY12}, we deal with these asymmetries by
introducing the \emph{pruning relation}, which allows us to ignore unused
\emph{i}) endpoint services and \emph{ii}) input branches.

Like in~\cite{CHY12} we can write $\epp{C}{} \prec C'$ as its does not lose any
precision since it is always possible to reconstruct appropriate typings.

The $\prec$ relation is a typed strong bisimulation because if $\epp{C}{} \prec
C'$ then $\epp{C}{}$ and $C'$ have the same observable behaviours except for
the visible input actions at pruned inputs (either input branches or services).

\begin{lemma}[Pruning Lemma\label{lemma:pruning_lemma}]
	$\prec$ is a strong reduction bisimilation over partial choreographies if
	$\epp{C}{} \prec C'$ and for some $\env$, $\env'$
	\begin{itemize}
		\item if $\env,\epp{C}{} \to \env',C''$ then $\env,C' \to \env',C'''$ and
		$C'' \prec C'''$ and
		\item if $\env,C' \to \env,C'''$ then $\env,\epp{C}{} \to \env,C''$ and
		$C'' \prec C'''$
	\end{itemize}
\end{lemma}

\begin{proof}[Proof]
	Since $\epp{C}{} \prec C'$ we know that $C'$ does not use any of the
	locations not typed by the minimal typing of $\epp{C}{}$. Similarly, the
	input branches pruned in $\epp{C}{}$ are only those that are never used in
	$C'$ and cannot contribute in the reduction.
\end{proof}

Then we prove Theorem~\ref{thm:epp_appendix} by proving \emph{(Completeness)}
by induction on the derivation of $\env,C \lto{\beta} \env',C'$ and
\emph{(Soundness)} by induction on the structure of $C$, which concludes the
proof of Theorem~\ref{thm:epp}.

\subsubsection{Proofs of Compiler}

The proof of Corollary~\ref{lemma:epp_encoding_correspondence} is trivial from the definition of Theorem~\ref{thm:epp} and Theorem~\ref{thm:encoding_operational_correspondence}.

To prove Theorem~\ref{thm:compilation_operational_correspondence} we prove the
following auxiliary results.

\begin{lemma}[Compilation Invariance\label{lemma:untitled}]
	Let $\Gamma \hlseq{\env,C}$, $\env,C \to \env',C'$, and $\Gamma'
	\hlseq{\env',C'}$ for some $\Gamma'$, $\filter{\Gamma}{\locs} =
	\filter{\Gamma'}{\locs}$ and $\{\pid p@l \ | \ \pid p@l \in \Gamma \} =
	\{\pid p@l \ | \ \pid p@l \in \Gamma' \}$, then $\genenc{\env',C'} =
	\genencp{\env',C'}$.
\end{lemma}
\begin{proof}[Proof]
	By cases on the derivation of $\env,C \to \env',C'$. From
	Definition~\ref{def:compilation}, the only information used by the compiler
	present in $\Gamma$ (respectively $\Gamma'$) are \emph{i}) the location of
	running processes ($\pid p@l$) and \emph{ii}) the service typings
	($\pair{\til l}{\serviceTyping{G}{\role A}{\roles B}{\roles C}}$).
	Therefore, provided $\Gamma$ and $\Gamma'$ have the same service typings and
	locations the compilation of the given choreography under $\Gamma$ produces
	the same result as the compilation of such choreography under $\Gamma'$.
\end{proof}

We provide some auxiliary results on variable substitution. We remind that the
only bound names in $DCC$ are the variables in $\prid{accept}$ terms (e.g.,
$x$ in $!(x);B$). However, the following lemmas prove that renaming free
variables with fresh names in processes (and, by extension, in services)
preservers bisimilarity.

In the following, we abuse the notation for $\alpha$-renaming to denote
variable renaming in running processes.

We define the variable renaming operator for DCC processes $P[x'/x]$.

\begin{definition}[DCC Variable Renaming Operator\label{def:variable_renaming}]
 Let $\jprc{B}{t}{M}$ be a DCC process, then $(\jprc{B}{t}{M})[x'/x] =
 \jprc{B[x'/x]}{t\tcopy{x'}{x(t)}\tcopy{x}{t_\bot}}{M}$ where $B[x'/x]$
 substitutes every occurrence of $x$ with $x'$.
\end{definition}

\begin{lemma}[DCC Process Variable Renaming\label{lemma:variable_renaming}]
	Let $P$ and $P'$ be two DCC processes such that $P=\jprc{B}{t}{M}$ and $P' =
	P[x'/x]$ and $x'$ is fresh in $B$ then $P \lto{\lambda} P'' \iff P'
	\lto{\lambda[x'/x]} P''[x'/x]$.
\end{lemma}

\begin{proof} 
The proof is by induction on the form of $P$.
\end{proof}

\paragraph{Completeness of Theorem~\ref{thm:compilation_operational_correspondence}.}
We can now prove \emph{(Completeness)} of
Theorem~\ref{thm:compilation_operational_correspondence}, which is done by
induction on the derivation of $\env,C \to \env',C'$.

The only interesting case, is that of the start of a new session $\genstart$,
where $\env,C$ creates a fresh session name, e.g., $k'$ and a set of new
process names $\pids r$. In $\genenc{\env,C}$, we mimic the evolution on fresh
names by first executing the whole sequence of actions to start the session in
DCC using $k$, let $\genenc{\env,C} \to^+ S$, then to prove $\enc{\env',C'} =
S$ \emph{i}) by Lemma~\ref{lemma:variable_renaming} we can $\alpha$-rename in
$S$ the path rooted in $k$ to $k'$ in the state of the involved processes
(i.e., those that are the compilation of processes $\{\pid p, \pids q\}$) and
\emph{ii}) thanks to Theorem~\ref{thm:encoding_operational_correspondence}, we
show that we can obtain a $\Gamma'$ for which $\eenc{\env'}{\Gamma'} = \aenv$
and $\aenv$ is compliant to the locations, states, and the queues maps in $S$.



\paragraph{Soundness of
Theorem~\ref{thm:compilation_operational_correspondence}.}

To prove \emph{(Soundness)} of
Theorem~\ref{thm:compilation_operational_correspondence} we extend the
semantics of DCC with annotations on transitions to bear the paths on which
operations are executed.

We range over transition labels with $\lambda$.
$$\lambda \gram x \ \Div \ \cq{x} \ \Div \ ?(x) \ \Div \ o \qfrom{x} \ \Div \
o@x \ \Div \ \tau$$

We also introduce the filtering and complement operators on sequences of DCC
transition labels. Let $\lambda,\til \lambda$ be a sequence of DCC labels, the
filtering of $\lambda,\til \lambda$ on $k$ , written $\filter{(\lambda,\til
\lambda)}{k}$ is defined as
%
$$
	\filter{(\lambda,\til \lambda)}{k} =
		\begin{cases}
			\lambda,(\filter{\til \lambda}{k}) & \mbox{if }
				\lambda \in \left\{ 
					\begin{array}c
						\jpath{k.x.y},\ \cq{\jpath{k.x.y}},\ ?(\jpath{k}),\\
						sync\qfrom{\jpath{k.x.y}},\ sync@\jpath{k.x.y}, \\
						start	\qfrom{\jpath{k.x.y}},\ start@\jpath{k.x.y} 		
					\end{array}
				\right\}
			\\
			\filter{\til \lambda}{k} & \mbox{otherwise}
		\end{cases}
$$

%
Let $\lambda_1,\til \lambda_1$ and $\lambda_2,\til \lambda_2$ be two sequences
of DCC labels, the complement of $\lambda_1,\til \lambda$ on $\lambda_2,\til
\lambda_2$ , written $(\lambda_1,\til \lambda_1)/(\lambda_2,\til \lambda_2)$ is
defined as
%
$$
	(\lambda_1,\til \lambda_1)/(\lambda_2,\til \lambda_2) =
	\begin{cases}
		\til \lambda_1/\til \lambda_2 & \mbox{if } \lambda_1 = \lambda_2 \wedge
		\til \lambda_2 \subseteq \til \lambda_1
		\\
		\lambda_1,(\til \lambda_1/(\lambda_2,\til \lambda_2)) & \mbox{if }
		\lambda_1 \neq \lambda_2 \wedge (\lambda_2,\til \lambda_2) \subseteq \til
		\lambda_1
	\end{cases}
$$

Below we state Lemma~\ref{lemma:dcc_permutations} that proves that we can
permute the order of transitions in DCC systems and obtain the same final
configurations. In particular, we prove such result on transitions that regard
the start of new sessions. The proof of Lemma~\ref{lemma:dcc_permutations} is
based on the simpler Lemma~\ref{lemma:dcc_single_permutation} that proves that
we can change the order of one start transition and eventually obtain the same
DCC system.

\begin{lemma}[Single DCC Start Permutation\label{lemma:dcc_single_permutation}]
	Let S be a composition of DCC services such that $S \lto{\til \lambda_1} S_1$
	and $S_1 \lto{\lambda_2} S_2$ where $\filter{\til \lambda_1}{k} = \emptyseq$
	and $\filter{\lambda_2}{k} = \lambda_2$ then $S \lto{\lambda_2} S_1'$ and
	$S_1' \lto{\til \lambda_1} S_2$.
\end{lemma}

\begin{proof}[Proof]
	The proof is by induction on the length of $\til \lambda_1$. Note that we can
	exclude to have transitions on session $k$ in $\til \lambda_1$ since by the
	premises they happen before $\lambda_2$ which, by the premises, at most may
	correspond to the last transition of the start of session $k$. 
\end{proof}

\begin{lemma}[DCC Start Permutations\label{lemma:dcc_permutations}]
	Let $S$ be a composition of DCC services such that $S \lto{\til
	\lambda} S'$ and $\til \lambda = (\jpath{k.C.l},\til \lambda')$ then $S
	\lto{\filter{\til	\lambda}{k}} S''$ and $S'' \lto{\til \lambda/\filter{\til
	\lambda}{k}} S'$.
\end{lemma}

\begin{proof}[Proof]
	Let $\filter{\til \lambda}{k} = \lambda^k_1,\ldots,\lambda^k_m$ and 
	$$
	\til \lambda = \lambda^k_1,\lambda_{1.1},\ldots,\lambda_{1.n_1},\ldots
								 \lambda^k_i,\lambda_{i.1},\ldots,\lambda_{i.n_i},\ldots
								 \lambda^k_m,\lambda_{m.1},\ldots,\lambda_{m.n_m}
	$$
	we can apply Lemma~\ref{lemma:dcc_permutations} inductively on each couple
	of the kind $\lambda^k_i$ and $\lambda_{i.1},\ldots,\lambda_{i.n_i}$, $i \in
	\{1,\ldots,n\}$.
	%
	Note that the proof holds also for configurations of $\til \lambda$ in which
	the elements of $\filter{\til \lambda}{k}$ appear next to each other (e.g.,
	$\til \lambda = \lambda^k_1,\ldots,
	\lambda^k_i,\lambda^k_i+1,\ldots,\lambda_{m.n_m}$) since it is a base case
	of Lemma~\ref{lemma:dcc_single_permutation} in which there are no
	transitions in $\til \lambda_1$.
\end{proof}


Next we state Lemma~\ref{lemma:start_completion} that proves that,
\emph{i}) given a well-typed FC choreography, \emph{ii}) its DCC projection,
and \emph{iii}) the DCC system that results from a sequence of reductions
belonging to the start of a session, we can complete the remaining sequences
of interactions and obtain the originating FC choreography after the reduction
to start the session.

\begin{lemma}[DCC Start Completion\label{lemma:start_completion}]
Let $\Gamma \hlseq{\env,C}$,

$$C= \req{k}{\prc pA}{l_1.[\role
B_1],\ldots,l_n.[\role B_n]};C_r \pp \prod_{i=1}^{n}\acc{k}{l_i.\pid q_i[\role
B_i];C_{\pid q_i}}$$ 

$\env,C \to \env',C'$, and $\genenc{\env,C}=S$ such that
$S \lto{\til \lambda} S'$ where $\filter{\til \lambda}{k} = \til \lambda$ then
\emph{i}) $S' \lto{\til {\lambda'}} S''$, and \emph{ii}) there exists some
$\Gamma'$ s.t. $\Gamma' \hlseq{\env',C'}$ and $\genencp{\env',C'} = S''$.
\end{lemma}

\begin{proof}
Proof by case analysis on the length of $\til \lambda$. The intuition is that
the only available action for $\env,C$ is a start. Then, we let the compiled
DCC system $S$ do some of the actions, contained in $\til \lambda$, for that
start, reaching state $S'$. In the conclusions of the Lemma, we can complete
the actions for the start, leading $S'$ to $S''$ and we can find $\Gamma' \hlseq{\env',C'}$ for which $\enc{\env,C}^{\Gamma'} = S''$.

\end{proof}

Finally, the proof of \emph{(Soundness)} of
Theorem~\ref{thm:compilation_operational_correspondence} is by induction on the
cardinality of $\til \lambda$. The proof strategy for the inductive cases is to
consider the actions in $\til \lambda$ (where $|{\til \lambda}| = 0$ and $|{\til \lambda}| = 1$ are base cases), let $|{\til \lambda}| = n$, if the first action it is
not the first belonging to a start of a new session, then we can easily prove the conclusion of the Soundness for that action because we have 1:1
correspondence between the evolution of DCC and FC for that action (e.g., think of the sending or reception of a message). Then, we can proceed by induction on the remaining $n-1$ actions in $\til \lambda$. 

Contrarily, if the first action in $\til \lambda$ is the first action of the
start of a new session, we filter $\til \lambda$ from all the actions in it
that correspond to that start (e.g., if the start is on a session $k$, we
filter out all the DCC actions for that $k$ with $\filter{\til \lambda}{k}$).
In the conclusion of the Soundness case, we execute the remaining actions to
complete the start and we let $\env,C$ to execute the same start, transitioning
to $\env',C'$. Thanks to Lemma~\ref{lemma:start_completion} the compilation of
the final FC choreography is equal to the obtained DCC system. Thanks to
Lemma~\ref{lemma:dcc_permutations}, we can proceed by induction on the
remaining labels in $\til \lambda$ where we removed those belonging to
$\filter{\til \lambda}{k}$.

\paragraph{Proof of Corollary~\ref{thm:applied_choreographies}.}
The proof of Corollary~\ref{thm:applied_choreographies} derives from the
application of Corollary~\ref{lemma:epp_encoding_correspondence},
Theorem~\ref{thm:compilation_operational_correspondence}, and
Lemma~\ref{lemma:endpoint_projection} (below).

\begin{lemma}\label{lemma:endpoint_projection}
	Let $\Gamma \hlseq{C}$ then $\epp{C}{}$ is a composition of endpoint
	choreographies
\end{lemma}
\begin{proof}
	Trivial from the Definition of $\Gamma \hlseq{C}$ and
	Definition~\ref{def:epp}.
\end{proof}


==> proofs/figures/annotated_chor_syntax.tex <==
%auto-ignore
\begin{figure}
{\arraycolsep=1.4pt\def\arraystretch{1.3} \small
\begin{displaymath}
\begin{array}{rlclll}
C \gram & \til n. \eta ; C 												& \prid{seq}
	& \Div & \cond{\pid p.e}{C_1}{C_2} 							& \prid{cond}
	\\
	\Div 	& C_1 \pp C_2 														& \prid{par}
	& \Div & \recDef{X}{C^\prime}{C}								& \prid{rec}
	\\
	\Div & \recCall{X}															& \prid{call}
	& \Div & \til n. \genbranchI										& \prid{recv}
	\\
	\Div & \inact																		& \prid{inact}
	& \Div & \til n. \genacc ; C										& \prid{acc}
% \\[.4em]
% H \gram & \pid p( \til x, \til k) &&&
% I \gram \; \pid p( \til e, \til k)
\\[.3em]
\eta \gram & \genstart 														& \prid{start}
	&		\Div & \genreq															& \prid{req}
	\\ 	\Div & 	\gencom 														& \prid{com}
	&		\Div & \gensend															& \prid{send}
\\[.3em]
R \gram & \dep, C
\end{array}
\end{displaymath}
}
\caption{Choreography Calculus - Annotated Syntax}
\label{fig:cc_annotated_syntax}
\end{figure}

==> proofs/figures/annotated_jc_syntax.tex <==
%auto-ignore
\begin{figure}
\begin{displaymath}
	\begin{array}{lcll}
		% S & \gram & \jsrv{B_s,P}{l} \quad \Div \quad S \pp S'
		S & \gram & \jsrv{B_s, P}{l} \quad \Div \quad S \pp S'
		\\[.3em]
		B_s & \gram & \wtil m.!(\jpath x);B
		\\[.3em] 
		P & \gram & \jprc{B}{t}{M} \quad \Div \quad P \pp P'
		\\[.3em] 
		B & \gram & \wtil m.\sum_{i}\choice{o_i(\jpath x_i) \qfrom \jpath{q}}{B_i} 
																													&	\prid{choice}
		\\[.3em] & \Div & \wtil m.o(\jpath x) \qfrom \jpath{q}; B  & \prid{input}
		\\[.3em] & \Div & \wtil m.?@e_1( e_2 );B                   & \prid{start}
		\\[.3em] & \Div & \wtil m.o@e_1( e_2 ) \qto \jpath{q};B    & \prid{output}
		\\[.3em] & \Div & \wtil m.\jpath{x} = e;B                  & \prid{assign}
		\\[.3em] & \Div & \wtil m.\cq{e};B                         & \prid{cqueue}
		\\[.3em] & \Div & \til m.\cond{e}{B_1}{B_2}                  & \prid{cond}
		\\[.3em] & \Div & \recDef{X}{B'}{B}										& \prid{rec}
		\\[.3em] & \Div & \mbox{X}														& \prid{call}
		\\[.3em] & \Div & \inact                              & \prid{inact}
	\end{array}
\end{displaymath}
	\caption{Correlation Calculus, annotated syntax}
	\label{fig:jc_annotated_syntax}
\end{figure}

==> proofs/macros.tex <==
% % %


==> proofs/operational_correspondence_BC_FC.tex <==
%auto-ignore
To prove Theorem~\ref{thm:encoding_operational_correspondence}, we analyse its
parts: \emph{(Completeness)} and \emph{(Soundness)}

The proof of Completeness is by induction on the derivation of $\env,C$. The
main observation is that the encoded system $\geneenc{\env},C$ enacts the same
semantic rule applied by $\env,C$. The only interesting case is for the starting
of a new session, where $\aenv$ and $\eenc{\env'}{\Gamma'}$ can differ only on
the correlation keys (note, their values, not their paths) used in the newly
created session to identify the related queues, which holds by the definition of
$\did{\aenv}{Start}$, Definition~\ref{def:session_descriptor}, and the algorithm
of encoding (Definition~\ref{fig:algo_encoding_deployment}). For this reason, we
can replace $\aenv$ with $\eenc{\env'}{\Gamma'}$ preserving the same semantics
of the choreography.

We can extend the same observation also for Soundness, which is proved by
induction on the derivation of $\geneenc{\env},C$.

==> proofs/proof.tex <==
%auto-ignore
% \newenvironment{subfigure}[1]{%
% 	\begin{minipage}[c]{#1}%
% 	}{%
% 	\end{minipage}%
% 	}

\section{Proofs of Subject Reduction and Session Fidelity\label{sec:proof_of_typing}}
\input{applied_choreographies/proofs/subject_reduction}

\section{Proof of Deadlock Freedom\label{sec:proof_of_deadlock_freedom}}
\input{applied_choreographies/proofs/deadlock-freedom}

\section{Proof of Endpoint Projection} % (fold)
\label{sec:proof_of_endpoint_projection}

\input{applied_choreographies/proofs/epp}

\section{Proof of Compilation} % (fold)
\label{sec:proof_of_applied_choreographies}

\input{applied_choreographies/proofs/applied_choreographies}

==> typing.tex <==
%auto-ignore

We equip FC with a typing discipline based on Multiparty Session
Types~\cite{HYC08,CDYP2015}, which checks that partial actions composed in
parallel are compatible. Our typing discipline is a straightforward adaptation
of that presented for Compositional Choreographies~\cite{MY13}, so we omit
most details here (see Appendix). However, the type system also gives us
important information that will be critical in the compilation that we will
develop later. Specifically, we use types to keep track of the location that
each process has been created at, the types of variables, the roles played by
processes in open sessions, and the role played by the processes spawned at
each location in a choreography. Keeping track of this information is obvious;
hence, for brevity, we simply report the definition of the typing environments
$\Gamma$ that we use to store it.
%
%We define our type system on the typing environment $\Gamma$. Below, we
%report and comment the main elements of $\Gamma$.
%
\vspace{-0.3cm}
$$
	\Gamma \gram \Gamma,
		\;\; 
			\geninitg 
		\;\; \Div \;\; 
		% 	\Gamma, k[\role A] : T
		% \;\; \Div \;\; 
			\Gamma, \pid p : k[\role A]
		\;\; \Div \;\; 
			\Gamma, \pid p.x : U
		% \;\; \Div \;\; 
			% \Gamma, X: \Gamma
		\;\; \Div \;\; 
		\;\; \Gamma, \pid p@l
		\;\; \Div \;\; 
			\emptyset
$$
%
In $\Gamma$, a \emph{service typing} $\geninitg$ types with the (standard, from~\cite{CDYP2015,MY13})
\emph{global type} $G$ any session started by contacting the services at the locations $\til l$. Role $\role A$ is the role of the active process, whereas roles $\roles B$ are the respective roles of the service processes located at $\til l$. (The roles $\roles C$ are used to keep track of whether the implementation of some roles is provided by external choreography modules.)
%For $\til l = l_1,\ldots,l_n$ and $\roles B = \role
%B_1, \ldots, \role B_n$, e.g., for $\Gamma,\geninitg$, all service
%processes started at $l_1$ play role $\role B_1$.
%As in~\cite{MY13},
%we use $\roles C$ (where $\roles C \subseteq \roles B$) to range over the roles
%implemented by the choreography typed by $\Gamma$: this enables modularity and
%forbids the composition of partial choreographies that implement the same
%roles.
%
% When we write $\Gamma, \geninitg$, we always assume that: \emph{i}) $\{\role
% A, roles B\} = \auxRoles(G)$, where $\auxRoles$ returns the set of roles in
% $G$; \emph{ii}) the locations $\til l$ are ordered lexicographically; and,
% \emph{iii}) the locations in $l$ do not appear in any other service typing in
% $\Gamma$.
%
% A \emph{session typing} $k[\role A] : T$ states that role $\role A$ follows the type $T$ in session $k$.
%
% We assume that roles in a session are typed by a
% single local typing, as in standard Multiparty Session Types~\cite{HYC08}.
%
An \emph{ownership typing} $\pid p : k[\role A]$ states that process $\pid p$
owns the role $\role A$ in session $k$.
%
% : each process can participate in multiple sessions, but can play only one
% role in each of such sessions. Hence, a process $\pid p$ may appear in more
% than one ownership typings in a $\Gamma$, but never more than once per
% session.
%
A \emph{location typing} $\pid p@l$ states that process $\pid p$ is runs at location $l$.
%
The typing $\pid p.x : U$ states that variable $x$ has type $U$ in the state of process $\pid p$. %and recursive procedures are standard.

% As an example, consider the rule for typing a complete communication action:
% \[
% \infer[\did{T}{Com}]
% {
% 	\Gamma, 
% 	\pair{k[\role A]}{\genlsendB},
% 	\pair{k[\role B]}{\genlrecvPrime}
% 	\hlseq{
% 		\com{k}{\pid p[\role A].e}{\pid q[\role B].o_j(x)};C}
% }
% {
% 	j \in I
% 	&
% 	% \Gamma \seq{\com{k}{\pid p[\role A]}{\pid q[\role B]}}
% 	\Gamma \seq \pair{\pid p}{k[\role A]},\pair{\pid q}{k[\role B]}
% 	&
% 	\Gamma \seq \pair{\pid p.e}{U_j}
% 	&
% 	\Gamma, \pair{\pid q.x}{U_j}, 
% 		\pair{k[\role A]}{T_j}, 
% 		\pair{k[\role B]}{T'_j}
% 		\hlseq{C}
% }
% \]
% Rule $\did{T}{Com}$ %uses types $T$ and environments $\Gamma$ to 
% checks that: \emph{i}) the chosen operation $o_j$ is among the ones that the
% sender can select, according to its local type; \emph{ii}) $o_j$ is among the
% operations offered by the receiver, according to its local type; \emph{iii})
% the processes $\pid p$ (sender) and $\pid q$ (receiver) own their respective
% roles in the session; 
% % (role ownerships are registered in the environment $\Gamma$);
% \emph{iv}) the expression of the sender ($e$) has the type
% % \footnote{The judgement $\seq t: U$ reads as ``tree $t$ has type $U$''.}
% $U_j$ expected by the protocol; \emph{v}) the receiver uses the reception
% variable accordingly in the continuation $C$; and \emph{vi}) processes $\pid p$
% and $\pid q$ proceed according to their respective types in $\Gamma$.

% \paragraph{Runtime Typing.}
% Previous choreography models~\cite{QZCY07,choOrchCorrespondence,CHY12,CM13}
% assumed that complete communications can always execute. \todo{Da controllare.
% Dato che anche in altri lavori ci sono le code, non vengono checkate dal type
% system?} Contrarily, in the semantics of choreographies in AC, Rule
% $\did{C}{Com}$ executes only if the deployment contains the intended queue of
% the receiver\todo{ora non vero per FC, perché è una funziona completa}; otherwise the choreography is deadlocked.
% %
% % ACs present a remarkable difference wrt previous works on choreographies.
% % %
% % Consider Rule $\did{C}{Com}$, the sender uses the data in its state to
% % ``find'' the receiver through correlation, but if such data do not correlate
% % with any of the queues in the deployment, the choreography becomes deadlocked.
% % %
% % Such conditions do not exist in previous works where choreographies can always
% % continue execution (see,
% % e.g.,~\cite{QZCY07,choOrchCorrespondence,CHY12,CM13}).
% %
% Thus, to ensure that well-typed FC programs never go wrong, we extend
% standard Multiparty Session Types to check that, given a running choreography
% $\env, C$, the deployment $\env$ supports the intended communications
% described in $C$.
% %
% Formally, we introduce a new typing rule:
% % 
% % 
% % % The solution to this issue constitutes the main novelty of our typing system.
% % % We extend our typing discipline to check runtime states, i.e., to check if a
% % % deployment can ``go wrong''. To do this, \emph{i}) we introduce partial
% % % receptions in our types to abstract the state of queues (following the idea
% % % presented in~\cite{DenielouY13}) and \emph{ii}) we add a judgement $\Gamma
% % % \hlseq{\env}$ to guarantee coherency between a deployment and its companion
% % % choreography, e.g., that queues have distinct correlation keys in the same
% % % location and message queues contain exactly the messages expected by the
% % % protocol that types the session they belong to.
% %
% % that message queues do not contain messages unexpected by the
% % protocol of the session in which their are used.
% % % 
% % % Formally, we extend $G$ with a new global type that represents partial
% % % receptions, we define a new kind of local types, called \emph{buffer types}
% % % and denoted $\btype[k]_\role B^\role A$, for typing message queues, and we
% % % extend global-type projection to relate global partial receptions with buffer
% % % types, i.e., projection $\epp{G}{\role B}^{\role A}$ returns the buffer type
% % % of the queue used by role $\role B$ to receive messages from role $\role A$ in
% % % session $k$.
% %
% % % Finally, we extend our typing discipline with a new Rule $\did{T}{\env C}$
% % % that checks for coherence among types, choreographies, and deployment. To
% % % define $\did{T}{\env C}$, we formalise a predicate, called \emph{partial
% % % coherence}\footnote{Partial because it accounts for missing typings of roles
% % % implemented by external partial choreographies.} and denoted $\pco (\Gamma)$,
% % % that checks if the local typings for all sessions in $\Gamma$ follow, i.e.,
% % % are a projection of the same global type $G$.
% % % 
% % % Intuitively, in the formal definition of $\pco(\Gamma)$ we check that for all
% % % sessions $k$ in the typing environment $\Gamma$:
% % % %
% % % the local type $T$ of a role $\role B$, written $\pair{k[\role B]}{T}$ and the
% % % buffer type $\btype[k]_\role B^\role A$ of $\role B$ and any other role $\role
% % % A$ in session $k$
% % % %
% % % are projection of the same global type $G$.
% % 
% %
% % Now we define a predicate for \emph{partial coherence}\todo{forse bisogna
% % spiegare perché è ``partial''}, called $\pco (\Gamma)$, that holds if and only
% % if, for all sessions $k$, the local and buffer typings of $k$ follow (are
% % projection of) the same global type $G$.
% % %
% % The idea is that, since $\env$ is a global deployment, we can check for
% % partial coherence of all sessions in Rule $\did{T}{\env C}$.
% % 
% % % \begin{definition}[Partial Coherence] We write $\pco(\Gamma)$ when, for all
% % % sessions $k$ in $\Gamma$, there exists a global type $G$ such that
% % % %
% % % $
% % % \forall\; \pair{k[\role B]}{T} \in \Gamma \Rightarrow T = \epp{G}{\role B}\
% % % \wedge \; \forall\; \role A \in \auxRoles(G)/\{\role B\} \Rightarrow
% % % 	\Gamma \seq \pair{\btype[k]_\role B^\role A}{\epp{G}{\role B}^\role A}
% % % $
% % % \end{definition} 
% % %
% % 
% % % \noindent Then, we can define Rule $\did{T}{\env C}$ as:

% \smallskip$
% \hspace{70pt}\did{T}{\env C} 
% \quad
% \pco(\Gamma) 
% 	\quad
% \Gamma \hlseq \env
% 	\quad
% \Gamma \hlseq C
% 	\quad \Rightarrow \quad
% \Gamma \hlseq{\env,C} \quad
% $\smallskip

% \noindent
% Predicate $\pco(\Gamma)$ holds if all local types of each session in a
% judgement are coherent~\cite{HYC08,CMSY15}, i.e., that they describe
% compatible behaviours. For example, if in its local type for session $k$ role
% $\role A$ sends a message to role $\role B$, then also the local type of
% $\role B$ for session $k$ must type a reception from role $\role A$.
% %
% % $\Gamma \hlseq{\env,C}$ 
% % states that $C$ and $\env$ are coherent
% % according to $\Gamma$ and all sessions in $\Gamma$ are coherent. $\Gamma$ is an
% % abstraction between $\env$ and $C$ and guarantees $\env$ to not go wrong. %
% %
% More interestingly, the Rule introduces the \emph{deployment judgement} $\Gamma
% \hlseq{\env}$, which checks that $\env$ supports all the session
% communications typed in $\Gamma$. Moreover, note that the typing of the deployment depends on how it is structured (indeed, we model different communication technologies just by changing the deployment, as we do in \cref{sec_aEC}). Hence, we formalise $\Gamma \hlseq{\env}$ on the structure of $\env$:

% \begin{definition}[Deployment Judgements]\label{def:deployment_judgements}
% $$ \Gamma \hlseq{\env} \iff \begin{cases}
% 			(1) \ \forall\ \pid p.x \in \Gamma, \env( \pid p).x : U
% 			\\
% 			(2) \ \forall\ \chanto{k}{\role A}{\role B}: T \in \Gamma \wedge \env(\chanto{k}{\role A}{\role B}) = \til m, \ \btypeop(\role A, \til m ) = T
% 	\end{cases}
% $$
% \end{definition}
% %
% We comment the checks performed by $\Gamma \hlseq \env$:
% %
% % \begin{itemize}[topsep=5pt,itemsep=-2pt,partopsep=1ex,parsep=1ex]
% %
% 	% \item 
% 	% \item 
% 	$(1)$ checks that, for each typing $\pair{\pid p.x}{U}$ in $\Gamma$, $\env$
% 	associates $x$, in the state of process $\pid p$, to a value of type
% 	$U$;
% 	%
% 	% \item 
% 	$(2)$ uses a new type, called \emph{buffer type}, introduced in $\Gamma$ to
% 	abstract the state of message queues. A buffer type associates a queue
% 	ownership to its type $\pair{\chanto{k}{\role A}{\role B}}{T}$, i.e., to the
% 	type $T$ enacted by the messages in the queue. Check $(5)$ holds if the
% 	typing of a message queue in $\Gamma$ is correct wrt to the actual sequence
% 	of messages stored by that queue in $\env$. We extract the type of a queue $\til m$, i.e., the sequence of message receptions from a role $\role A$, with function $\btypeop(\role A, \til m)$.

% \begin{example}
% As an example of how $(2)$ works, consider the running choreography
% %
% \\
% %
% %
% $\env,\com{k}{\role C}{\pid s[\role S].buy(x)};\ldots$
% %
% %
% which is the one in \cref{example:intro} after process $\pid c$ sent its
% message to $\pid s$, applying Rule $\did{C}{Com}$. Now, the queue used by $\role S$ to receive from $\role C$ in session $k$ has one
% message on operation $buy$ that contains the ordered product, say
% \texttt{"book"}, formally $\env( \chanto{k}{\role C}{\role S} ) = (buy, \texttt{"book"})$. The extracted local type of the queue is $\btypeop(\ \role C,
% \env( \chanto{k}{\role C}{\role S} )\ ) = ?\role C.buy(\tstring)$, which, by
% $(2)$, shall match with the buffer type $\pair{\chanto{k}{\role C}{\role S}}{?\role C.buy(\tstring)} \in \Gamma$.

% \end{example}

% Notably, we can automatically perform all checks on the deployment (e.g., we
% can infer buffer types from global types), hence the programmer only needs to
% specify standard Multiparty Session Types as usual~\cite{MY13,CM13,HYC08}.
% % \todo{Sposterei in conclusions $\to$ (Actually, it would even be easy
% % to develop a complete type inference system by following the reasoning
% % in~\cite{M13:phd}.)} 

A typing judgement $\Gamma \hlseq{\env,C}$ establishes that $\env$ and $C$ are typed according to $\Gamma$. If such a $\Gamma$ exists, we say that $\env,C$ is well-typed.
%Well-typed provides the typical session fidelity property of session
%types, omitted here (see Appendix).
%
%In the remainder, we say that $\env, C$ is well-typed if there exists $\Gamma$
%such that $\Gamma \hlseq{\env,C}$.
%
%Typing ensures the standard property of session fidelity from session types~\cite{HYC08} (see Appendix).
Well-typed frontend choreographies that contain all necessary modules never deadlock.
%
\begin{theorem}[Deadlock freedom\label{thm:deadlock-freedom}]
$\Gamma \hlseq{\env,C}$ 
and $\cofn(\Gamma)$ 
imply that either (i) $C \equiv
\inact$ or (ii) there exist $\env'$ and 
$C'$ such that $\env,C \to \env',C'$.
\end{theorem}
%
Predicate $\cofn$ checks that $C$ has all the choreography modules needed by its requests terms.
%
%in $\Gamma$
%% Coherence extends partial coherence to check that
%\emph{i}) there are all needed services to start new sessions via requests and
%\emph{ii}) each role in any open session (i.e., with a free name) is played by
%a process.
%
% Coherent and well-typed systems are deadlock-free:
